Popcorns-Pro: A Cooperative Network-Server Approach for Data Center Energy Optimization

Data centers have become a popular computing platform for various applications, and they account for nearly 2% of total US energy consumption. Therefore, it has become important to optimize data center power, and reduce their energy footprint. Most existing work optimizes power in servers and networks independently and does not address them together in a holistic fashion that has the potential to achieve greater power savings. In this article, we present PopcornsPro, a cooperative server network framework for energy optimization. We present a comprehensive power model for heterogeneous data center switches along with low power mode designs in combination with the server power model. We design job scheduling algorithms that place tasks onto servers in a power-aware manner, such that servers and network switches can take effective advantage of low power state and available network link capacities. Our experimental results show that we are able to achieve significantly higher savings up to 80% compared to the previously well-known server and network power optimization policies.

==> 2020-popcorns-T-SUSC (copy)/Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}
In this article, we presented \PopCorns, where we explore techniques that make smart use of line card and port low power states in switches and orchestrate them with intelligent joint task placement and routing algorithm for more effective power management. The results show good promise in achieving considerable power savings compared to the baseline policies. Our experimental results show that smart management of low power states achieves upto 80\% over policies optimizing servers and network policies separately, while still keeping energy savings low.

==> 2020-popcorns-T-SUSC (copy)/Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}

%\todo{add more contributions to compare with the conference paper}
Data centers have spurred rapid growth in computing, and an increasing number of user applications have continued to migrate toward cloud computing in the past few years. With this growing trend, data centers now account for about 2\% of US energy consumption \cite{barrosoCaseEnergyProportionalComputing2007}. Many public cloud computing environments have power consumption in the order of several Gigawatts. Therefore, energy is key challenges in data centers.

 Data center servers are typically provisioned for peak performance to always satisfy user demands. This, however, also translates to higher power consumption. Hardware investments have resulted in power saving mechanisms, such as DVFS and low-power or idle states~\cite{acpi}. 
% Through using such mechanisms, as servers continue to become more energy-proportional, other active data center components such as the data center network are growing to dominate overall power~\cite{abtsEnergyProportionalDatacenter2010} \cite{KoutitasChallengesenergyefficiency}. Therefore, it is important to holistically address the power consumed by both data center servers and networks for an effective solution to this problem. 

We note that power reduction strategies in network switches and routers have been largely studied in large-scale network settings. Gupta et al.~\cite{guptaGreeningInternet2003} proposed a protocol-level support for coordinated entry into low-power states, where routers broadcast their sleep states for routing decisions to be changed accordingly. Adaptive Link Rate (ALR) for ethernet~\cite{gunaratneReducingEnergyConsumption2008} allows the network links to reduce their bandwidth adaptively for increased power efficiency. Such approaches may not be very effective in data center settings where application execution times have a higher dependence on network performance and Quality of Service (QoS) demands by the users. 

In this article, we propose PopCorns-Pro, a new framework to holistically optimize data center power through a cooperative network-server approach. We propose power models for data center servers and network switches (with support for low-power modes) based on power measurements in real system settings and memory power modeling tools from MICRON~\cite{lalSLCMemoryAccess2019}
and Cacti \cite{balasubramonianCACTINewTools2017}. We then study job placement algorithms that take communication patterns into account while optimizing the amount of sleep periods for both servers and line cards. Our experimental results show that we are able to achieve more than 20\% higher energy savings compared to a baseline strategy that relies on server load-balancing to optimize data center energy. 

We note that further power savings can be obtained at the application level through carefully tuning them for usage of processor resources~\cite{chenWattsinsideHardwaresoftwareCooperative2013} or through load-balancing tasks across cores in multicore processor settings to avoid keeping cores unnecessarily active. %~\cite{lime_icse11}.
Such strategies can complement our proposed approach, and boost further power savings in data center settings.

 We extended upon our previous work~\cite{luPopCornsPowerOptimization2018} by proposing a multi-state power model for data center network switches and servers based on available power measurements in real system settings and memory power modeling tools. We formulate a power optimization problem that jointly considers both server
(with multiple cores) and network switches (with multiple line cards). We improve network traffic modeling accuracy by including link capacities. We also consider realistic heterogeneous switches in the Fat tree topology with different performance and power characteristics for switches at Core, Aggregate and Edge levels.
We compare our approach against a server load-balancing mechanism for task placement and a traditional Djikstra based network routing algorithm. We also consider a server energy optimization algorithm and a greedy bin packing network routing policy which consolidates traffic into fewer switches. These four policy combinations are compared with our Popcorns server algorithm to find that a combined server-network energy aware algorithm is more efficient than optimized versions of individual approaches previously considered as datacenter energy optimization. We consider real world job arrival traces, as well as with synthetic bursty arrivals at different job network demands to characterize the benefits of our combined server network selection policy in terms of energy consumption and job latencies. We found that our approach provides 25-80\% reduction in energy consumption compared to the case of optimizing server and network separately with conventional techniques.

 important goals and overall contributions of our work are:
\begin{itemize}
	\item We conceptualize the architectural sleep states for the switch, based on functional
	components and architectural design of real world data center switches. We
	motivate the benefit of such sleep states to the overall system power efficiency.
	\item We propose a new algorithm that considers servers and networks energy
	characteristics to coordinate server task placement while considering the power
	drawn by network components. Transition between power states in switches is
	controlled by buffer sizes and traffic patterns.
	\item We evaluate the impact of having the low-power states in the switch
	and our policy which optimizes for lower energy consumption in our data-center
	simulator. We consider a FatTree data center topology with various configuration parameters
	such as network traffic sizes, CPU traces, server and network performance
	models.
\end{itemize}
%



==> 2020-popcorns-T-SUSC (copy)/RelatedWork.tex <==
\section{Related Work}
\label{sec:RelatedWork}
With the energy consumption of large data centers reaching Gigawatt scale, its energy saving techniques are increasingly being studied in recent years. % and can be broadly classified into 1) Energy reductions for servers. 2) Energy reduction for the network components 3) Combined server, network power efficiency strategies.
Common techniques used for server energy reduction include Dynamic voltage and
frequency scaling (DVFS) to reduce the energy at the cost of server performance
%\cite{2013WangEnergyawareParallelTask}
 ,Co-ordinated DVFS and sleep states for
server processors \cite{yaoTSBatProImprovingEnergy2018} \cite{yaoWASPWorkloadAdaptive2017}, and
virtualization to consolidate VMs into fewer servers
\cite{hsuOptimizingEnergyConsumption2014}.  TS-Bat ~\cite{yaoTSBatProImprovingEnergy2018}
demonstrates that, through temporally batching the jobs and by grouping them
onto specific servers spatially, higher power savings can be obtained.
WASP~\cite{yaoWASPWorkloadAdaptive2017} shows that intelligent use of low power states in
servers can be used to boost server power savings.
%But network energy consumption still accounts for 25\% of the total data center power consumption \cite{KoutitasChallengesenergyefficiency}.

For the energy efficiency in network, earlier works have looked at switches and
routers for Internet-scale large area networking. Gupta et
al.~\cite{guptaGreeningInternet2003} first proposed the need for power saving in
networks and pointed to having network protocol support for energy management.
Adaptive Link Rate (ALR) \cite{gunaratneReducingEnergyConsumption2008} reduces
link energy consumption by dynamically adjusting data link rate depending on
traffic requirements. Other approaches include turning off switches when not
required, or to put them in sleep mode depending on packet queue length
\cite{yuEnergyefficientDelayawarepacket2015}
%\cite{2012Sidistributedenergysaving}.
 Prior work on reducing data center network
power rely on DVFS and sleep states \cite{iqbalEfficienttrafficaware2012} to
opportunistically reduce power consumption of individual switches. In these
approaches, switches may enter sleep states without knowledge of incoming server
traffic and may be forced to wake up prematurely. We study a co-ordinate server
job placement and network allocation required to optimize the amount of sleep
time and save network energy consumption.Recently,
DREAM~\cite{zhouDREAMDistRibutedEnergyAware2019} proposed a probability based
network traffic distribution scheme by splitting flows to save network power.


There are existing works which combine server and network power saving.
Mahadevan et al.\cite{mahadevanEnergyAwareNetwork2009} and Heller et al.
~\cite{hellerElasticTreeSavingEnergy2010} have proposed a heuristic based
algorithm for a coarse-grained load variation which dynamically allocates the
servers required for the workload and powers off the unneeded switches for the
server configuration. Other approaches consolidate VMs in fewer servers and in
turn fewer switches \cite{zhengJointpoweroptimization2014}. These approaches
assume an unrealistically high amount of idle period to offset the large wakeup
latencies to transition between On and Off states. To the best of our knowledge
our solution is the only one to consider network sleep states to target higher
power savings in the data center. The EEPRON~\cite{zhouJointServerNetwork2018}
discussed using the network slack available to reduce the energy consumption of
servers with frequency scaling.
%(pro: bin packing, Con: ECMP in Data) CARPO (Con: Long term flow based scheduling), Adnan and Rajesh Gupta 

%The combined energy efficiency management of network and servers are considered to give more savings than individual power management strategies.(Cite Mahadevan). (Joint VM consolidation based work)





==> 2020-popcorns-T-SUSC (copy)/ack.tex <==
\section*{Acknowledgment}

\label{ack}
This material is based upon work supported in part by the National Science Foundation 
under CAREER Award CCF-1149557 and CNS-1320226.

==> 2020-popcorns-T-SUSC (copy)/acknowledgement.tex <==
\section*{Acknowledgment}
\label{sec:acknowledgement}
This material is based in part upon work supported by the National Science Foundation under Grant Number CNS-178133. Kathy Nguyen and Gregory Kahl were supported through a REU supplement under the NSF award.
%Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation.


==> 2020-popcorns-T-SUSC (copy)/algorithms.tex <==
\subsection{Estimating the energy consumption}
\label{sec:algorithms}
Modeling this joint power optimization problem in Datacenter Networks (DCN) as an Integer Linear Programming (ILP) formulation is a solution, and optimization tools like MathProg can be used to provide a near-optimal result. However, the computation complexity increases exponentially with the number of servers and switches~\cite{wangExpeditusCongestionAwareLoad2017}. In a typical data center with tens of thousands of servers and hundreds of switches, it is computationally prohibitive to solve the optimization problem. We therefore propose a computationally-efficient heuristic algorithm in this section.

\input{motivation}
%\todo {Attempt ILP formulation}
\begin{comment}
In this section, we first present an Integer Linear Programming (ILP) formulation for the joint optimization problem in details. We then propose heuristic algorithms for solving the optimization problem efficiently.
%We then propose two heuristics for the static case, and later adapt them to the dynamic case.

\subsection{ILP formulation}
In the ILP formulation, the input parameters are shown in Table~\ref{table2:notation}.

\begin{table}
	%\centering
	\caption{\label{table2:notation} Notations in ILP formulation}
	\scalebox{0.5}{
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Meaning} \\ 
		\hline
		$v$ & an arbitrary network node  \\
		\hline
		$s$ & an arbitrary server  \\
		\hline
		$V$ & set of network nodes (e.g. servers, switches)  \\
		\hline
		$S$ & set of servers  \\
		\hline
		$j$ & an arbitrary job  \\
		\hline
		$L$ & set of links in the network  \\
		\hline
		$P_{m,n}^{linecard}$ & power consumption of line card $m$ in switch $n$ \\
		\hline
		$P_{n}^{base}$ & power consumption of all parts other than line cards in switch $n$ \\
		\hline
		$N^{switch}$ & number of switches  \\
		\hline
		$P_{c,s}^{core}$ & power consumption of core $c$ in server $s$ \\
		\hline
		$P_{s}^{base}$ & power consumption of all parts other than cores in server $s$ \\
		\hline
		$N_{s}^{core}$ & number of cores in server $s$  \\
		\hline
		$N^{server}$ & number of servers  \\
		\hline
		$T^{j}$ & set of tasks in job $j$  \\
		\hline
		$t^{j}$ & an arbitrary task in job $j$, $t^{j}\in{T^{j}}$  \\
		\hline
		$N^{job}$ & number of jobs  \\
		\hline
		$B_{r,t}^{j}$ & bandwidth requirement between task $r$ and task $t$ of job $j$, task $r$ is in server $s_r$, task $t$ is in server $s_t$  \\
		\hline
		$l_{n_1,n_2}$ & link between node $n_1$ and $n_2$, $l_{n_1,n_2}$ $\in$ L  \\
		\hline
		$C_{l_{n_1,n_2}}$ & capacity of link $l_{n_1,n_2}$  \\
		\hline
		$L_{m, n}$ & set of links connected to line card $m$ in switch $n$  \\
		\hline
		$f_{l_{n_1,n_2}}$ & number of flows on link $l_{n_1,n_2}$ \\
		\hline
		$l_{p,s_1,q,s_2}$ & link between line card p in switch $s_1$ and line card q in switch $s_2$ $s$ to node $d$ \\
		\hline
		$l_{s,d}$ & an arbitrary path from node $s$ to node $d$ \\
		\hline
		$f_{l_{n_1,n_2}}$ & set of flows on link $l_{n_1,n_2}$ \\
		\hline
		$d^{l_{n_1,n_2}}_f$ & data rate of flow $f$ on link $l_{n_1,n_2}$ \\
		\hline
	\end{tabular}}
\end{table}

\begin{center}
	\scalebox{0.8}{
	Objective: ${Minimize(P^{switches}+P^{servers})}$}
	\scalebox{0.8}{
	$=\min{\sum_{n=1}^{N^{switch}}(P^{base}_n+\sum_{m=1}^{N_n^{linecard}}P_{m,n}^{linecard}x_m^n) +\sum_{s=1}^{N^{server}}(P_s^{base}+\sum_{c=1}^{N_s^{core}}P_{c,s}^{core}z_c^s)}$}
		
		%\sum_{k=1}^{H}(\left\lceil \frac{w_i^j}{k} \right\rceil-1)a^j_{i, v, k}}$}

\end{center}

Decision Variables:

a)
\begin{equation*}
a^{j}_{t, c, s}=
\begin{cases}
1, \quad\makebox{if task } t \makebox{ of job } j \makebox{ is assigned to core } c \makebox{ in server }  s  \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

b)

\begin{equation*}
z^{j}_{t, r, s}=
\begin{cases}
1, \quad\makebox{if task } t \makebox{ and } r \makebox{ of job } j \makebox{ are assigned to server }  s  \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

c)
\begin{equation*}
y^{s}_{c}=
\begin{cases}
1, \quad\makebox{if core } c \makebox{ in server } s \makebox{ is operating; } \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

d)
\begin{equation*}
x^{n}_{m}=
\begin{cases}
1, \quad\makebox{if line card } m \makebox{ in switch } n \makebox{ is active; } \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

d)
\begin{equation*}
\lambda^{l}_{p_{s,d}}=
\begin{cases}
1, \quad\makebox{if link } l \makebox{ is on path } p_{s,d} \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

Constraints:

a) Each task of each job can be assigned to only one core. For all $j, t$
\begin{equation*}
\sum_{s=1}^{N^{server}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}

b) The number of tasks being executed on a server cannot exceed the number of its cores. For all $s$
\begin{equation*}
\sum_{j=1}^{N^{job}} \sum_{t\in{T^j}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}

c) Constraints to find the value of $z^{j}_{t, r, s}$. For all $j, t, r, s$
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \leq 1 + z^{j}_{t, r, s}
\end{equation*}
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \geq 2z^{j}_{t, r, s}
\end{equation*}

d) If link $l_{n_1,n_2}$ is on path $p_{s,d}$, there must exist another link from node $n_1, n_2$ respectively on this path.
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \leq 1 + z^{j}_{t, r, s}
\end{equation*}
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \geq 2z^{j}_{t, r, s}
\end{equation*}

e) If link $l_{s_1,s_2}$ is on the task communication path $p_{s,d}$, then the corresponding line cards in $s_1$ and $s_2$ must be active and the link between them is also on $p_{s,d}$. For $l_{p,s_1,q,s_2}$ $\in$ $L_{p,s_1}$, $l_{p,s_1,q,s_2}$ $\in$ $L_{q,s_2}$
\begin{equation*}
\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} = \lambda^{l_{s_1,s_2}}_{p_{s,d}} = x^{s_1}_{p} = x^{s_2}_{q}
\end{equation*}
\begin{equation*}
x^{s_1}_{p}\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} \geq \lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}}
\end{equation*}
\begin{equation*}
x^{s_2}_{q}\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} \geq \lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}}
\end{equation*}

f) Line card $m$ in switch $n$ is off only when all the links connected to it are not on any path.
\begin{equation*}
\left| L_{m,n} \right| x^{n}_{m} \geq \sum_{l\in{L_{m,n}}}\lambda^{l}_{p_{s,d}}
\end{equation*}

g) Total flow rate on a link cannot exceed the link capacity.
\begin{equation*}
\sum_{f\in{f_{l_{n_1,n_2}}}}^{N^{server}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}
\end{comment}

\subsection{Heuristic Algorithms}
In this section, we first present a power management algorithm for the transition of line card and port power state, a simple power transition algorithm for servers, and then propose joint job placement and network routing algorithm for solving the optimization problem efficiently.

%It is computationally prohibitive and NP-hrad to solve the ILP problem above and get the optimal solution for large-scale cases. We therefore propose two computation-efficient heuristic algorithms in this section. The main idea of our algorithm is to jointly consider the status of server pool and network before assigning jobs.

\subsubsection{Power State Transition Algorithm}

%{remove the port Low Power Idle (LPI) transition from the algorithm (save very little power), add more line card power states, the transition algorithm to control the transition}



As not all switches in DCN need to be active all the time, if we can intelligently control the transition of active and low power state for ports and line cards, then data center network power consumption could be saved. Therefore, we propose the Power State Transition Algorithm~\ref{algorithm1} to implement network power management. The notations are elaborated in Table~\ref{algorithm1table}. We assume that there is a global controller that keeps record of all the line cards, ports, and server status, including their power state, queue size, etc. The global controller monitors the current traffic load (number of pending flows or packets) at each port and decides whether the current line card power state should change. It then decides if the port state should change as a feedback. In our design, we couple the line card and port power state and their transition: if a line card is in sleep or off state, then all the ports are also in LPI or off state; if a line card is active, then its ports can be in LPI or active state, and LPI ports can be woken up to become active in a short time. %~\ref{algorithm1} describes our proposed design in details.


%\begin{figure}
%	\captionsetup{font=small}
%	\centering\includegraphics[width=0.5\textwidth]{figures/Presentation2.pdf}
%	\caption{Power state transition overview.}
%	\label{figure3}
%\end{figure}


\begin{algorithm}
	\SetAlgoNoLine
	\scriptsize
	\caption{Power State Transition Algorithm}
	\label{algorithm1}
	\KwIn{$T_s$, $T_a$, $Q_{iL}$}
	\KwOut{Line card and port state transition}
	Initialization: All line cards are in sleep state, all ports are in LPI state\;
	
	\While{there are jobs to be executed}
	{
		\If{a flow arrives at port $i$ of line card $L$ at time $t$}
		{
			\If{$L$ is in sleep state} {
				\If{$Q_{iL} > T_s$} {
					$L$ begins waking up from sleep state\;
					$i$ begins waking up from LPI state\;
				} 
				\Else
				{
					$L$ begins waking up after $\tau_{wakeup}^{LC}$\;
					$i$ begins waking up after $\tau_{wakeup}^{port}$\;
				}
				
			} 
		}
		\If{a flow is transimitted from port $i$ of line card $L$ at time $t$} {
			\If{$Q_{iL} < T_s$} {
				$i$ starts transition to LPI after $\tau_{LPI}$\;
				\If{after $\tau_{LPI}$, all the ports of $L$ are in LPI state} {
					$L$ starts transition to deeper sleep state after $\tau_{sleep}^{LC}$;
				}
			}
		}
	}
	
\end{algorithm}

%\subsubsection{Server State Transition Algorithm}
%
%As mentioned in Section~\ref{sec:serverpower}, we model two power states for the server: active and C6 sleep state. Algorithm~\ref{algorithm4} describes our policy on managing the server power states. We assume that each server in DCN has a local queue to buffer the tasks, and tasks should first be dispatched to active servers whose queue size do not exceed a threshold. The threshold controls the job latency.
%
%\begin{algorithm}
%	\SetAlgoNoLine
%	\small
%	\caption{Server State Transition Algorithm}
%	\label{algorithm4}
%	\KwIn{ server wakeup latency $\tau_{wakeup}^{server}$, local queue of server $S$}
%	\KwOut{Server power state transition}
%	
%		\If{a task arrives at a server $S$}
%		{
%			\If{$S$ is in sleep state} {
%				$S$ begins waking up after wakeup latency $\tau_{wakeup}^{server}$\;
%			} 
%		   \Else {
%		   		task is put in the local queue of $S$\;
%	   		}
%		}
%		\If{a task is finished executing at a server $S$}
%		{
%			\If{local queue of $S$ is empty} {
%				$S$ begins turning into sleep state\;
%			} 
%		}
%	
%	
%\end{algorithm}

\subsubsection{\PopCorns-Cooperative Network-Server Algorithm}

%{\bf GV- Should the title be Popcorns-Pro?{\color{green} Changed}}
{

The main idea of our algorithm is to jointly consider the status of server pool and network before assigning jobs. To be more specific, for a job consisting of several pairs of interdependent tasks, if we place task pairs based on their interdependence, and choose the core pair with the minimum routing cost, instead of randomly placing them on available cores without awareness of communication requirement between tasks, then the placement together with its corresponding routing path must be the optimal. And in the context of this paper, network routing cost is energy consumption, since every line card on the chosen routing path has to be active, or it will have to be woken up.

Based on this idea, we propose the Cooperative Network-Server (CNS) Algorithm~\ref{algorithm2} %{\bf GV- check the algorithm reference}.
The notations are elaborated in Table~\ref{algorithm1table}. In the initial stage, we compute and store all possible routing paths between any pair of network nodes. As mentioned in the previous section, we have a global controller to keep track of all the line cards, ports, and server statuses. Thus, when a job consisting of a set of interdependent tasks arrive, we first check the server side to select all server pairs whose power state is active and local queue sizes do not exceed a threshold. If no server statisfies these requirements, then servers with full local queue and servers in C6 sleep state will be selected. Note that if a task is assigned to a server in sleep state, then the server will be activated immediately and enter active state after a wakeup latency. For each server pair we select possible routing paths between them from the pre-computed routing paths set. Along each path, line cards could be active, sleeping, or off, and ports could be active, LPI, or off, but if we assign a path to the task pair, all the line cards and ports along it should become active. In other words, we need to wake up the inactive line cards and ports on the chosen path, which results in extra power consumption and wakeup latency. Based on this, we can compute and assign a weight, which is a measurement of the number of active line cards and ports, to each possible routing path, and choose the server pair with minimum routing cost. And our proposed Cooperative Network-Server Algorithm will output the least-weight path and its corresponding server pair for each task pair.}

\begin{table}
	\centering
	\captionsetup{font=small}
		\scalebox{0.7}{
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Description} \\ 
		\hline
		$P$ & all the routing paths between any pair of network nodes  \\
		\hline
		$Q_s$ & local queue size of server $s$  \\
		\hline
		$T_s^{server}$ & local queue size threshold of server $s$\\
		\hline
		$S$ & all the servers in DCN  \\
		\hline
		$S_{ava}$ & all the servers whose current queue size doesn't exceed $T_s^{server}$  \\
		\hline
		$P_{x, y}$ & all the routing paths between node $x$ and $y$ in DCN\\
		\hline
			$T_s$ & traffic threshold for port waking up  \\
		\hline
		$T_a$ & traffic threshold for port turning into LPI state  \\
		\hline
		$Q_{iL}$& current traffic load at port $i$ in line card $L$  \\
		\hline
		$\tau_{wakeup}^{port}$ & port wakeup delay  \\
		\hline
		$\tau_{wakeup}^{LC}$ & line card wakeup delay  \\
		\hline
		$\tau_{LPI}^{port}$ & port turning into LPI state delay \\
		\hline
		$\tau_{sleep}^{LC}$ & line card turning into sleep state delay \\
		\hline	
	\end{tabular}
}
	\caption{\label{algorithm1table} Notations in \PopCorns Cooperative Network-Server Algorithm.}
\end{table}

\begin{algorithm}[!htb]
	\SetAlgoNoLine
	\scriptsize
	\caption{\PopCorns  - Cooperative Network-Server Algorithm}
	\label{algorithm2}
	\KwIn{$P$, $Q_s$, $T_s$, line cards and ports power state, task dependency within a job}
	\KwOut{Job placement and corresponding routing path}
	
	\While{job $j$ consisting of task set $T^j$ arrives}
	{
		\For{each pair of interdependent tasks $(T^j_m, T^j_n)$ in $T^j$}
		{
			select $S_{ava}$ from $S$\;
			\For {each pair of available servers $(x, y)$ in $S_{ava}$}
			{
				compute $P(x, y)$ for server pair $(x, y)$ from $P$\;
				\For {each path $p$ in $P(x, y)$}
				{
					get power states of all the ports and line cards along $P$ from the global controller, compute path weight $w(x, y)$ in terms of energy consumption\;
				}
			}
			choose the least-weight path associated with corresponding server pair for task pair $(T^j_m, T^j_n)$\;
		}
	}
\end{algorithm}


\begin{algorithm}
	\SetAlgoNoLine
	\scriptsize
	\caption{\PopCorns - Weight assignment algorithm between two nodes}
	\label{algorithm3}
	\KwIn{$Link(i,j)$, $QoS$, $Link_{Capacity}$}
	\KwOut{$W(i,j)$ Weight for the edge connecting nodes i and j} 
	
	
	
	\If{ Node $i$ is Server} {
		 $LinkWeight(i,j) += (ServerActivePower - CurrentSleepStatePower) *( taskSize + EdgeLinkBW / FlowSize)$;
	 }
	\If{ Node $j$ is a Switch} 
	{
		$LinkCapacity_{remaining} \leftarrow Link_{fullCapacity}$;
		
		\For {$Every Flow F_{i}  on  Link(i,j)$ }
			{
				$Flow_{i_{remainingTime}} \leftarrow  FSize_{i_{Remaining}} / FcurBW_{i}$;
				
				 
				\If {$F_{i_{remainingTime}} > SlowestTime$ } 
					{
					 $SlowestTime \leftarrow  F_{i_{remainingTime}}$;
					 
					 $SlowestFlow \leftarrow F_{i}$;
					 
					}
				$LinkCapacity_{remaining} -= FcurBW_{i}$
			}
		$availBW \leftarrow min(Link_{fullCapacity} - LinkCapacity_{remaining} \text{ and } EdgeLinkBW)$;
		
		\If { $availBW > MinBWforQoS$ }
		{ 
			$timeForNewFlow \leftarrow availBW/ FSize_{newFlow}$;
			
			$additionalTimeAwake \leftarrow MAX(SlowestTime \text{ and } timeForNewFlow  )$;
			
			$LinkWeight(i,j) += additionalTimeAwake * ActivePower_{j}$;
		} \Else {
			$FcurBW_{newFlow} \leftarrow FSize_{newFlow}/QoSRequiredTime$;
			
			$FcurBW_{Slowest}' \leftarrow (FcurBW_{Slowest} - (availBW - (FcurBW_{newFLow}/NumFlowsOnLink))$;
		
			$AdditionalTime_{SlowestFlow} \leftarrow       (FcurBW_{Slowest} - FcurBW_{Slowest}')/ FlowDataremaing_{Slowest}$;
			
			$timeForNewFlow \leftarrow QoSRequiredTime$
			
			$additionalTimeAwake \leftarrow MAX(timeForNewFlow \text{ and } AdditionalTime_{SlowestFlow})$;
			
			$LinkWeight(i,j) += additionalTimeAwake * ActivePower_{j}$;
		 
		}
	}
\end{algorithm}


\begin{algorithm}
	\SetAlgoNoLine
	\caption{Job scheduling Algorithm}
	\label{algorithm2}
	\scriptsize
	\KwIn{$P$, $Q_s$, $T_s$, line cards and ports power state, task dependency within a job}
	\KwOut{Job placement and corresponding routing path}

	\While{job $j$ consisting of task set $T^j$ arrives}
	{
		\For{each pair of interdependent tasks $(T^j_m, T^j_n)$ in $T^j$}
		{
			select $S_{ava}$ from $S$\;
			\For {each pair of available servers $(x, y)$ in $S_{ava}$}
			{
				compute $P(x, y)$ for server pair $(x, y)$ from $P$\;
				\For {each path $p$ in $P(x, y)$}
				{
					get power states of all the ports and line cards along $P$ from the global controller, compute path weight $w(x, y)$ in terms of energy consumption\;
				}
			}
			choose the least-weight path associated with corresponding server pair for task pair $(T^j_m, T^j_n)$\;
		}
	}
\end{algorithm}

%\subsection{Scalability of the Popcorns++ Algorithm}
\todo{TBD}

% \begin{figure}
%   \captionsetup{font=small}
%   \centering\includegraphics[width=0.6\textwidth]{figures/scalability/chart.pdf}
%   \caption{Computation overhead }  \label{figure3}
% \end{figure}


==> 2020-popcorns-T-SUSC (copy)/algorithms__Santosh_Dayapule_s_conflicted_copy_2019-08-08_.tex <==
\section{Solution Approach}
\label{sec:algorithms}
Modeling this joint power optimization problem in DCN as an Integer Linear Programming (ILP) formulation is a solution, and optimization tools like MathProg can be used to provide a near-optimal result. However, the computation complexity increases exponentially with the number of servers and switches~\cite{wang2012carpo}. In a typical data center with tens of thousands of servers and hundreds of switches, it is computationally prohibitive to solve the optimization problem. We therefore propose a computationally-efficient heuristic algorithm in this section. 

\begin{comment}
In this section, we first present an Integer Linear Programming (ILP) formulation for the joint optimization problem in details. We then propose heuristic algorithms for solving the optimization problem efficiently.
%We then propose two heuristics for the static case, and later adapt them to the dynamic case.

\subsection{ILP formulation}
In the ILP formulation, the input parameters are shown in Table~\ref{table2:notation} .

\begin{table}
	%\centering
	\caption{\label{table2:notation} Notations in ILP formulation}
	\scalebox{0.5}{
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Meaning} \\ 
		\hline
		$v$ & an arbitrary network node  \\
		\hline
		$s$ & an arbitrary server  \\
		\hline
		$V$ & set of network nodes (e.g. servers, switches)  \\
		\hline
		$S$ & set of servers  \\
		\hline
		$j$ & an arbitrary job  \\
		\hline
		$L$ & set of links in the network  \\
		\hline
		$P_{m,n}^{linecard}$ & power consumption of line card $m$ in switch $n$ \\
		\hline
		$P_{n}^{base}$ & power consumption of all parts other than line cards in switch $n$ \\
		\hline
		$N^{switch}$ & number of switches  \\
		\hline
		$P_{c,s}^{core}$ & power consumption of core $c$ in server $s$ \\
		\hline
		$P_{s}^{base}$ & power consumption of all parts other than cores in server $s$ \\
		\hline
		$N_{s}^{core}$ & number of cores in server $s$  \\
		\hline
		$N^{server}$ & number of servers  \\
		\hline
		$T^{j}$ & set of tasks in job $j$  \\
		\hline
		$t^{j}$ & an arbitrary task in job $j$, $t^{j}\in{T^{j}}$  \\
		\hline
		$N^{job}$ & number of jobs  \\
		\hline
		$B_{r,t}^{j}$ & bandwidth requirement between task $r$ and task $t$ of job $j$, task $r$ is in server $s_r$, task $t$ is in server $s_t$  \\
		\hline
		$l_{n_1,n_2}$ & link between node $n_1$ and $n_2$, $l_{n_1,n_2}$ $\in$ L  \\
		\hline
		$C_{l_{n_1,n_2}}$ & capacity of link $l_{n_1,n_2}$  \\
		\hline
		$L_{m, n}$ & set of links connected to line card $m$ in switch $n$  \\
		\hline
		$f_{l_{n_1,n_2}}$ & number of flows on link $l_{n_1,n_2}$ \\
		\hline
		$l_{p,s_1,q,s_2}$ & link between line card p in switch $s_1$ and line card q in switch $s_2$ $s$ to node $d$ \\
		\hline
		$l_{s,d}$ & an arbitrary path from node $s$ to node $d$ \\
		\hline
		$f_{l_{n_1,n_2}}$ & set of flows on link $l_{n_1,n_2}$ \\
		\hline
		$d^{l_{n_1,n_2}}_f$ & data rate of flow $f$ on link $l_{n_1,n_2}$ \\
		\hline
	\end{tabular}}
\end{table}

\begin{center}
	\scalebox{0.8}{
	Objective: ${Minimize(P^{switches}+P^{servers})}$}
	\scalebox{0.8}{
	$=\min{\sum_{n=1}^{N^{switch}}(P^{base}_n+\sum_{m=1}^{N_n^{linecard}}P_{m,n}^{linecard}x_m^n) +\sum_{s=1}^{N^{server}}(P_s^{base}+\sum_{c=1}^{N_s^{core}}P_{c,s}^{core}z_c^s)}$}
		
		%\sum_{k=1}^{H}(\left\lceil \frac{w_i^j}{k} \right\rceil-1)a^j_{i, v, k}}$}

\end{center}

Decision Variables:

a)
\begin{equation*}
a^{j}_{t, c, s}=
\begin{cases}
1, \quad\makebox{if task } t \makebox{ of job } j \makebox{ is assigned to core } c \makebox{ in server }  s  \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

b)

\begin{equation*}
z^{j}_{t, r, s}=
\begin{cases}
1, \quad\makebox{if task } t \makebox{ and } r \makebox{ of job } j \makebox{ are assigned to server }  s  \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

c)
\begin{equation*}
y^{s}_{c}=
\begin{cases}
1, \quad\makebox{if core } c \makebox{ in server } s \makebox{ is operating; } \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

d)
\begin{equation*}
x^{n}_{m}=
\begin{cases}
1, \quad\makebox{if line card } m \makebox{ in switch } n \makebox{ is active; } \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

d)
\begin{equation*}
\lambda^{l}_{p_{s,d}}=
\begin{cases}
1, \quad\makebox{if link } l \makebox{ is on path } p_{s,d} \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

Constraints:

a) Each task of each job can be assigned to only one core. For all $j, t$
\begin{equation*}
\sum_{s=1}^{N^{server}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}

b) The number of tasks being executed on a server cannot exceed the number of its cores. For all $s$
\begin{equation*}
\sum_{j=1}^{N^{job}} \sum_{t\in{T^j}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}

c) Constraints to find the value of $z^{j}_{t, r, s}$. For all $j, t, r, s$
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \leq 1 + z^{j}_{t, r, s}
\end{equation*}
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \geq 2z^{j}_{t, r, s}
\end{equation*}

d) If link $l_{n_1,n_2}$ is on path $p_{s,d}$, there must exist another link from node $n_1, n_2$ respectively on this path.
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \leq 1 + z^{j}_{t, r, s}
\end{equation*}
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \geq 2z^{j}_{t, r, s}
\end{equation*}

e) If link $l_{s_1,s_2}$ is on the task communication path $p_{s,d}$, then the corresponding line cards in $s_1$ and $s_2$ must be active and the link between them is also on $p_{s,d}$. For $l_{p,s_1,q,s_2}$ $\in$ $L_{p,s_1}$, $l_{p,s_1,q,s_2}$ $\in$ $L_{q,s_2}$
\begin{equation*}
\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} = \lambda^{l_{s_1,s_2}}_{p_{s,d}} = x^{s_1}_{p} = x^{s_2}_{q}
\end{equation*}
\begin{equation*}
x^{s_1}_{p}\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} \geq \lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}}
\end{equation*}
\begin{equation*}
x^{s_2}_{q}\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} \geq \lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}}
\end{equation*}

f) Line card $m$ in switch $n$ is off only when all the links connected to it are not on any path.
\begin{equation*}
\left| L_{m,n} \right| x^{n}_{m} \geq \sum_{l\in{L_{m,n}}}\lambda^{l}_{p_{s,d}}
\end{equation*}

g) Total flow rate on a link cannot exceed the link capacity.
\begin{equation*}
\sum_{f\in{f_{l_{n_1,n_2}}}}^{N^{server}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}
\end{comment}

\subsection{Heuristic Algorithms}
In this section, we first present a power management algorithm for the transition of line card and port power state, a simple power transition algorithm for servers, and then propose joint job placement and network routing algorithm for solving the optimization problem efficiently.

%It is computationally prohibitive and NP-hrad to solve the ILP problem above and get the optimal solution for large-scale cases. We therefore propose two computation-efficient heuristic algorithms in this section. The main idea of our algorithm is to jointly consider the status of server pool and network before assigning jobs.

\subsubsection{Power State Transition Algorithm}

{\color{blue}remove the port Low Power Idle (LPI) transition from the algorithm (save very little power), add more line card power states, the transition algorithm to control the transition}

\begin{table}
	\centering
	\captionsetup{font=small}
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Description} \\ 
		\hline
		$T_s$ & traffic threshold for port waking up  \\
		\hline
		$T_a$ & traffic threshold for port turning into LPI state  \\
		\hline
		$Q_{iL}$& current traffic load at port $i$ in line card $L$  \\
		\hline
		$\tau_{wakeup}^{port}$ & port wakeup delay  \\
		\hline
		$\tau_{wakeup}^{LC}$ & line card wakeup delay  \\
		\hline
		$\tau_{LPI}^{port}$ & port turning into LPI state delay \\
		\hline
		$\tau_{sleep}^{LC}$ & line card turning into sleep state delay \\
		\hline	
	\end{tabular}
	\caption{\label{algorithm1table} Notations in PopCorns power state transition algorithm.}
\end{table}

As not all switches in DCN need to be active all the time, if we can intelligently control the transition of active and low power state for ports and line cards, then data center network power consumption could be saved. Therefore, we propose the Power State Transition Algorithm~\ref{algorithm1} to implement network power management. The notations are elaborated in Table~\ref{algorithm1table}. An overview of our approach is shown in Figure~\ref{figure3}. We assume that there is a global controller that keeps record of all the line cards, ports, and server status, including their power state, queue size, etc. The global controller monitors the current traffic load (number of pending flows or packets) at each port and decides whether the current line card power state should change. It then decides if the port state should change as a feedback. In our design, we couple the line card and port power state and their transition: if a line card is in sleep or off state, then all the ports are also in LPI or off state; if a line card is active, then its ports can be in LPI or active state, and LPI ports can be woken up to become active in a short time. %~\ref{algorithm1} describes our proposed design in details.


\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.5\textwidth]{figures/Presentation2.pdf}
	\caption{Power state transition overview.}
	\label{figure3}
\end{figure}


\begin{algorithm}
	\SetAlgoNoLine
	\caption{Power State Transition Algorithm}
	\label{algorithm1}
	\KwIn{$T_s$, $T_a$, $Q_{iL}$}
	\KwOut{Line card and port state transition}
	Initialization: All line cards are in sleep state, all ports are in LPI state\;
	
	\While{there are jobs to be executed}
	{
		\If{a flow arrives at port $i$ of line card $L$ at time $t$}
		{
			\If{$L$ is in sleep state} {
				\If{$Q_{iL} > T_s$} {
					$L$ begins waking up from sleep state\;
					$i$ begins waking up from LPI state\;
				} 
				\Else
				{
					$L$ begins waking up after $\tau_{wakeup}^{LC}$\;
					$i$ begins waking up after $\tau_{wakeup}^{port}$\;
				}
				
			} 
		}
		\If{a flow is transimitted from port $i$ of line card $L$ at time $t$} {
			\If{$Q_{iL} < T_s$} {
				$i$ starts transition to LPI after $\tau_{LPI}$\;
				\If{after $\tau_{LPI}$, all the ports of $L$ are in LPI state} {
					$L$ starts transition to sleep state after $\tau_{sleep}^{LC}$;
				}
			}
		}
	}
	
\end{algorithm}

\subsubsection{Server State Transition Algorithm}

{\color{blue}multi-core servers, multiple power states}

As mentioned in Section~\ref{sec:serverpower}, we simply model two power states for the server: active and C6 sleep state. Algorithm~\ref{algorithm4} describes our policy on managing the server power states. We assume that each server in DCN has a local queue to buffer the tasks, and tasks should first be dispatched to active servers whose queue size do not exceed a threshold. The threshold controls the job latency.

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Server State Transition Algorithm}
	\label{algorithm4}
	\KwIn{ server wakeup latency $\tau_{wakeup}^{server}$, local queue of server $S$}
	\KwOut{Server power state transition}
	
		\If{a task arrives at a server $S$}
		{
			\If{$S$ is in sleep state} {
				$S$ begins waking up after wakeup latency $\tau_{wakeup}^{server}$\;
			} 
		   \Else {
		   		task is put in the local queue of $S$\;
	   		}
		}
		\If{a task is finished executing at a server $S$}
		{
			\If{local queue of $S$ is empty} {
				$S$ begins turning into sleep state\;
			} 
		}
	
	
\end{algorithm}

\subsubsection{Cooperative Network-Server Algorithm}

{\color{blue}periodical global control/computation, traffic prediction like TS-Bat}

The main idea of our algorithm is to jointly consider the status of server pool and network before assigning jobs. To be more specific, for a job consisting of several pairs of interdependent tasks, if we place task pairs based on their interdependence, and choose the core pair with the minimum routing cost, instead of randomly placing them on available cores without awareness of communication requirement between tasks, then the placement together with its corresponding routing path must be the optimal. And in the context of this paper, network routing cost is energy consumption, since every line card on the chosen routing path has to be active, or it will have to be woken up.

Based on this idea, we propose the Cooperative Network-Server (CNS) Algorithm~\ref{algorithm2}. The notations are elaborated in Table~\ref{algorithm2table}. In the initial stage, we compute and store all possible routing paths between any pair of network nodes. As mentioned in the previous section, we have a global controller to keep track of all the line cards, ports, and server statuses. Thus, when a job consisting of a set of interdependent tasks arrive, we first check the server side to select all server pairs whose power state is active and local queue sizes do not exceed a threshold. If no server statisfies these requirements, then servers with full local queue and servers in C6 sleep state will be selected. Note that if a task is assigned to a server in sleep state, then the server will be awoken immediately and enter active state after a wakeup latency. For each server pair we select possible routing paths between them from the pre-computed routing paths set. Along each path, line cards could be active, sleeping, or off, and ports could be active, LPI, or off, but if we assign a path to the task pair, all the line cards and ports along it should become active. In other words, we need to wake up the inactive line cards and ports on the chosen path, which results in extra power consumption and wakeup latency. Based on this, we can compute and assign a weight, which is a measurement of the number of active line cards and ports, to each possible routing path, and choose the server pair with minimum routing cost. And our proposed Cooperative Network-Server Algorithm will output the least-weight path and its corresponding server pair for each task pair.

\begin{table}
	\centering
	\captionsetup{font=small}
		\scalebox{0.7}{
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Description} \\ 
		\hline
		$P$ & all the routing paths between any pair of network nodes  \\
		\hline
		$Q_s$ & local queue size of server $s$  \\
		\hline
		$T_s^{server}$ & local queue size threshold of server $s$\\
		\hline
		$S$ & all the servers in DCN  \\
		\hline
		$S_{ava}$ & all the servers whose current queue size doesn't exceed $T_s^{server}$  \\
		\hline
		$P_{x, y}$ & all the routing paths between node $x$ and $y$ in DCN\\
		\hline
	\end{tabular}
}
	\caption{\label{algorithm2table} Notations in PopCorns Cooperative Network-Server Algorithm.}
\end{table}

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Cooperative Network-Server Algorithm}
	\label{algorithm2}
	\KwIn{$P$, $Q_s$, $T_s$, line cards and ports power state, task dependency within a job}
	\KwOut{Job placement and corresponding routing path}
	
	\While{job $j$ consisting of task set $T^j$ arrives}
	{
		\For{each pair of interdependent tasks $(T^j_m, T^j_n)$ in $T^j$}
		{
			select $S_{ava}$ from $S$\;
			\For {each pair of available servers $(x, y)$ in $S_{ava}$}
			{
				compute $P(x, y)$ for server pair $(x, y)$ from $P$\;
				\For {each path $p$ in $P(x, y)$}
				{
					get power states of all the ports and line cards along $P$ from the global controller, compute path weight $w(x, y)$ in terms of energy consumption\;
				}
			}
			choose the least-weight path associated with corresponding server pair for task pair $(T^j_m, T^j_n)$\;
		}
	}
\end{algorithm}

{\color{blue}
\begin*{algorithm}
	\SetAlgoNoLine
	\caption{Popcorns Weight assignment algorithm}
	\label{algorithm3}
	\KwIn{$i$, $j$, Server/line card power state, Number of flows on Link (i,j), LinkBandwidth, FlowSize, AverageNumberOfHops }
	\KwOut{$W(i,j)$ Weight for the edge connecting nodes i and j} 
	
	LinkWeight(i,j) \leftarrow 0;
	
	\If{$i$ is Server}
	{
		LinkWeight(i,j) + \leftarrow (ServerActivePower - Current Sleep state power) * taskSize + EdgeLinkBW /FlowSize;
	}
	\If{$j$ is a Switch} 
	{
		AvailableBandwidth = min(EdgeLinkBW,MaxLinkRate(i,j)/number_of_flows);
		
		LinkWeight (i,j)+ \leftarrow Switch $j$ ActivePower * FlowSize/EdgeLinkBW ;
		
		delayedTime \leftarrow  (FlowSize/(EdgeSwitchBW - AvailableBandwidth);
		LinkWeight (i,j) + \leftarrow  (Switch $j$ ActivePower + 2 * ServerActivePower) * delayTime / AverageHopCount;
	}
\end*{algorithm}
}

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Job scheduling Algorithm}
	\label{algorithm2}
	\KwIn{$P$, $Q_s$, $T_s$, line cards and ports power state, task dependency within a job}
	\KwOut{Job placement and corresponding routing path}

	\While{job $j$ consisting of task set $T^j$ arrives}
	{
		\For{each pair of interdependent tasks $(T^j_m, T^j_n)$ in $T^j$}
		{
			select $S_{ava}$ from $S$\;
			\For {each pair of available servers $(x, y)$ in $S_{ava}$}
			{
				compute $P(x, y)$ for server pair $(x, y)$ from $P$\;
				\For {each path $p$ in $P(x, y)$}
				{
					get power states of all the ports and line cards along $P$ from the global controller, compute path weight $w(x, y)$ in terms of energy consumption\;
				}
			}
			choose the least-weight path associated with corresponding server pair for task pair $(T^j_m, T^j_n)$\;
		}
	}
\end{algorithm}

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Job Scheduling Algorithm}
	\label{algorithm3}
	\KwIn{input}
	\KwOut{output}
	\If{there is job to be finished}{then-block}
	content...
\end{algorithm}

==> 2020-popcorns-T-SUSC (copy)/baselines.tex <==
%\section{Baseline policies}
\begin{figure*}
	\centering
	\captionsetup{font=small}
	\subfloat[Shortest Path and Random Server job scheduling]{
		\includegraphics[width=0.33\textwidth]{figures/heatmaps/heatmap_djikstra_user_specify_random_.png}
		\label{djikstra_heat_random}
	}
	\subfloat[Elastic Tree and Random Server job scheduling]{
		\includegraphics[width=0.33\textwidth]{figures/heatmaps/heatmap_elastic_tree_user_specify_random_.png}
		\label{elastic_tree_heat_random}
	}
	\subfloat[Shortest Path and WASP Server job scheduling]{
		\includegraphics[width=0.33\textwidth]{figures/heatmaps/heatmap_djikstra_user_specify_wasp_.png}
		\label{djikstra_heat_wasp}
	}
	
	\subfloat[Elastic Tree and WASP Server job scheduling]{
		\includegraphics[width=0.33\textwidth]{figures/heatmaps/heatmap_elastic_tree_user_specify_wasp_.png}
		\label{elastic_tree_heat_wasp}
	}
	\subfloat[Popcorns based server and network scheduling]{
		\includegraphics[width=0.33\textwidth]{figures/heatmaps/heatmap_popcorns_user_specify_popcorns_.png}
		\label{popcorns_heat_popcorns}
	}
	\caption{Illustration of the average sleep state for switches and server with
		different policies. \PopCorns scheduling policy achieves greater consolidation of server and network flows. }
	\label{fig:heatmap-graph}
\end{figure*}

Figure ~\ref{fig:heatmap-graph}, illustrates the heat map after the end of the execution of the same Poisson based random job arrival arrival pattern with mean arrival rate $\lambda$=0.5 Jobs/second using the different server and network job scheduling policies for a small 16 server Fat-Tree topology. We note that with random server selection , all servers are equally utilized with elastic tree based network scheduling performing more network consolidation for better savings.
When using random server selection for tasks with Shortest path routing ~\ref{djikstra_heat_random} and Elastic based  routing ~\ref{elastic_tree_heat_random}, we can see that there are more aggregate switches in the dark green allowing more switches to stay in deep sleep state. Similarly for the WASP server selection scheme in figures ~\ref{djikstra_heat_wasp} %{\bf GV-- wrong label?{\color{green} Changed}}
and ~\ref{elastic_tree_heat_wasp}, we see that there are unequal usage of the servers and more flows consolidated into fewer switches. It can be see that even with server energy optimization in WASP, and our combined server and network policy \PopCorns ~\ref{popcorns_heat_popcorns} %{\bf GV-- what is this? {\color{green} corrected }}
can achieve much higher savings than each of the individual optimizations. \PopCorns algorithm is able achieve this mainly due to being aware of network energy aware state when scheduling jobs on the servers. It is further able to reduce energy savings by increased consolidation of flows and servers by utilizing the latency slacks available at each node in the data center.

==> 2020-popcorns-T-SUSC (copy)/delaytimer_tstw.tex <==
\section{Workload Adaptation}
\label{sec:tstw_exp}
\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.3]{./figure/algorithm_chart.pdf}
	\caption{\titlename Power Management Framework}
	\label{fig:alg_overview}
\end{figure}
While delay timers are useful in saving energy, we note that they lack workload awareness. Large values of delay timers could cause the system to remain in higher power states for longer than necessary resulting in increased energy consumption, while too small values for delay timers result in premature entry into low-power states. This can be problematic on two counts: 
\begin{inparaenum}
\item The transition energy between power states can be high. 
\item The wakeup latencies from low-power states can degrade system performance.
\end{inparaenum} 

To incorporate workload-awareness, we explore a two-level adaptive strategy that controls the active and low-power state transitions using a  local server power controller and a global server farm power manager. 

\subsection{\titlename: Workload-Adaptive Algorithm}
\label{sec:handler}
We now present the design for our \titlename framework. As shown in Figure~\ref{fig:alg_overview}, the server farm power manager in the front end monitors the current load (number of pending jobs per server) and sends control commands to the local power controller. The server farm power manager puts the servers in either active or sleep modes. The bottom part of Figure~\ref{fig:alg_overview} presents state transitions coordinated by the local server power controllers. 


\begin{table}[htbp]	
	\captionsetup{font=footnotesize}
	\begin{footnotesize}
		%\begin{center}
		\begin{center}
		\caption{Notations in \titlename power management algorithm}
		\begin{tabular}{|c|l|}
			\hline
			{\bf Symbol} &{\bf \hspace{0.8in}Description}\\
			\hline
			{\normalsize $V_{act}$} & servers in active/package sleep mode \\ 
			\hline
			{\normalsize $V_{s}$} & servers in system sleep mode \\ 
			\hline
			{\normalsize $T_{s}$} & workload threshold to reduce active servers \\
			\hline
			{\normalsize $T_{w}$} & workload threshold to increase active servers \\
			\hline
			{\normalsize $N_{p}$} & number of provisioned shallow sleep servers \\
			\hline
			{\normalsize $\tau$} & delay time before entering system sleep \\
			\hline		
		\end{tabular}
		\label{table:notation}
		\end{center}
	\end{footnotesize}
	%\end{center}
\end{table}

\begin{algorithm}[ht]
	\footnotesize
	%\SetAlgoLined
	\KwIn{$T_{s}$, $T_{w}$, $N_{p}$, $\tau$, $n$ (total number of servers)}
	%\small
	%\tcc{By default, all servers are placed in $\mathcal{V}_{act}$}
	%\tcc{Initial state of each server is $lp_1$, the shallowest sleep state}
	\small
	%
	%\tcc{$jop\_threshold$ -- empirically estimated score value that may likely 
	%indicate JOP attack}
	%
	Initialization: 
	$V_{act}=\{s_1,s_2,...,s_n\} $; $V_{s}=\{\}$\;
	%	\For{i in [1,n]}{
	%		power state of $s_i$ $\leftarrow$ $idle$\;
	%		initial processor frequency  $f$ for $s_i$\;
	%	}
	\While{there are unfinished jobs}{
		
		\If{a new job $j$ arrives at time $t_a$}{		  
			%add $j$ to the global queue\;
			%$qsize \leftarrow qsize + 1$\;
			%update $H_q$ with $(t_a, qsize)$\;
			%		        \If{an active server with free core exists} {
			%		          schedule the new job on a free core\;
			%		          // priority: highest utilized server first\;
			%		          continue\;
			%		        }
			%            collect total number of jobs in system\;
			%		    add $j$ to the global queue\;
			compute $load\_per\_active\_server$\;
			\If{$load\_per\_active\_server>T_w$ and $|V_{s}|>0$}{
				%\If{$V_{s}$ is not empty}{
				retrieve a server $s$ from $V_{s}$\;
				$V_{act}$.add($s$)\; 
				%					//$s$ will be in active mode\;
				create a \emph{trans\_to\_active\_mode} request \emph{$tta\_r$}\;
				send \emph{$tta\_r$} to server $s$'s power controller\;
				%}
			}
			%      {
			%       keep $\mathcal{V}_{act}$ and $\mathcal{V}_{lp}$ unchanged\;
			%       }
		}
		
		\If{a job $j$ finishes at time $t_d$}{
			%$qsize \leftarrow qsize - 1$\;
			%update $H_q$ with $(t_d, qsize)$\;
			%	collect total number of jobs in system\;
			compute $load\_per\_active\_server$\;
			\If{$load\_per\_active\_server<T_s$ and $|V_{act}|>0$ }{
				%	\If{$V_{act}$ is not empty}{
				retrieve a server $s$ in $V_{act}$\;
				$V_{s}$.add($s$) \;
				%	//$s$ will be set to sleep mode\;
				create a \emph{trans\_to\_sleep\_mode} request \emph{$tts\_r$}\;
				\If{count of shallow sleep servers$>N_{p}$}{
					\emph{$tts\_r$}.enableDelayTimer($\tau$)\;
				}
			    \Else{
			    	\emph{$tts\_r$}.enableDelayTimer(infinity)\;
		    	}
				send \emph{$tts\_r$} to server $s$'s power controller\;
				%	}
			}
			%       {
			%        keep $\mathcal{V}_{act}$ and $\mathcal{V}_{lp}$ unchanged\;
			%        }
		}	
	}
	\caption{Global Server Farm Power Manager}
	\label{alg:scheduler}	
\end{algorithm}

\titlename automatically activates servers when the pending load becomes too high (that could lead to higher average job latency), and then places servers in low-power sleep mode to conserve energy when the workload becomes light. We achieve our goal of balancing energy consumption and latency by estimating the current load and placing servers in different power modes. There are two important parameters in Algorithm~\ref{alg:scheduler} that govern transitioning between active and sleep modes: 1. $T_s$, workload threshold per active server below which \titlename will put an active server to sleep, and 2. $T_w$, workload threshold per active server above which \titlename will wake up an inactive server.

{\bf Global Server Farm Power Manager}: All servers are initially in the shallow low-power state, and arriving jobs are placed in the server's local job queue. As jobs arrive, the \emph{load per active mode server} is computed dynamically by the power manager in the front end based on the number of jobs sent to individual servers and the completed jobs. The global server farm power manager maintains lists of servers in active and sleep modes. When new jobs arrive, it first checks if current load per active server is above $T_w$. If so, it selects a server in sleep server pool (if available) and sends a power mode transition request to the active state for that server. When the load per active server falls below $T_s$, the power manager selects an active server and sends a power mode transition request to enter sleep mode. Algorithm~\ref{alg:scheduler} describes the \titlename power manager with its notations shown in Table~\ref{table:notation}. 
 

\textbf{Local Server Power Controller:} The processor transitions to package sleep state when it becomes idle, and stays in that state until it receives the request to wakeup from the global power manager. If the server receives a request for transition to sleep mode, it will first finish up all the pending jobs in the local queue and then enters package sleep after which a delay timer is started. The server enters system sleep upon delay timer expiration. However, if the scheduler chooses to wake up the server before timer expiration (e.g., due to sudden load increase), the timer is reset and the server goes back to active mode.

For large server farms, we can adopt one of two possible solutions: 
\begin{inparaenum}
	\item Adopt a distributed power management approach where energy is optimized within individual domains of servers with their own power managers.
	\item Adopt a hierarchical solution with multiple levels of global power managers. 
\end{inparaenum} 
We note that a distributed power management approach may be more scalable with lower implementation complexity compared to a hierarchical approach that may involve longer latencies for decision making and higher bookkeeping overheads for the servers. 

\subsection{Adaptive Server Provisioning}
\label{sec:provision}
Job arrival pattern may have local spikes (bursty), during which the service latency may suffer, especially when the servers are in low power modes. To mitigate this problem, we provision a subset of servers in shallow sleep states dynamically by setting their delay timer values to infinity. \titlename determines the number of provisioned servers {\it dynamically} through measuring the current standard deviation in the job arrival rate observed over a period of 2 minutes. Specifically, the server provision module samples the number of arrivals and calculates the utilization for each sample period (one second in our current setting). It then uses the sampling window to determine the standard deviation in the level of system utilization. The module will provision $\alpha\times stdev\times number\_servers$ dynamically in shallow sleep state. $\alpha$ is a tunable parameter. By default we set it to 3.0, since it typically covers a vast majority of the population (e.g., more than 99\% of the population in Gaussian distribution).  


==> 2020-popcorns-T-SUSC (copy)/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
\subsection{Processor/System Low-power States and Power Model}
%\begin{asparaenum}
%\item[\textbf{ACPI-defined low power states}] 

%Emerging from embedded devices, low-power states are now an important feature targeted for power management in modern computer systems. Advanced Configuration and Power Interface (ACPI)~\cite{acpi} provides a standardized specification for platform-independent power management. The ACPI-defined interfaces have been adopted by several major operating system vendors~\cite{acpi_linux,acpi_bsd} and supported by various hardware vendors such as Intel and IBM~\cite{ibm_power7, intel_manual}. ACPI uses global states, \emph{Gx}, to represent states of the entire system that are visible to the user. Within each \emph{Gx} state, there are one or more system sleep states, denoted as \emph{Sx}. For instance, \emph{S0} is the working state and \emph{S1}, \emph{S3} are the system sleep states. When a computer system is in the \emph{S0} state, the processor is allowed to be in a set of \emph{C} states such as \emph{C0}, \emph{C1}, and \emph{C6}. A higher-numbered C state typically indicates more aggressive energy savings but also corresponds to longer wake-up latencies. Modern processors generally provide high parallelism by integrating multiple cores within one package. Therefore, low-power sleep states are supported at both core level and package level. Typically, the package \emph{C} state is automatically resolved to the shallowest sleep state among all the cores. In the rest of the paper, we will denote package \emph{C}  state as package sleep state. 
Low-power states are now an important feature that are widely supported in today's computing systems. The Advanced Configuration and Power Interface (ACPI)~\cite{acpi}
% provides a standardized specification for platform-independent power management. 
%The ACPI-defined interfaces have been adopted by several major operating system vendors~\cite{acpi_linux,acpi_bsd} and supported by various hardware vendors such as Intel and IBM~\cite{ibm_power7, intel_manual}. ACPI uses global states, \emph{Gx}, to represent states of the entire system that are visible to the user. Within each \emph{Gx} state, 
specifies various processor low power states, denoted as \emph{Cx}, and system low-power states, denoted as \emph{Sx}. 
%For instance, \emph{S0} is the working state and \emph{S3}, \emph{S4} are the system sleep states. When a computer system is in the \emph{S0} state, the processor is allowed to be in a set of \emph{C} states such as \emph{C0}, \emph{C1}, \emph{C3}, and \emph{C6}. 
A higher level C state or S state typically indicates more aggressive energy savings but also corresponds to longer wake-up latencies. 
%Modern processors generally provide high parallelism by integrating multiple cores within one package. 
For multi-core processor, low-power sleep states are supported at both core level and package level. When all cores become idle and  reside in some \emph{Core C state}, the entire package would be resolved to a certain C state, denoted as \emph{package sleep state}, which further reduces power. 
%Typically, the package \emph{C} state is automatically resolved to the shallowest sleep state among all the cores. 
Although processor sleep states can significantly reduce the power consumed by the processor, servers can still consume a considerable amount of power, as the platform may still remain active. As a result, in order to achieve further energy savings, \emph{system sleep states}, that also put platform components into low-power state, are considered for server farm power management.
%we consider additional full system sleep state. \titlename uses \emph{S3} as full system sleep state as it can further achieve substantial energy savings especially at low demand for server utilization.
%Other system sleep state such as \emph{S4} introduces hundreds of seconds of wakeup overhead, which is not applicable to latency sensitive workloads.  
%Figure~\ref{fig:power_profile} shows the power consumption for Xeon-E5 2680 processor with C1 and C6 processor sleep state enabled respectively. The power numbers are collected using PAPI API that interacts with the RAPL (Runing Average Power Limit) interfaces. %From the figure we can see that processor in  package C6 sleep state consumes much less power than processor in active state. 
%When the processor is in the \emph{C0} state, it may be associated with a performance state \emph{Px}, which corresponds to a specific DVFS setting. A hierarchical view of the low-power states specified in ACPI is shown in~\ref{fig:acpi_diagram}. The combination of system low-power state and CPU low-power state is used to characterize the low-power mode of an entire server. 
%\begin{figure}[h]
%	\centering
%	\vspace{-0.1in}
%	\centering
%	\includegraphics[scale=0.6]{./figure/power-profile.pdf}
%	\caption[Test]{Power profile of a 10-core Xeon processor with different C-state configurations. The y-axis is the range of power for the processor with the specific number of cores active and various utilization levels ranging from 10\% to 100\%.} %Note that each of the active cores settings, we generate various level of utilization to the active cores and measured the power, which explains why the power consumption for a specific number of active cores are a range of numbers.  }
%	\label{fig:power_profile}
%	\vspace{-0.1in}
%\end{figure}
%\footnote{We use a microbenchmark that can calibrate itself and occupy the core according to each utilization setting. To occupy multiple cores, we run multiple processes of this microbenchmark, each pinned to a specific core.}
\subsection{Server and Job Model}
We model the server farm as a multi-server system that could process multiple jobs (upto the number of total cores) at a time. 
%In this paper, we use four synthetic workloads with average job execution times shown in brackets next to them: Google search [4.2 ms], Apache [75 ms], Mail [92 ms] and DNS query [194 ms] jobs, and one real system trace, Wikipedia, with an average workload execution time of 3.5 ms. 
%The job execution time parameters were derived from prior works and actual workload traces~\cite{wiki_trace,meisner2012dreamweaver}. 
{\em Utilization factor} is defined as the product of the job arrival rate and the average execution time, which is also the fraction of time that the server is expected to be busy executing a job.
%The term {\em Utilization factor} is defined as $\rho=\frac{\lambda}{\mu}$, the fraction of time the server is expected to be busy executing a job. 
We assume that a system-wide load balancer dispatches jobs to the servers within the server farm. 
%{\bf FAN: Plug in details about the window of observation, number of servers}. 
The {\em job latency} is defined as the time elapsed from when a job arrives to when the job completes its execution and departs the server. In this paper, the $90^{th}$ percentile job latency is considered as the QoS target.
%\begin{figure}[ht]
%	\centering
%	%\subfloat[b][Overview of \titlename Hiearchical Algorithms]{
%	\includegraphics[scale=0.3]{./figure/algorithm_chart.pdf}
%	%}
%	%	\vspace{-0.3in}
%	%	\subfloat[b][MPPP]{
%	%		\includegraphics[scale=0.58]{../figure/scalability/google_scal_mmpp.pdf}
%	%		\label{fig:google_scal_mmpp}}
%	\caption{\titlename Power Management Framework.}
%	\label{fig:alg_overview}
%	\vspace{-0.2in}
%\end{figure}



==> 2020-popcorns-T-SUSC (copy)/exp_setup.tex <==
\section{Experimental Setup} 
We perform two sets of experiments: 1. simulations to explore the Pareto-optimal energy-latency tradeoff as well as corresponding $T_s$, $T_w$ and $\tau$ settings, and 2. prototype implementation on a testbed with web server deployment. In this section, we elaborate on the experimental setup for both approaches.
\begin{figure}[htbp]
	\captionsetup{font=small}
	\centering
	\includegraphics[scale=0.60]{./figure/power_profile_cloud.pdf}
	\caption[test]{Power profile of a 10-core Xeon E5 processor with C0-C1 and C0-C6 transition settings whenever the server is idle.\protect\footnotemark}
	\label{fig:power_profile}
\end{figure}
\footnotetext{We use a microbenchmark that can calibrate itself and occupy the core based on required utilization settings. To occupy multiple cores, we run multiple copies of this microbenchmark each pinned to a core.}

\begin{table}[htbp]
	\footnotesize
	\captionsetup{font=small}
	\centering	
    \caption{Power (W) breakdown for a system with $n_{a}$ active cores} 
	\begin{tabular}{|p{1.5cm}<{\centering}|p{1.3cm}<{\centering}|p{1.4cm}<{\centering}|p{1.3cm}<{\centering}|p{0.8cm}<{\centering}|}
		\hline
		\multirow{2}{*}{\bf Component} & Core sleep C1$^{\ast}$& Core sleep C6 $^{\dagger}$& Pkg. sleep C6 &  System sleep \\
		\hline
		%	{\bf Component} & Core sleep & Core sleep&Pack. sleep & Server sleep \\
		%	& C1& C6 & C6&   \\
		%  \hline
		\multirow{2}{*}{CPU} & 33.0+$3.1\times(n_{a}-1)$ & 23.0+$3.8\times(n_{a}-1)$ & \multirow{2}{*}{8.3} & \multirow{2}{*}{8.3} \\
		%\hline
		%{Chipset~\cite{liu2014sleepscale}} & 3.7 & 3.7 & 3.7 & 3.7 \\
		\hline
		RAM~\cite{intel_e5}     & 10.8 & 10.8 & 4.9 & 1.4 \\
		\hline
		Platform~\cite{powernap}     & 45.5 & 45.5 & 23.6 & 4.8 \\
		\hline
		\multirow{2}{*}{Total Power} & 89.3+$3.1\times(n_{a}-1)$ & 79.3+$3.8\times(n_{a} -1)$ & \multirow{2}{*}{36.8} & \multirow{2}{*}{14.5} \\
		\hline	
	\end{tabular} \\
	${\ast} $ processor is active and the rest of the idle cores are in $C1$ state. \\ 
	$\dagger$ processor is active and the rest of the idle cores are in $C6$ state.
	\label{table:powermode}
\end{table}

\begin{table}[htbp]
	\footnotesize
	\captionsetup{font=small}
	\centering
    \caption{Processor/System low-power states and wakeup latencies}
	\begin{tabular}{|c|c|c|}
		\hline
		Low-power State & Wake-up latency \\ \hline
		core sleep C1   & 10 $\mu$s           \\ \hline
		core sleep C6   & 82 $\mu$s           \\ \hline
		package sleep C6   & 1 ms           \\ \hline
		system sleep    & 5 s      \\ \hline
	\end{tabular}    
	\vspace{-0.15in}
	\label{table:latency-table}
\end{table}

\subsection{Processor Power Profile and Server Power Model}

We profile the power consumption of the Intel Xeon E-5 processor~\cite{intel_e5} using Intel's \emph{Running Average Power Limit} (RAPL) interface. We build a customized cpuidle governor that allows specified low-power state transitions. The processor is programmed to transition between active state (C0) and low-power state $Cx$ (e.g., C1, C6). Figure~\ref{fig:power_profile} shows the measured power consumption of the processor for two configurations: \emph{C0-C1}, \emph{C0-C6} and at utilization levels from 0\% to 100\%. Using linear regression, a power model is built for the processor based on the sleep state selection and the number of active cores at full utilization. Table~\ref{table:powermode} shows the power consumption when a certain state is chosen for sleep mode. Table~\ref{table:latency-table} shows the wakeup latencies for various low-power states. Note that the processor sleep state transition latencies are reported by the Linux cpuidle driver~\cite{pallipadi2007cpuidle}.

\subsection{Simulation Platform}

\titlename uses an event-driven simulator based on Bighouse~\cite{bighouse} that models server farm workloads and multi-server activity. We simulate a server farm with 100 ten-core servers (by default).  In all of our experimental results, we report the steady state statistics by disregarding the warm-up period of the first 10,000 jobs. In the simulation, we use short latency (Web service-like) jobs with $s=4.2 ms$ and long latency (DNS service-like) jobs with $s=194 ms$ as representatives based on prior studies~\cite{powernap}. For each of the representative workloads, we generate synthetic job arrivals with different utilization levels (0.1 for low, 0.3 for average~\cite{barroso_isca07}, and 0.6 for high). Random job arrivals are modeled by Poisson process~\cite{meisner2012dreamweaver}. Besides synthetic workload, we also perform simulation based on Wikipedia traces.

\subsection{Real System Experiments on Testbed}

We deploy a testbed with a cluster of 10 application servers together with one load-generating server and one load-balancing server; all servers support Intelligent Power Management Interface (IPMI) interface~\cite{openipmi} for system-level power monitoring. Each application server is configured with the apache web service. The load generator keeps sending web requests to the system according to real system traces (See Section~\ref{sec:evaluation} for further details).


==> 2020-popcorns-T-SUSC (copy)/experiment.tex <==
\section{Evaluation}
\label{sec:experiment}
\subsection{Experimental Setup}
%{\color{blue}Found some real traces}
Our experiments were performed using HolDCSim, an event-driven simulator~\cite{HolDCSimHolisticSimulator},
which simulates interdependent asynchronous task executions, and implement
custom server job scheduling and network routing algorithms. This allows us to
simulate a large number of servers and switches relatively easily. The simulator
allows us to specify our own power model and sleep state transition mechanisms
and calculate the overall energy consumption for the simulator. The network is
configured using a fat tree-topology as shown in Figure~\ref{figure12}.  We
simulate two classes of real-world applications: %{\bf GV- itemize the list {\color{blue}Done}} 
%\begin{itemize}
\emph{web service}: two large sized (uniformly distributed around 500 ms service time) parent-child tasks,
\emph{web search}: a parent task search task querying five subtasks to run smaller search process (uniformly distributed around 100 ms CPU service time). All the network routing policies consider the QoS threshold of 10X the total CPU time of all tasks in the job when choosing the job selection.
%\end{itemize}

We assume that each of the tasks can be executed on any server machine and if enough processing cores available co-located in the same server.  The communication patterns and the DAG for the two workloads are illustrated in Figure~\ref{fig:ws-graph}, and Figure~\ref{fig:wsv-graph}.

We carefully select delay timer values for sleep state transitions~\cite{yaoWASPWorkloadAdaptive2017} for server and network by trying each value in the search-space, starting with first determining the delay timer value for Sleep state 1 with the lowest energy consumption, then fixing the lowest timer value found previously for state 1 to determine the delay timer for sleep state 2, and so on.



% We simulate a data center cluster with 16 servers and 20 switches.  We simulate three classes of real applications: \emph{web service} (small-sized workload), \emph{web search} (medium-sized workload), and \emph{DNS service} (large-sized workload). For each of the representative workloads, we generate synthetic job arrivals with different utilization levels (10\% for low, 30\% for average, and 60\% for high utilization~\cite{fan2007power}). Random job arrivals are modeled by Poisson process~\cite{meisner2012dreamweaver}... The switch and server power under different sleep states is based on Tables~\ref{Switch Power model} and ~\ref{Serverpowermodel}. Besides, we set the server wakeup latency as 1ms and local queue size threshold in Algorithm~\ref{algorithm4} as 10. For the traffic thresholds and latency values in Table~\ref{algorithm1table}, we set $T_s$ as 10, $T_a$ as 2, $\tau_{wakeup}^{LC}$ as 2ms, $\tau_{wakeup}^{port}$ as (2ms$2$\mu$s), $\tau_{LPI}^{port}$ as$1$\mu$s, $\tau_{sleep}^{LC}$ as$1$\mu$s, and $\tau_{off}^{LC}$ as 2s.

\subsubsection{Job arrivals patterns}
\label{workloads}

We use two kinds of job arrivals in our study.
%\begin{itemize}
%\emph{Poisson based Random arrival of jobs}: Jobs are generated based on Poisson process for arrival times and a uniform distribution for task service times. The average arrival rate $\lambda$ value for each three load levels low, medium and high is derived from the approximate desired utilization levels for the server farm $\rho$ in this case. 
% \begin{comment}
%{\bf GV- I thought that we moved away from target utilization and simply wanted to have three levels of arrival rates. Can you double check and change as necessary? {\color{orange} Wanted to hint at how we arrive the arrival rate numbers. Added that it will not be thre resultant }}
%\end{comment} 
The arrival rate is given by $\lambda = (Num_Servers * Num * Cores * \rho)/ Avg_TaskSize * NumTasksperJob$. Thereby targeting $\rho$ values of 15\%, 30\% and 60\% we derive the $\lambda$ values. Due to the variation in the scheduling policy, task inter-dependency, randomized job task and arrival times and sleep state transitions the resultant server utilization level may not match with targeted utilization levels.

\emph{Markov Modulated Poisson Process}: Similar to workload used in \cite{yaoWASPWorkloadAdaptive2017}, MMPP arrivals generates a two different states of arrival rates. The normal utilization phase similar to the Poisson workload and a bursty period where the arrival rate is 1.5X the $\lambda$ in the normal phase. We choose the bursty period to last 10 secs between 20 seconds of normal phase. The load levels of low, medium and high arrival rate and obtained in the similar fashion as the basic poisson based arrival workload.

 \emph{Trace based arrival job arrival pattern}: We use publicly available job arrival trace from NLANR~\cite{NationalLabApplied} for a real world system. We chose NLANR trace since it inherently has a high variation in job inter-arrival rate. The load levels of low, medium and high arrival traces are obtained by scaling the inter-arrival times between the jobs in the original trace by a factor.

%\end{itemize}


\begin{figure} [!h]
	\centering
	\captionsetup{font=small}
	\subfloat[Steps in a web search request.]{		\includegraphics[scale=0.34]{figures/wsearchdraw.pdf}
		\label{fig:ws-figure90}
}
	\subfloat[DAG of a web search job.]{		\includegraphics[scale=0.15]{figures/wsearchDAG.pdf}
		\label{fig:ws-dag}
}
	\caption{Web search communication patterns (left) and DAG of a web search job (right). 
		Task 1 is executed by the master server, while task 2 - 6 are processed by different indexers, and master server communicates with all the indices.}%{\bf GV--tiny font}}
	\label{fig:ws-graph}
\end{figure}

\begin{figure} [!h]
	\centering
	\captionsetup{font=small}
	\subfloat[Steps in a web service request.]{
		\includegraphics[scale=0.34]{figures/wsdraw-2.pdf}
		\label{fig:wsv-figure90}
s	}
	\subfloat[DAG of a web service job.]{
		\includegraphics[scale=0.15]{figures/wsDAG.pdf}
		\label{fig:wsv-dag}
	}
	\caption{Web service communication patterns (top) and DAG of a web service job (bottom). 
		Task 1 is executed by application server, while task 2 is assigned to database server.}%{\bf GV--tiny font{\color{green} Changed}}}
	\label{fig:wsv-graph}
\end{figure}

\subsubsection{Quality of Service Constraints}
We consider the minimum time a job takes to complete to be the sum of computation time of each task in the job and time it takes for all the inter-task communications to finish at the fastest possible bandwidth in the network. For instance, for a two-task job with 500ms of CPU cost each and a 10 MB of network communication on the 10 Gbps maximum link capacity between two nodes, the minimum time for job execution will be \textit{500ms x 2 + 75 ms (data transfer time) = 1075 ms}. Similar to other works (e.g.,~\cite{yaoWASPWorkloadAdaptive2017}), we consider the quality of Service (QoS) deadline for the job scheduler to be 10 X the minimum job execution to enable enough slack to allow multiple jobs and enable energy optimizations.

\subsection{Baseline policies and Evaluation methodology}

There are two major objectives: first to prove that the smart use of line card sleep states with our proposed Algorithm~\ref{algorithm1}, does reduce power consumption in Popcorns-Pro compared to no power management policy on the switches at all; second, our proposed \PopCorns %{\bf GV-- Repeated use of Popcorns in many places. Should change it to Popcorns-Pro{\color{green} Changed all}}
algorithm~\ref{algorithm2} can further save power, compared to other job placement algorithms not taking both the network and server status into consideration. We consider the four combinations of the below server-specific and network-specific energy optimization policies. As shown in the section ~\ref{sec:motivation}, we have seen that switch sleep states without any optimization can still yield some energy savings, and it is important to further optimize the energy savings for them.

\subsubsection{Server based policies}
	The below two policies represent a common server selection policy and energy optimized server policy.
{\textbf{Random Server allocation}-\textit{SB}} %{\bf GV--boldify this and everything similar below{\color{green} Changed}}
Following a traditional server load balancing approach, tasks are assigned randomly to all servers and the processing cores as they come in, without any consideration for task dependency and core locality in the data centers. 

{\textbf{Workload Adaptive using Server Low-Power State Partitioning-\textit{WASP}}} This policy represents recent works~\cite{yaoWASPWorkloadAdaptive2017} which consolidate jobs into fewer server while optimizing for keeping more servers in sleeping state. These optimizations are typically developed by system developers without considering the network energy optimization. In WASP, a set of servers are kept in the unused state to allow them to achieve the most energy efficient sleep state, while the remaining jobs are processed on the remaining servers. The servers are reassigned between the two sets depending the measured input load on the entire server pool.

\subsubsection{Network based policies}
The following two approaches to network routing in the data center.

{\textbf{Shortest Path-\textit{SP}}} This baseline network path allocation uses Djikstra's algorithm to forward flows across the two end points. This policy represents the traditional network routing algorithm available which chooses the shortest number of hops which also considering the QoS latency requirements for the current flow. 

{\textbf{Elastic tree-\textit{ET}}} Recent work on the improving network energy efficiency have considered various heuristics to consolidate flows into fewer switches. The Elastictree ~\cite{hellerElasticTreeSavingEnergy2010} baseline represents one of the most commonly cited work in this area, which tries keep fewer switches in active state in highly redundant network typologies such as the fat tree topology. We implement the greedy bin packing approach in our experiment where the heuristic chooses the leftmost path at every switch exit to reach the destination. These approaches assume a fixed server task allocation and hence cannot fully optimize for efficiency.

\input{baselines}
%
% The baseline comparison policy in our experiment is the Server-Balanced (SB) Algorithm for task placement, which dispatches tasks uniformly to all the servers (i.e.,$n_{th}$ task mapped to server with index $n\%N$), with the same power management policy on switches (Algorithm~\ref{algorithm1}), but not on the servers. In other words, the baseline Algorithm~\ref{algorithm4} does not consider current power state and local queue size of servers, nor the joint task placement and routing.
%%$n$ to server $n\%N^{server}$, where $N^{server}$ denotes the totoal number of servers that could be scheduled in DCN. 
%After tasks are scheduled on servers, the Server-Balanced Algorithm uses single shortest path routing (e.g., Dijkstra's algorithm) for interdependent tasks communication in the network. 
%%This algorithm neither considers task interdependence within a job nor the network status. 
%Thus as long as there is an inactive line card or port on the routing path, it needs to be awakened. Note that since tasks of the same job are placed on adjacent servers, the communication between interdependent tasks would mostly be within a pod (See section~\ref{sec:dc-sys}), which involves only 2$\sim$4 hops. Therefore this baseline algorithm might already perform better than random job placement in terms of DCN power consumption in this sense.
%%{\color{blue}FY: I am not convinced by this argument}. Thus we come up with another vanilla baseline algorithm that randomly places tasks on servers, and the routing path between interdependent tasks is also randomly chosen.



%

\begin{comment}
\begin{algorithm}
	\SetAlgoNoLine
	\caption{Server-Balanced Algortihm}
	\label{algorithm3}
	\KwIn{Pre-computed Dijkstra's shortest paths set $DijkstraPaths$ between any pair of network nodes, number of sevres $N$ in DCN }
	\KwOut{Job placement and corresponding routing path}
	
	\While{task $t_i$ with task id $i$ of job $j$ arrives}
	{
		place $t_i$ on server $i\%N$;
		
		then the interdependent task $t_k$ of $t_i$ with task id $k$ will be placed on server $k\%N$;
		
		get the routing path $P$ from server $i\%N$ to server $k\%N$ from $DijkstraPaths$;
		
		return server $i\%N$ and path $P$;
	}
\end{algorithm}
\end{comment}

%\subsection{Power Consumption}
%%
%In this section, we compare the simulation results on power consumption under three power management policies. The first one is what we propose in algorithm~\ref{algorithm1}, namely port will transition to LPI state when traffic load is below threshold $T_{a}$, and line card will transition to sleep state when all its ports are in LPI state; line card will transition to active state as long as traffic load of one of its port exceeds threshold $T_{s}$. And the results for this power management is corresponding to $LC (Line Card) + SP (Switch Port)$ in figure~\ref{figure4}. The second policy is that all the line cards remain active, but port can transition to LPI mode when current traffic load is below $T_{a}$, the result of which is represented by $SP$ in figure~\ref{figure4}. In the third power management policy, all the ports remain active, but line card can transition to sleep state, and the result under this policy is denoted by $LC$ in figure~\ref{figure4}. 
%To demonstrate the effectiveness of Popcorns in terms of energy savings, we evaluate three power management policies. The first policy, denoted as $SP$, only considers low power mode for the ports. The line cards remain active all the time. However, ports can transition to LPI mode whenever current traffic load for the port is below a threshold $T_{a}$. The second power management policy--$LC$ leverages line card sleep states. Contrary to the $SP$ policy, all the ports are kept active. On the other hand, the line cards in switches can transition to power-saving sleep state. The third policy is PorpCorns' power network management policy as shown in~\ref{algorithm1} that leverages both port and line card low power states (denoted as  $LC (Line Card) + SP (Switch Port)$). Specifically, under this scheme, switch ports transition to LPI state when traffic load is below the threshold $T_{a}$, and line card will transition to sleep state when all its ports are in LPI state; line card will transition to active state as long as traffic load of one of its port exceeds anotehr threshold $T_{s}$. For each of the policies, we setup two different job placement configurations: Global Foresight Algorithm (shown using the suffix of $-GP$) and Server-Balanced Algorithm (shown using the suffix of $-SB$).
%To demonstrate the effectiveness of Popcorns in terms of the first objective, we break the power saving into two parts: network and server power saving. We calculate the power consumption of network part with PorpCorns' network power management policy as shown in Algorithm~\ref{algorithm1}, compare it with the case when all the line cards and ports are kept active all the time, and obtain the network power saving. To achieve our second objective, we set up two different job placement configurations: Cooperative Network-Server Algorithm (shown using the suffix of $-CNS$) and Server-Balanced Algorithm (shown using the suffix of $-SB$).


%energy savings, we evaluate three power management policies. The first policy, denoted as $SP$, only considers low power mode for the ports. The line cards remain active all the time. However, ports can transition to LPI mode whenever current traffic load for the port is below a threshold $T_{a}$. The second power management policy--$LC$ leverages line card sleep states. Contrary to the $SP$ policy, all the ports are kept active. On the other hand, the line cards in switches can transition to power-saving sleep state. The third policy is PorpCorns' power network management policy as shown in~\ref{algorithm1} that leverages both port and line card low power states (denoted as  $LC (Line Card) + SP (Switch Port)$). Specifically, under this scheme, switch ports transition to LPI state when traffic load is below the threshold $T_{a}$, and line card will transition to sleep state when all its ports are in LPI state; line card will transition to active state as long as traffic load of one of its port exceeds anotehr threshold $T_{s}$. 

%\subsection{DNS Service}
 %Figure~\ref{fig:dnsdraw} and ~\ref{fig:dnsdag} shows the process of DNS
service and its corresponding job DAG. In simulation, we set the flow size to be
100KBytes and average job service time is randomly generated between 150ms and 200ms based on prior studies~\cite{meisnerPowerNapEliminatingServer}.

%\begin{figure*}[htbp]
%	\centering
%	\captionsetup{font=small}
%	\subfloat[b][Steps in DNS Resolution of www.gwu.edu.]{
%		\includegraphics[scale=0.7]{figures/dnsdraw.pdf}
%		\label{fig:dnsdraw}}
%	\subfloat[b][DAG of DNS jobs generated in our experiment, with random size between 100ms and 150ms. Each job consists of 4 tasks, and there are interdependence and communication between task 1 and 2, 3, 4.]{
%		\includegraphics[scale=0.3]{figures/DNSdag.pdf}
%		\label{fig:dnsdag}}
%	\vspace{-6pt}
%	\caption{DNS service.}
%	\label{fig:dnsjob}
%	\vspace{-0.16in}
%\end{figure*}


%\begin{figure}
%	\captionsetup{font=small}
%	\centering\includegraphics[width=0.25\textwidth]{figures/DNSdag.pdf}\caption{DAG of DNS jobs simulated in our experiment, with random job size between 100ms and 150ms. Each job consists of 4 tasks, and there are interdependence and communication between task 1 and 2, 3, 4.}  
%	\label{figure99}
%\end{figure}


%\begin{figure}[!h]
%	\centering
%	\captionsetup{font=small}
%	\subfloat[Low Arrival Rate \newline $\lambda$ = 10 Jobs/Sec]{
%		\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=user_specify_Q=10_FS=100_C=4_U=25.png}
%		\label{2poi-elastic_tree_h_random}
%	}
%	\subfloat[Medium Arrival Rate \newline($\lambda$ = 30 Jobs/sec)]{
%		\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=user_specify_Q=10_FS=100_C=4_U=40.png}
%		\label{2poi-elastic_tree_h_random}
%	}
%	\subfloat[High Arrival Rate \newline ($\lambda$ = 60 Jobs/sec)]{
%		\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=user_specify_Q=10_FS=100_C=4_U=70.png}
%		\label{2poihigh-elastic_tree_h_wasp}
%	}
%	\caption{Energy Savings comparison for different server and network path selection algorithms with Poisson Job Arrival Pattern for service based jobs two-task model}
%	\label{fig:poi-ser}
%\end{figure}

\begin{figure*}[!h]
	\centering
	\captionsetup{font=small}
	\subfloat[Low Arrival Rate \newline $\lambda$= 8 Jobs/Sec]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=mmpp_Q=100_FS=100_C=1_U=10.png}
		\label{djikstra_h_random}
	}
	 \subfloat[Medium Arrival Rate \newline $\lambda$ = 15 Jobs/Sec]{
	 	\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=mmpp_Q=100_FS=100_C=1_U=25.png}
	 	\label{elastic_tree_h_random}
	 }
	\subfloat[High Arrival rate \newline $\lambda$ = 30 Jobs/Sec ]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=mmpp_Q=100_FS=100_C=1_U=40.png}
		\label{elastic_tree_h_wasp}
	}
	\caption{Energy Savings comparison for different server and network path selection algorithms with MMPP based Job Arrival Pattern for service based 2 task model. Every 30 seconds we have 10-second bursts with 1.5x Arrival rate.}
	\label{fig:mmpp-ser}	
\end{figure*}
\begin{figure*}[!h]
	\centering
	\captionsetup{font=small}
	\subfloat[Low Arrival Rate \newline Avg. Rate = 10 Jobs/Sec ]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=trace_Q=10_FS=100_C=4_U=10.png}
		\label{djikstra_h_random}
	}
	 \subfloat[Medium Arrival Rate \newline Avg. Rate = 16 Jobs/Sec]{
	 	\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=trace_Q=10_FS=100_C=4_U=25.png}
	 	\label{elastic_tree_h_random}
	 }
	\subfloat[High Arrival rate \newline Avg. Rate= 32 Jobs/Sec]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/service/W=trace_Q=10_FS=100_C=4_U=55.png}
		\label{elastic_tree_h_wasp}
	}
	
	\caption{Energy Savings comparison for different server and network path selection algorithms with NLANR trace based Job Arrival Pattern for service based 2 task model.} %{\bf GV--make figure and fonts bigger}{\color{green} Changed}}
	\label{fig:trace-ser}
\end{figure*}

%\begin{figure}[!h]
%	\centering
%	\captionsetup{font=small}
%	\subfloat[Low Arrival Rate\newline $\lambda$=10 Jobs/Sec]{
%		\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=user_specify_Q=10_FS=10_C=4_U=15.png}
%		\label{djikstra_h_random}
%	}
%	\subfloat[Medium Arrival Rate \newline $\lambda$=30 Jobs/Sec ]{
%		\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=user_specify_Q=10_FS=10_C=4_U=35.png}
%		\label{elastic_tree_h_random}
%	}
%	\subfloat[High Arrival Rate \newline $\lambda$=50 Jobs/Sec ]{
%		\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=user_specify_Q=10_FS=10_C=4_U=55.png}
%		\label{elastic_tree_h_wasp}
%	}
%	\caption{Energy Savings comparison for different server and network path selection algorithms with Poisson Job Arrival Pattern for search based 6-task job model.}
%	
%	\label{fig:pois-search}
%	
%\end{figure}

\begin{figure*}[!h]
	\centering
	\captionsetup{font=small}
	\subfloat[Low Arrival Rate \newline $\lambda$=8 Jobs/Sec]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=mmpp_Q=10_FS=10_C=4_U=15.png}
		\label{djikstra_h_random}
	}
	 \subfloat[Medium Arrival Rate \newline $\lambda$=15 Jobs/Sec ]{
	 	\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=mmpp_Q=10_FS=10_C=4_U=35.png}
	 	\label{elastic_tree_h_random}
	 }
	\subfloat[High Arrival Rate \newline $\lambda$=25 Jobs/Sec]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=mmpp_Q=10_FS=10_C=4_U=55.png}
		\label{elastic_tree_h_wasp}
	}
	
	\caption{Energy Savings comparison for different server and network path selection algorithms with MMPP based Job Arrival Pattern for search based 6-task job model. Every 30 seconds we have 10-second bursts with 1.5x Average Arrival rate.}% {\bf GV--make figure and fonts bigger}{\color{green} Changed}}
	\label{fig:mmpp-search}
	
\end{figure*}

\begin{figure*}[!h]
	\centering
	\captionsetup{font=small}
	\subfloat[Low Arrival Rate \newline Avg. Rate = 9 Jobs/Sec]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=trace_Q=10_FS=10_C=4_U=15.png}
		\label{djikstra_h_random}
	}
	 \subfloat[Medium Arrival Rate \newline Avg. Rate = 15 Jobs/Sec]{
	 	\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=trace_Q=10_FS=10_C=4_U=25.png}
	 	\label{elastic_tree_h_random}
	 }
	\subfloat[High Arrival Rate \newline Avg. Rate = 30 Jobs/Sec]{
		\includegraphics[width=0.33\textwidth]{figures/evaluation/search/W=trace_Q=10_FS=10_C=4_U=50.png}
		\label{elastic_tree_h_wasp}
	}
	
	\caption{Energy Savings comparison for different server and network path
    selection algorithms with NLANR trace based Job Arrival Pattern for search
    based 6-task job model.}
	\label{fig:trace-search}

\end{figure*}

%\twocolumn
\subsection{Evaluation Results}
%%
\subsubsection{Energy Savings Comparison}
We compare the average energy consumption per job, for different combination of
network and server selection algorithm with Popcorn's selection algorithm. We
compare against a combination baseline policies WASP and random server
allocation policies with Elastictree and Shortest Path network selection
algorithms. As shown in Figure~\ref{fig:mmpp-ser}, popcorn algorithm for 2-task
service based job model for random arrival job provides significant savings
compared to Shortest-path based policies. This is attributed to fewer switches
and server being active. For ElasticTree based runs in figure
~\ref{fig:mmpp-ser}, using WASP as server allocation policy does provide more
opportunities for network consolidation and hence decreased savings. As we
increase the arrival rate to 60 Jobs/sec in figure, we see that Elastictree based runs perform
closer to \PopCorns as there are fewer opportunities for savings. We note that due to the bursty
nature of MMPP arrival rates (as discussed in section ~\ref{workloads}), the increased
delay in waking up additional switches leads to slower flow transmission rate
and increased energy consumption. We gather that server-only optimizations are
not always optimal when considering the whole data center energy consumption.
With NLANR trace based job arrivals. 

For Search based workload discussed in beginning of section ~\ref{sec:experiment}, the \PopCorns algorithm still results in significant savings.
We also see WASP based server optimization consistently performing better than Random server allocation. This is attributed to smaller communication size between each parent and child tasks and minimal time wasted waiting for the network data to arrive for processing. 






\subsection{Flow size sensitivity}

The goal of this experiment is to determine if the routing path and server selection
by \PopCorns algorithm is resilient to increases in network flow sizes and
thereby increased network utilization. As we see in figure ~\ref{fig:flows} the
\PopCorns policy's is able to select paths and servers which are least affected
by the increase in flowsizes. Shortestpath based policies use most number of
switches and with increasing flow sizes there are fewer chances going to sleep
and hence consume the most energy. Elastic tree's greedy bin packing of flow
consolidation benefits from some network consolidation but with the non-optimal
server selection leading to longer flow communication times, the energy
consumption increases exponentially.

\begin{figure}[h]
	\captionsetup{font=small}
	\centering\includegraphics[width=.85\linewidth]{figures/flowsize/W=user_specify_U=11_Q=10.png}
	\caption{Energy consumption/Job for various flow sizes for different server
    scheduling and network routing algorithms. The experiment involves a 1024
    server fat-Tree topology with WebService jobs arriving randomly with a Poisson random
    variable value $\lambda$ = 25 jobs/sec and 10X QoS threshold.} %{\bf GV--have you defined QoS as a function of execution time elseshere? {\color{green}DONE-In the experimental section}}.}
	\label{fig:flows}
\end{figure}

%\subsection{Sleep Timer Sensitivity}
%
%\begin{figure}
%	\captionsetup{font=small}
%	\centering\includegraphics[width=\textwidth]{figures/parameter_study/s1.png}\caption{Exploring S2 parameters}
%	\label{figure13}
%\end{figure}


\subsection{Job completion latency Comparison}
\begin{figure}[!h]
	\captionsetup{font=small}
	\includegraphics[width=1\linewidth]{figures/cdf/cdf33.png}\caption{Cumulative-Distributed-function
    plot of job latencies for different server scheduling and network routing
    algorithms. The experiment involves a 1024 server fat-Tree topology with
    WebService modeled jobs arriving randomly with a Poisson random variable value $\lambda$ = 25
    jobs/sec and QoS threshold as 10X.}%{\bf GV-- have you defined acronymns above?{\color{green} Added in the baseline section}}}
	\label{cdf}
\end{figure}

Although all the algorithms discussed, consider the QoS latency threshold of
10x (Sum of Task Size of all the tasks in the job) for network
routing path selection, we see that the jobs in the \PopCorns algorithm are much
below the threshold in figure ~\ref{cdf}. Comparing WASP based policies with Server
balanced random server selection scheme, fewer servers being utilized in WASP,
the transmission time is higher and thus resulting in higher latencies.
\begin{figure} []
	\captionsetup{font=small}
	\includegraphics[width=1\linewidth]{figures/energy_distribution/popcorns.pdf}
	\caption{Component-wise energy distribution for Popcorns in Joules for 500
		second execution of 1024 server Fat-Tree topology with WebService model jobs arriving randomly (Poisson distribution) with $\lambda$ = 25 jobs per second. The energy consumed at different sleep states of the switch is also shown. }
	\label{fig:Popcorn-component}
\end{figure}

\begin{figure} []
	\captionsetup{font=small}
	\centering\includegraphics[width=1\linewidth]{figures/energy_distribution/wasp-et.pdf}\caption{Component-wise
		energy distribution for WASP server scheduling policy with Elastic tree
		as network routing algorithm in Joules for 500 second execution of 1024
		server Fat-Tree topology with WebService model jobs arriving randomly (Poisson distribution) with $\lambda$=25 jobs per second. The energy consumed at different sleep states of the switch is also shown.}
	\label{fig:WASP-component}
	
\end{figure}

\subsection{Energy Distribution}

In this section we illustrate how system architects can utilize our simulated
settings and the power model to understand which component in the hardware
%infrastructure to focus on for most effective savings in energy. Figure
~\ref{fig:Popcorn-component} shows the energy consumed by each component in the
switch power model at each of the sleep state of the switch for typical
workload. This allows the system architect to focus their limited resources
towards optimizing a particular system architecture. For instance, looking at
figures ~\ref{fig:Popcorn-component} and ~\ref{fig:WASP-component}, we see that
most energy consumed by the network processor in its deepest sleep state. It can
also tell that a high cost design change for Sleep state S1 has more benefit
when using the Popcorns policy when compared to WASP and Elastictree policy.


 
\begin{comment}

	\subsubsection{Real traces}
	{\color{blue}Results from real traces}
	
	\subsubsection{DNS Service}
	Figure~\ref{figure100} and Figure~\ref{figure99} show the process of DNS service and its corresponding job DAG. In simulation, we set the flow size to be 100MB and the average job service time is randomly generated between 150ms and 200ms based on prior studies~\cite{meisner2009powernap}~\cite{he2013next}. Since our experiment is based on multi-task job, we define the service time as average task size (e.g. 75ms$\sim$100ms for a DNS task based on job DAG), and the system utilization rate is defined as \emph{service time}$*$\emph{arrival rate}.
	
	%{\color{blue}FY: how do you define server time for a multi-task job?}.
	\begin{figure*}
	\centering
	\captionsetup{font=small}
	\subfloat[DNS average power]{
	\includegraphics[scale=0.1]{figures/powerdns.pdf}
	\label{fig:dnspower}
	}
	\subfloat[DNS latency, Utilization=0.1]{
	\includegraphics[scale=0.1]{figures/dnsp1-0.pdf}
	\label{fig:dns_pp_0.1_90th}
	}
	\subfloat[DNS latency, Utilization=0.3]{
	\includegraphics[scale=0.1]{figures/dnsp3-0.pdf}
	\label{fig:dns_pp_0.3_90th}
	}
	\subfloat[DNS latency, Utilization=0.6]{
	\includegraphics[scale=0.095]{figures/dnsp6-0.pdf}
	\label{fig:dns_pp_0.6_90th}
	}
	
	\caption{DCN executes 2000 Poisson-arrival DNS jobs under low, medium, and high system utilization respectively. Suffix $-CNS$ represents Cooperative Network-Server Algorithm and $-SB$ denotes Server-Balanced Algorithm.}
	\label{fig:dns-exp}
	
	\end{figure*}
	
	
	%Figure~\ref{fig:dnspower} shows the power saving corresponding to the execution of 2000 DNS jobs, compared to the baseline policies. We can see that for each configuration, Popcorns is able to achieve the most power savings with smart use of both line card and port low power state. Also, note that the $LC$ policy can also save considerable amount of power. This indicates that line card sleep state accounts for a large portion of power saving in DCN. And this conclusion can also be validated from the observation that the $SP$ policy saves less than 1\% power no matter what job placement scheme is used.
	Figure~\ref{fig:dnspower} shows the power saving corresponding to the execution of 2000 DNS jobs, compared to the baseline policies. In our experiment setup, if all the line cards and ports remain active, the switch power is 398.76$W$. We can see that for each configuration, the avaerage power of Popcorns is 233$\sim$312$W$, namely Popcorns is able to achieve approximately 18\%$\sim$39\% network power savings, while the baseline policy also saves 20\%$\sim$34\% network power with smart use of both line card and port low power state, compared to no power management on line cards and ports at all.
	
	Additionally, we can see that on the server side, using the Cooperative Network-Server Algorithm~\ref{algorithm2}, Popcorns further consumes approximately 19\%$\sim$22\% less power than the Server-Balanced Algorithm. There is no power saving on the servers for the latter algorithm, since all the servers are kept active, the power of which is 92$W$~\ref{Serverpowermodel}. In this sense, we can conclude that intelligently scheduling tasks based on their interdependence and system status, together with the use of server C6 package sleep state further saves more power.
	%We note that network power saving percentage decreases with increasing system utilization, which is due to less line card, port, and server low power state time. Actually our extensive experiments show that the network power saving percentage difference between two algorithms converges to 5\% as job arrival rate keeps increasing to alarge value (e.g. 2000 tasks/sec).
	%Figure~\ref{fig:converge} in the last section shows that the network power saving percentage difference between two algorithms converges to 6.5\% with utilization rate keeps increasing. 
	%{\color{red}FY: the evaluation looks weak on the server power management side. Need more discussion on the server power management scheme and the benefit of server low power state}
	
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Global Foresight Algorithm]{
	%		\includegraphics[scale=0.18]{figures/powerdnsheu.eps}
	%		\label{fig:powerdnsheu}}
	%	\subfloat[b][Server-Balanced Algorithm]{
	%		\includegraphics[scale=0.18]{figures/powerdnsb.eps}
	%		\label{fig:powerdnsb}}
	%	\vspace{-6pt}
	%	\caption{Power saving results in DNS Service experiment.}
	%	\label{fig:dnspower}
	%	\vspace{-0.16in}
	%\end{figure*}
	%
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Web Service, Utilization=0.1]{
	%		\includegraphics[scale=0.11]{figures/2000jobpoint7uDNS.eps}
	%		\label{fig:google_pp_0.1_90th}}
	%	\subfloat[b][Web Service, Utilization=0.3]{
	%		\includegraphics[scale=0.11]{figures/2000job2uDNS.eps}
	%		\label{fig:google_pp_0.3_90th}}
	%	\subfloat[b][Web Service, Utilization=0.6]{
	%		\includegraphics[scale=0.11]{figures/2000job4uDNS.eps}
	%		\label{fig:google_pp_0.6_90th}}
	%	\vspace{-6pt}
	%	\caption{CDF of job latency when executing 2000 Poisson-arrival DNS jobs under low, medium, and high system utilization respectively.}
	%	\label{fig:dnslatency}
	%	\vspace{-0.16in}
	%\end{figure*}
	
	Figure~\ref{fig:dns_pp_0.1_90th}, ~\ref{fig:dns_pp_0.3_90th}, and ~\ref{fig:dns_pp_0.6_90th} show the CDF of job latency in DNS Service experiment. We can see that the $90^{th}$ percentile job latency is the best under low system utilization, and gradually increases as utilization increases. Prior study~\cite{yao2017wasp} shows that low system utilization is a more practical case in real scenarios. Thus, we note that our proposed power management policy together with job placement algorithm saves a large portion of power in DCN while maintaining the QoS demands.
	
	%Figure~\ref{figure5}, ~\ref{figure6}, ~\ref{figure7} and ~\ref{figure8} show the CDF of job latency when executing 2000 Poisson-arrival jobs with 50, 500, 1000, and 2000 arrival rate by these two algorithms respectively. We can see that no matter the job arrival load is low, medium, or heavy, the job service time is almost the same with two algorithms. And the tail of job latency distribution with Global Foresight Algorithm is only slightly longer than Server-Balanced Placement, which means the delay caused by globally computing each potential path weight can almost be ignored.
	
	%\subsection{Web Search}
	%Figure~\ref{fig:wsearchdraw} and ~\ref{fig:wsearchdag} shows the steps in processing a web search request and its corresponding job DAG. In simulation, we set the flow size to be 10MBytes and average job service time is randomly generated between 20ms and 60ms based on prior studies~\cite{alizadeh2013pfabric}~\cite{hadjilambrou2015characterization}.
	
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Steps in processing a web search request.]{
	%		\includegraphics[scale=0.5]{figures/wsearchdraw.pdf}
	%		\label{fig:wsearchdraw}}
	%	\subfloat[b][Example of a web search job DAG. Task 1 is executed by the master server, while task 2 - 6 are processed by different indexers, and master server needs to communicate with all the indexers.]{
	%		\includegraphics[scale=0.3]{figures/wsearchDAG.eps}
	%		\label{fig:wsearchdag}}
	%	\vspace{-12pt}
	%	\caption{Web search.}
	%	\label{fig:wsearchjob}
	%	\vspace{-0.16in}
	%\end{figure*}
	
	%\begin{figure}
	%	\captionsetup{font=small}
	%	\centering\includegraphics[width=0.2\textwidth]{figures/wsearchDAG.eps}\caption{DAG of web search jobs simulated in our experiment, with random job size between 20ms and 60ms. Task 1 is executed by the master server, while task 2 - 6 are processed by different indexers, and master server needs to communicate with all the indexers}
	%	\label{figure89}
	%\end{figure}
	
	\subsubsection{Web Search}
	Figure~\ref{fig:ws-graph} shows the steps in processing a web search request and its corresponding job DAG. In simulation, we set the flow size to be 100MB, and average job service time is randomly generated between 20ms and 60ms based on prior studies~\cite{alizadeh2013pfabric}~\cite{hadjilambrou2015characterization}. Thus, the average web search task size is 10ms$\sim$30ms in our job model.
	%{\color{blue} FY: more discussion needed. mention actual numbers}
	
	\begin{figure*}
	\centering
	\captionsetup{font=small}
	\subfloat[Web search average power]{
	\centering\includegraphics[scale=0.1]{figures/powerwsearch.pdf}
	\label{fig:wsearchpower}
	}
	\subfloat[b][Web search latency, Utilization=0.1]{
	\includegraphics[scale=0.1]{figures/wsearchp1-0.pdf}
	\label{fig:ws.1_90th}
	}
	\subfloat[b][Web search latency, Utilization=0.3]{
	\includegraphics[scale=0.1]{figures/wsearchp3-0.pdf}
	\label{fig:ws_pp_0.3_90th}
	}
	\subfloat[b][Web search latency, Utilization=0.6]{
	\includegraphics[scale=0.095]{figures/wsearchp6-0.pdf}
	\label{fig:ws_pp_0.6_90th}
	}
	
	\caption{DCN executes 2000 Poisson-arrival web search jobs under low, medium, and high system utilization respectively. Suffix $-CNS$ represents Cooperative Network-Server Algorithm and $-SB$ denotes Server-Balanced Algorithm.}
	\label{fig:ws-exp}
	\end{figure*}
	
	\begin{figure*}
	\centering
	\captionsetup{font=small}
	\subfloat[Web service average power]{
	\centering\includegraphics[scale=0.1]{figures/powerws.pdf}
	\label{fig:wsvpower}
	}
	\subfloat[b][Web service latency, Utilization=0.1]{
	\includegraphics[scale=0.1]{figures/wsp1-0.pdf}
	\label{fig:wsv_pp_0.1_90th}
	}
	\subfloat[b][Web service latency, Utilization=0.3]{
	\includegraphics[scale=0.1]{figures/wsp3-0.pdf}
	\label{fig:wsv_pp_0.3_90th}
	}
	\subfloat[b][Web service latency, Utilization=0.6]{
	\includegraphics[scale=0.095]{figures/wsp6-0.pdf}
	\label{fig:wsv_pp_0.6_90th}
	}
	\caption{DCN executes 2000 Poisson-arrival web service jobs under low, medium, and high system utilization respectively. Suffix $-CNS$ represents Cooperative Network-Server Algorithm and $-SB$ denotes Server-Balanced Algorithm.}
	\label{fig:wsv-exp}
	\end{figure*}
\todo{update all diagrams}
	Figure~\ref{fig:wsearchpower} shows the power saving corresponding to the execution of 2000 DNS jobs, compared to the baseline policies. We can see that for each configuration, Popcorns is able to achieve $\sim$42\% network power savings under high system utilization rate, and even with low utilization, $\sim$16\% network power savings is achieved. As for the Server-Balanced case, the numbers are 33\% and 18\% respectively, which demonstrates the benefits of smart use of low power states of switch components.
	
	What is more, on the server side, Popcorns further saves approximately $\sim$13\% power than the Server-Balanced Agorithm, which has no power saving on the servers. The results are basically in accordance with the previous DNS experiment.
	%Figure~\ref{fig:converge} in the last section shows that the network power saving percentage difference between two algorithms converges to 6.5\% with utilization rate keeps increasing. 
	%{\color{red}FY: the evaluation looks weak on the server power management side. Need more discussion on the server power management scheme and the benefit of server low power state}
	
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Global Foresight Algorithm]{
	%		\includegraphics[scale=0.18]{figures/powerdnsheu.eps}
	%		\label{fig:powerdnsheu}}
	%	\subfloat[b][Server-Balanced Algorithm]{
	%		\includegraphics[scale=0.18]{figures/powerdnsb.eps}
	%		\label{fig:powerdnsb}}
	%	\vspace{-6pt}
	%	\caption{Power saving results in DNS Service experiment.}
	%	\label{fig:dnspower}
	%	\vspace{-0.16in}
	%\end{figure*}
	%
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Web Service, Utilization=0.1]{
	%		\includegraphics[scale=0.11]{figures/2000jobpoint7uDNS.eps}
	%		\label{fig:google_pp_0.1_90th}}
	%	\subfloat[b][Web Service, Utilization=0.3]{
	%		\includegraphics[scale=0.11]{figures/2000job2uDNS.eps}
	%		\label{fig:google_pp_0.3_90th}}
	%	\subfloat[b][Web Service, Utilization=0.6]{
	%		\includegraphics[scale=0.11]{figures/2000job4uDNS.eps}
	%		\label{fig:google_pp_0.6_90th}}
	%	\vspace{-6pt}
	%	\caption{CDF of job latency when executing 2000 Poisson-arrival DNS jobs under low, medium, and high system utilization respectively.}
	%	\label{fig:dnslatency}
	%	\vspace{-0.16in}
	%\end{figure*}
	
	Figure~\ref{fig:ws.1_90th}, ~\ref{fig:ws_pp_0.3_90th}, and ~\ref{fig:ws_pp_0.6_90th} show the CDF of job latency in the Web Search experiment. We can see that the $90^{th}$ percentile job latency is also the best under low system utilization, and gradually increases with utilization rate getting higher. 
	%Thus, we can note that our proposed power management policy together with job placement algorithm saves a large portion of power in DCN while maintaining the QoS demands.
	
	%Figure~\ref{figure5}, ~\ref{figure6}, ~\ref{figure7} and ~\ref{figure8} show the CDF of job latency when executing 2000 Poisson-arrival jobs with 50, 500, 1000, and 2000 arrival rate by these two algorithms respectively. We can see that no matter the job arrival load is low, medium, or heavy, the job service time is almost the same with two algorithms. And the tail of job latency distribution with Global Foresight Algorithm is only slightly longer than Server-Balanced Placement, which means the delay caused by globally computing each potential path weight can almost be ignored.
	
	%\subsection{Web Search}
	%Figure~\ref{fig:wsearchdraw} and ~\ref{fig:wsearchdag} shows the steps in processing a web search request and its corresponding job DAG. In simulation, we set the flow size to be 10MBytes and average job service time is randomly generated between 20ms and 60ms based on prior studies~\cite{alizadeh2013pfabric}~\cite{hadjilambrou2015characterization}.
	
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Steps in processing a web search request.]{
	%		\includegraphics[scale=0.5]{figures/wsearchdraw.pdf}
	%		\label{fig:wsearchdraw}}
	%	\subfloat[b][Example of a web search job DAG. Task 1 is executed by the master server, while task 2 - 6 are processed by different indexers, and master server needs to communicate with all the indexers.]{
	%		\includegraphics[scale=0.3]{figures/wsearchDAG.eps}
	%		\label{fig:wsearchdag}}
	%	\vspace{-12pt}
	%	\caption{Web search.}
	%	\label{fig:wsearchjob}
	%	\vspace{-0.16in}
	%\end{figure*}
	
	%\begin{figure}
	%	\captionsetup{font=small}
	%	\centering\includegraphics[width=0.2\textwidth]{figures/wsearchDAG.eps}\caption{DAG of web search jobs simulated in our experiment, with random job size between 20ms and 60ms. Task 1 is executed by the master server, while task 2 - 6 are processed by different indexers, and master server needs to communicate with all the indexers}
	%	\label{figure89}
	%\end{figure}
	
	%\subsection{Web Service}
	%Figure~\ref{fig:wsdraw} and ~\ref{fig:wsdag} shows the process of a web service response and its corresponding job DAG. In simulation, we set the flow size to be 10MBytes and average job service time is randomly generated between 2ms and 10ms based on prior studies~\cite{wu2013adaptive}~\cite{meisner2009powernap}.
	
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Steps in processing a web service request.]{
	%		\includegraphics[scale=0.6]{figures/wsdraw.pdf}
	%		\label{fig:wsdraw}}
	%	\subfloat[b][Example of a web service job DAG. Task 1 is executed by the application server, while task 2 is assigned to be processed by database server, and task 3 is executed by backup server.]{
	%		\includegraphics[scale=0.4]{figures/wsDAG.pdf}
	%		\label{fig:wsdag}}
	%	\vspace{-6pt}
	%	\caption{Web service.}
	%	\label{fig:wsjob}
	%	\vspace{-0.16in}
	%\end{figure*}
	%\begin{figure}
	%	\captionsetup{font=small}
	%	\centering\includegraphics[width=0.3\textwidth]{figures/wsdraw.pdf}\caption{Process of a web service request.}
	%	\label{figure80}
	%\end{figure}
	%
	%\begin{figure}
	%	\captionsetup{font=small}
	%	\centering\includegraphics[width=0.2\textwidth]{figures/wsDAG.pdf}\caption{DAG of web service jobs simulated in our experiment, with random job size between 2ms and 10ms.. Task 1 is executed by the application server, while task 2 is assigned to database server, and task 3 is executed by backup server.}
	%	\label{figure79}
	%\end{figure}
	
	\subsubsection{Web Service}
	Figure~\ref{fig:wsv-graph} shows the process of a web service response and its corresponding job DAG. In simulation, we set the flow size to be 100MB, and average job service time is randomly generated between 2ms and 10ms based on prior studies~\cite{wu2013adaptive}~\cite{meisner2009powernap}. Therefore, the average web service task size is 1ms$\sim$5ms in our job model.
	
	
	%\begin{figure}
	%	\captionsetup{font=small}
	%	\centering\includegraphics[width=0.45\textwidth]{figures/powerws.pdf}\caption{Power saving results in Web Service job experiment.}
	%	\label{fig:wspower}
	%\end{figure}
	
	%\begin{figure*}[htbp]
	%	\centering
	%	\captionsetup{font=small}
	%	\subfloat[b][Web Service, Utilization=0.1]{
	%		\includegraphics[scale=0.13]{figures/wsp1.pdf}
	%		\label{fig:google_pp_0.1_90th}}
	%	\subfloat[b][Web Service, Utilization=0.3]{
	%		\includegraphics[scale=0.13]{figures/wsp3.pdf}
	%		\label{fig:google_pp_0.3_90th}}
	%	\subfloat[b][Web Service, Utilization=0.6]{
	%		\includegraphics[scale=0.13]{figures/wsp6.pdf}
	%		\label{fig:google_pp_0.6_90th}}
	%	\vspace{-6pt}
	%	\caption{CDF of job latency when executing 2000 Poisson-arrival Web service jobs under low, medium, and high system utilization respectively.}
	%	\label{fig:wslatency}
	%	\vspace{-0.16in}
	%\end{figure*}
	
	Figure~\ref{fig:wsv-exp} shows the power consumption for the execution of 2000 web service jobs, which further reinforce the conclusion of previous experiment and priority of our proposed algorithms. We can see that for a DCN executing small-sized jobs like \emph{web service}, smart use of server sleep state also saves $\sim$7\% power. And two configuration both achieve  $\sim$27\% network power saving under three system utilization.
	
	%(29\%$\sim$33\%) compared to medium- and large-sized workload shown in Figure~\ref{fig:dnspower} and ~\ref{fig:wsearchpower}.
	% {\color{blue} FY: more discussion needed. mention actual numbers}
	
	%\begin{figure}
	%	\captionsetup{font=small}
	%	\centering\includegraphics[width=0.35\textwidth]{figures/power.pdf}\caption{Power consumption comparison.}
	%	\label{fig:converge}
	%\end{figure}
	
	%The power saving percentage shown in figure~\ref{figure4} is obtained by running our proposed Global Foresight Algorithm~\ref{algorithm2}, Server-Balanced Algorithm~\ref{algorithm3}, and random placement algorithm under three power management policies above respectively. We are dynamicly generating 2000 jobs subject to Poisson arrival in the DCN, and the DAG of each job is shown in figure~\ref{figure11}. Y-axis here represents the power saving percentage compared to no power management at all, and x-axis is the job arrival rate. Since the performance of random placement is unstable and can result in extremely worst or best power saving, we take and show the average case.
	
	%\begin{figure}
	%	\captionsetup{font=small}
	%	\centering\includegraphics[width=0.5\textwidth]{figures/power.eps}\caption{Power consumption comparison.}
	%	\label{figure4}
	%\end{figure}
	
	%We can see that for each algorithm, the power management policy proposed in algorithm~\ref{algorithm1} with smart use of both line card and port low power state saves the most power, and is just slightly larger than power saving of $LC$ policy, which means line card sleep state does account for a large portion of power saving in DCN. And this conclusion can also be proved by the results that the $SP$ policy saves less than 1\% power no matter what job placement algorithm is used.
	
	%From another aspect to compare three job placement algorithms, we can see that our proposed Global Foresight Algorithm~\ref{algorithm2} saves approximately 6\% power more than Server-Balanced Placement~\ref{algorithm3}, which further saves 8\% power more than Random Placement on average. In this sense, we can conclude that intelligently placing tasks on servers based on their interdependence and system status further saves more power.
	
	%\subsection{Evaluation}
	
	%Figure~\ref{figure4} shows that intelligent job placement algorithms considering task interdependence and network status can further save power in DCN. In this section, we evaluate and compare two algorithms with this property, Global Foresight Algorithm~\ref{algorithm2} and Server-Balanced Placement~\ref{algorithm2}, to see if there is a tradeoff to achieve power saving.
	
	%Figure~\ref{figure5}, ~\ref{figure6}, ~\ref{figure7} and ~\ref{figure8} show the CDF of job latency when executing 2000 Poisson-arrival jobs with 50, 500, 1000, and 2000 arrival rate by these two algorithms respectively. We can see that no matter the job arrival load is low, medium, or heavy, the job service time is almost the same with two algorithms. And the tail of job latency distribution with Global Foresight Algorithm is only slightly longer than Server-Balanced Placement, which means the delay caused by globally computing each potential path weight can almost be ignored.
	
	%To give a comprehensive comparison on performance of these two algorithms, we additionally present their flow completion time and task latency results in figure~\ref{figure9} and ~\ref{figure10}.
\end{comment}


==> 2020-popcorns-T-SUSC (copy)/job_model.tex <==
\subsection{Modeling Job{\color{blue}-------$>$Multi-task v.s. single-task job models}}
We model the execution of jobs at the server side as follows. A job consists of multiple inter-dependent tasks that include both spatial and temporal inter-dependence. Application tasks are typically executed by specific server types. For example, a web service request will first be processed by an application or web server, and a search request is processed by a database server, and this kind of task relationship is called spatial inter-dependence. In terms of temporal inter-dependence, a task cannot start executing until all of its 'parent' tasks have finished their execution, and until after their results have been communicated to the server assigned to the task. A job is considered to have finished when all of its tasks finish execution. As for servers, there are multiple cores per server and one core can only process one task. In this paper, we configure single-core processor for the servers.

Each job $j$ can be represented as a directed acyclic graph (DAG) $G^j(V^j, E^j)$, where $V^j$ is the set of tasks of job $j$. In DAG, if there is a link from task $i$ to task $r$, then task $i^j$ must finish and communicate its results to task $r^j$ before $r^j$ can start processing. Each task $v^j \in V^j$ has a workload requirement, namely task size or execution time requirement $w^j_v$ for the core. For each link in $E^j$, there is a data transfer size $D^j_l$ associated with it, which denotes the bandwidth requirement to transfer the result over link $l$ (from the task at the head of DAG link to the task at the tail) when assigned a network flow. Figure~\ref{figure1} shows an example of a job DAG.

%\begin{figure}[htbp]
%	\captionsetup{font=small}
%	\centering
%	\vspace{-0.1in}
%	\includegraphics[scale=1.0]{./figures/wsDAG.eps}
%	\caption[test]{Example of a web service job DAG. Task 1 is executed by the application server, while task 2 is assigned to be processed by database server.\protect\footnotemark}
%	\label{fig:wsDAG}
%	\vspace{-0.1in}
%\end{figure}

\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.15\textwidth]{figures/DAG.pdf}\caption{Example of a job DAG. Numbers 1-6 denote task 1-task 6 respectively. Numbers around the tasks represent task size, while numbers on the links represent flow size.}
	\label{figure1}
\end{figure}

\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.5\textwidth]{figures/fat_tree.png}
	\caption{Fat tree topology.}
	\label{figure12}
\end{figure}

==> 2020-popcorns-T-SUSC (copy)/motivation.tex <==
%\section{Motivation}
%

%{\bf GV: Doesn't look very relevant to motivation. Move this to related work, and this section may be removed.}
\subsection{Need for Switch sleep states}
\label{sec:motivation}
In this section, we motivate the need for having more sleep states in switches. As discussed in sections \ref{sec:transition} and \ref{sec:switchpower}, the switch power consumption can be temporarily reduced by selectively turning off parts of the line cards and woken up when required. For components which do not have any memory or state the wakeup latency is the time it takes to initialize the system. For other components such as DRAM storing address forwarding tables should be reinitialized from the host line cards. In our study, we find that having multiple sleep states for the switch helps in trade-off various levels of wake-up latency for energy consumption reduction. This scheme is inherently useful when the idle period is not large enough to accommodate the high wastage of energy spent during waking from a single deepest sleep state and would cause network transmission to get delayed. 

\begin{figure}[!h]
	\captionsetup{font=small}
	\centering\includegraphics[width=0.4\textwidth]{figures/motivation/service.png}\caption{Network Energy consumption normalized per job for a 1024 server FatTree topology network. Jobs containing two dependent tasks of 500ms CPU duration each arrive at 30 Job/second. The Switch sleep state and latency models are constructed using the power model defined in section~\ref{sec:switchpower}.} %{\bf GV- make it a bit more descriptive with type of job, sleep states and what y-axis captures.{\color{green}DONE}}}
	\label{motivation12}
\end{figure}
%
%\begin{figure}
%	\captionsetup{font=small}	\centering\includegraphics[width=0.8\textwidth]{figures/motivation/search.png}\caption{Total Energy per job}
%	\label{Search Workload}
%\end{figure}


 


==> 2020-popcorns-T-SUSC (copy)/problemstatement.tex <==
\section{Design}
\subsection{Problem Definition}
\label{sec:problem solution}
In this section, we formulate the joint server and data center network power
optimization as a constrainted optimization problem using the switch power model
and job model defined above. First, to obtain the power consumption of a switch
$k$, assume the number of active line cards and ports are $\zeta^{active}_k$ and
$\rho^{active}_k$ respectively, and the number of line cards in respective sleep states and ports in LPI mode are $\zeta^{sleep}_k$ and $\rho^{LPI}_k$ respectively. Since the total power of a switch is the sum of base power $P_k^{base}$, power of ports, and power of line cards, then we have $P_k^{switch}=P_k^{base}+\zeta^{active}_k*P_{line card}^{active}+\rho^{active}_k*P_{port}^{active}+\zeta^{sleep}_k*P^{sleep}_{line card}+\rho^{LPI}_k*P_{port}^{LPI}$.
To calculate the power consumption of server $i$, since our system consideres the core as basic processing unit in server, the total power of a server is the sum of idle power $P_i^{idle}$ and dynamic power which is linear in the number of active cores $C_i^{on}$. Then we have $P_i^{server}=P_i^{idle}+C_i^{on}*P_{core}^{on}$, where $P_{core}^{on}$ denotes the power consumed by an active core. 
%First, to obtain the power consumption of a switch $k$, assume the number of active line cards and ports are $L^{active}_k$ and $P^{active}_k$ respectively, and the number of line cards in sleep state and ports in LPI mode are $L^{sleep}_k$ and $P^{LPI}_k$ respectively. Since the total power of a switch is the sum of base parts power, ports power, and line cards power, then we have $P_k^{switch})=P_k^{base}+L^{active}_k*P_{line card}^{active}+P^{active}_k*P_{port}^{active}+L^{sleep}_k*P^{sleep}_{line card}+P^{LPI}_k*P_{port}^{LPI}$. To calculate the power consumption of server $i$, since our system models the core in server as basic processing unit, the we have $P_i^{server}=P_i^{idle}+C_i^{on}*P_{core}^{on}$. The total power of a server is the sum of idle power and dynamic power, and the dynamic power is linear to the number of active cores, in other words, if the core is turned off, the power is 0.

Then the joint power optimization problem can be formulated as minimize
$\sum_{k=1}^{N_{switch}}{P_k^{switch}}+\sum_{i=1}^{N_{server}}{P_i^{server}}$
under both network-side and serve-side constraints, such as link capacity,
computation resources, etc.



\begin{table*}
	\centering
	\scriptsize
	\caption{Estimating the energy consumption}
	\label{tab:estimatingenergy}
	\arrayrulecolor{black}
	\begin{tabular}{|l|l|l|} 
		\hline
		\multicolumn{2}{|c|}{\textbf{Energy Component} }                                                                                                                                                                                         & \textbf{Description}                                                                                                                                                                                        \\ 
		\hline
		\multicolumn{3}{|l|}{\textbf{~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ Server Energy} }                                                                                                                                                                                                                                                                                                                                \\ 
		\hline
		\multirow{2}{*}{\textbf{Candidate server} }                                                                              & Server Task Execution Energy                                                                                  & Energy consumed when the task is being executed                                                                                                                                                             \\ 
		\arrayrulecolor[rgb]{0.651,0.651,0.651}\cline{2-3}
		& Server waiting for tranmission                                                                                & Energy consumed when the task is waiting for communication to complete.                                                                                                                                     \\ 
		\hline
		\multirow{3}{*}{\textbf{Server (If sleeping)} }                                                                          & Wakeup Energy during transistion                                                                              & Energy spent during wakeup.                                                                                                                                                                                 \\ 
		\cline{2-3}
		& Core Energy savings loss Sleep                                                                                & If sleeping, Energy savings loss due to Active state                                                                                                                                                        \\ 
		\cline{2-3}
		& Package Energy savings loss Sleep                                                                             & If the first core being woken up, CPU package sleep savings loss.                                                                                                                                           \\ 
		\arrayrulecolor{black}\hline
		\multicolumn{3}{|l|}{\textbf{~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~ ~Network Energy} }                                                                                                                                                                                                                                                                                                                                  \\ 
		\hline
		\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{For Each Switch in the }\\\textbf{candidate flow path} \end{tabular}} & \begin{tabular}[c]{@{}l@{}}Network Energy cost based \\on Bandwidth-allocated \end{tabular}                   & \begin{tabular}[c]{@{}l@{}}Every flow is allocated a BW based on the network congestion and~\\link capacity of the entire flow path,~flow's minimum bandwidth \\the requirement to meet QoS. \end{tabular}  \\ 
		\arrayrulecolor[rgb]{0.651,0.651,0.651}\cline{2-3}
		& Wakeup Energy during transistion                                                                              & Energy spent to transistion to active state                                                                                                                                                                 \\ 
		\cline{2-3}
		& Line card Active energy                                                                                       & If the Linecard is sleeping, the energy cost is the full active power consumption.                                                                                                                          \\ 
		\hline
		\begin{tabular}[c]{@{}l@{}}\textbf{For Every flow in common }\\\textbf{path of the candidate path} \end{tabular}         & \begin{tabular}[c]{@{}l@{}}Energy savings due to decreased \\Bandwidth for the every other flow \end{tabular} & \begin{tabular}[c]{@{}l@{}}For every other switch in the current flow path whose BW is reduced,\\calculate the energy spent on it. \end{tabular}                                                            \\
		\arrayrulecolor{black}\hline
	\end{tabular}
\end{table*}

% \begin{sidewaystable}[!htp]\centering
% \caption{Energy estimation for candidate server and flow path selection}\label{tab: }
% \scriptsize
% \begin{tabular}{lrrr}\toprule
% \multicolumn{2}{c}{\textbf{Energy Component}} &\textbf{Description} \\\midrule
% \multirow{2}{*}{\textbf{Server Energy }} &Server Task Execution Energy &Energy consumed when the task is being executed \\
% &Server waiting for tranmission &Energy consumed when the task is scheduled and is waiting for completion \\
% \multirow{3}{*}{\textbf{Server (If sleeping)}} &Wakeup Energy during transistion &Energy spent during wakeup. \\
% &Core Energy savings loss Sleep &If sleeping, Energy savings loss due to Active state \\
% &Package Energy savings loss Sleep &If first core being wokenup, CPU package sleep savings loss. \\
% \textbf{} & & \\
% \textbf{Network Energy} & & \\
% \multirow{3}{*}{\textbf{For Each Switch in the candidate flow path}} &Network Energy cost based on BW-allocated &Every flow is allocated a BW based on the network congestion and link capacity of the entire flow path, flow's minimum bandwidth requirement to meet QoS. \\
% &Wakeup Energy during transistion &Energy spent to transistion to active state \\
% &Line card Active energy &If the Linecard is sleeping, the energy cost is the full active power consumption. \\
%  \textbf{For Every flow in common path of the candidate path} &Energy savings due
%                                                                  to decreased BW
%                                                                  for the every
%                                                                  other flow &For
%                                                                               every
%                                                                               other
%                                                                               switch
%                                                                               in
%                                                                               the
%                                                                               current
%                                                                               flow
%                                                                               path
%                                                                               whose
%                                                                               BW
%                                                                               is
%                                                                               reduced,
%                                                                               calculate
%                                                                               the
%                                                                               increased
%                                                                               energy
%                                                                               spent
%                                                                               on
%                                                                               it. \\
% \bottomrule
% \end{tabular}
% \end{sidewaystable}

% \begin{table}[!htp]\centering
% \caption{Generated by Spread-LaTeX}\label{tab: }
% \scriptsize
% \begin{tabular}{lrrr}\toprule
% \multirow{2}{*}{\textbf{Server Energy}} &Server Task Execution Energy &Energy consumed when the task is being executed \\\midrule
% &Server waiting for tranmission &Energy consumed when the task is scheduled and is waiting for completion \\
% \multirow{3}{*}{\textbf{Server (If sleeping)}} &Wakeup Energy during transistion &Energy spent during wakeup. \\
% &Core Energy savings loss Sleep &If sleeping, Energy savings loss due to Active state \\
% &Package Energy savings loss Sleep &If first core being wokenup, CPU package sleep savings loss. \\
% \textbf{} & & \\
% \textbf{Network Energy} & & \\
% \multirow{3}{*}{\textbf{For Each Switch in the candidate flow path}} &Network Energy cost based on BW-allocated &Every flow is allocated a BW based on the network congestion and link capacity of the entire flow path, flow's minimum bandwidth requirement to meet QoS. \\
% &Wakeup Energy during transistion &Energy spent to transistion to active state \\
% &Line card Active energy &If the Linecard is sleeping, the energy cost is the full active power consumption. \\
% \textbf{For Every flow in common path of the candidate path} &Energy savings due to decreased BW for the every other flow &For every other switch in the current flow path whose BW is reduced, calculate the increased energy spent on it. \\
% \bottomrule
% \end{tabular}
% \end{table}

%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{table}[!htp]\centering
% % \begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb] %
% \caption{Generated by Spread-LaTeX}\label{tab: }
% \scriptsize
% \begin{tabular}{|l|l|r}\toprule
% \multicolumn{2}{c}{\textbf{Energy Component}} &\textbf{Description} \\\midrule
% \multirow{2}{*}{\textbf{Server Energy}} &Server Task Execution Energy &Energy consumed when the task is being executed \\
% &Server waiting for tranmission &Energy consumed when the task is scheduled and is waiting for completion \\
% \multirow{3}{*}{\textbf{Server (If sleeping)}} &Wakeup Energy during transistion &Energy spent during wakeup. \\
% &Core Energy savings loss Sleep &If sleeping, Energy savings loss due to Active state \\
% &Package Energy savings loss Sleep &If first core being wokenup, CPU package sleep savings loss. \\
% \textbf{} & & \\
% \textbf{Network Energy} & & \\
% \multirow{3}{*}{\textbf{For Each Switch in the candidate flow path}} &Network Energy cost based on BW-allocated &Every flow is allocated a BW based on the network congestion and link capacity of the entire flow path, flow's minimum bandwidth requirement to meet QoS. \\
% &Wakeup Energy during transistion &Energy spent to transistion to active state \\
% &Line card Active energy &If the Linecard is sleeping, the energy cost is the full active power consumption. \\
% \textbf{For Every flow in common path of the candidate path} &Energy savings due to decreased BW for the every other flow &For every other switch in the current flow path whose BW is reduced, calculate the increased energy spent on it. \\
% \bottomrule
% \end{tabular}
% \end{table}
% % \end{threeparttable}\end{adjustwidth}

==> 2020-popcorns-T-SUSC (copy)/switchpower.tex <==
Switch operates as OSI layer 2 network device, forwarding data frame from source
port to destination port and a router works at layer 3 for routing interdomain
network communication. A modular commercial switch such as the CISCO nexus line of switches consists of the following components:

\begin{itemize}
	\item \textit{Switch Chassis}: It houses the switch backplane, where all the
    modules are connected, power and cooling components. The chassis can also
    contain a variable number of configurable modules containing network
    interfaces and management modules.
	\item \textit{Modules}: There can two kinds: Supervisor and I/O modules. The supervisor modules contains the decision making components of the switch, and I/O modules such as linecard where network ports are connected.
\end{itemize}

Due to lack of detailed power models for commercial switches, we propose and
derive our switch power model based on available literature,
~\cite{panZerotimeWakeupLine2016} and corroborating with the cisco power
calculator~\cite{CiscoPowerCalculator} for Nexus line of switches, and tools
such as Cacti ~\cite{balasubramonianCACTINewTools2017}  Micron power modeling tools~\cite{MicronMemoryPower}.


\subsubsection{Supervisor modules}
As shown in figure ~\ref{figure13}, the control pane where all
forwarding decisions is performed by the SUP(Supervisor) module which consists
of the Route Processor (OSI layer 3 function) and Switch Processing card(OSI
layer 2 functions).
The CISCO SUP2E contains DRAM upto 32GB(Core switches).
According to Cisco power calculator~\cite{CiscoPowerCalculator}, a routing
processor card consumes upto 69W. We breakdown the components of the route
processing card in table ~\ref{tab:switchchassis}.

\subsubsection{Line Card power Model}
A linecard consists of several components such as ASICs, TCAMs, DRAM memory, and ports. Our power model for each component is explained below:

Due to lack of detailed power models for commercial switches, we propose and
derive our switch power model based on available literature and memory power
modeling tools from Micron~\cite{MicronMemoryPower}. A switch used in production uses
the several components such as ASICs, TCAMs, DRAM memory, and ports. Our power model for each component is explained below:


\label{sec:switcharch}
\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=1.2\linewidth]{figures/Switcharch.png}\caption{Illustration of Switch architecture.}	\label{figure13}
\end{figure}

%\begin{table*}[!htp]\centering
%	\caption{Linecard Power model}\label{tab:linecardpower}
%	\scriptsize 
%	\begin{tabularx}{480pt}{|X|X|X|X|X|X|}\toprule
%		&\textbf{Active} &\textbf{Data-plane low power state1)} &\textbf{Low power state 2} &\textbf{Low Power state 3} &\textbf{Line Card Off} \\\midrule
%		Packet Forwarding\\(Forwarding and replication Engines) &165 &132 &66 &33 &0 \\
%		&\cellcolor[HTML]{d9d9d9}Active-Max Clock frequency &\cellcolor[HTML]{d9d9d9}DVFS savings for the network
%                       processor &\cellcolor[HTML]{d9d9d9} Clock gating the
%                                   lookup caches in the forwarding engines,
%                                   Replication engines clock gated.
%                                  &\cellcolor[HTML]{d9d9d9} Forwarding engine's Core clock and bus stopped.
%                                  &\cellcolor[HTML]{d9d9d9} Architectural state flushed to DRAM and Forwarding engine and replication engine aare powergated.\\
%		VoQ (M) (INPUT + OUTPUT)(max) &15.5+2 x 6 mW per MB of flow &15.5+1 x 6mW per MB flow &4 &0 &0 \\
%		&\cellcolor[HTML]{d9d9d9}Both Input and Output buffers active &\cellcolor[HTML]{d9d9d9}Output VoQ buffer turned off &\cellcolor[HTML]{d9d9d9}DRAM clock gated and contents lost. &\cellcolor[HTML]{d9d9d9}DRAM Power gated &\cellcolor[HTML]{d9d9d9}DRAM power gated \\
%		TCAM(max) &12W+2.6 mW per MB of flow &12W+2.6 mW per MB of flow &12W+2.6 mW per MB of flow &12 &0 \\
%		&\cellcolor[HTML]{d9d9d9}TCAM active and synchronised &\cellcolor[HTML]{d9d9d9}TCAM Active and synchronised &\cellcolor[HTML]{d9d9d9}TCAM active and synchronised &\cellcolor[HTML]{d9d9d9}TCAM stop synchronized, and clock gated. &\cellcolor[HTML]{d9d9d9}TCAM-routing tables flushed and power gated \\
%		Interconnect Fabric interface &23 &23 &23 &0 &0 \\
%		&\cellcolor[HTML]{d9d9d9}Active for Control plane operations &\cellcolor[HTML]{d9d9d9}Active for Control plane operations &\cellcolor[HTML]{d9d9d9}Active for Control plane operations &\cellcolor[HTML]{d9d9d9}Power gated: Control plane operation stopped &\cellcolor[HTML]{d9d9d9}Power gated: Control plane operation stopped \\
%		Host Processor &24 &22 &9 &9 &3 \\
%		&\cellcolor[HTML]{d9d9d9}Active and running LineCard OS &\cellcolor[HTML]{d9d9d9}Active and running LineCard OS, with DVFS &\cellcolor[HTML]{d9d9d9}C3 state. Halt mode &\cellcolor[HTML]{d9d9d9}C3 state. Halt mode &\cellcolor[HTML]{d9d9d9}C5 state: deeper sleep state \\
%		Ports &29 &15 &4 &4 &4 \\
%		&\cellcolor[HTML]{d9d9d9}All 24 ports active &\cellcolor[HTML]{d9d9d9}Output ports in Low Power Idle- Wake on Arrival &\cellcolor[HTML]{d9d9d9}All ports in Low Power Idle- Wake on Arrival &\cellcolor[HTML]{d9d9d9}All ports in Low Power Idle- Wake on Arrival &\cellcolor[HTML]{d9d9d9}All ports in Low Power Idle- Wake on Arrival \\
%		\textbf{(Power Consumption at full Utilization 1Gbps)} &\textbf{310} &\textbf{250} &\textbf{151} &\textbf{45} &\textbf{7} \\
%		\bottomrule
%	\end{tabularx}
%\end{table*}



\begin{table*}
	\centering
	\small
	\setlength{\extrarowheight}{0pt}
	\addtolength{\extrarowheight}{\aboverulesep}
	\addtolength{\extrarowheight}{\belowrulesep}
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\caption{Single Linecard Power model for an Edge level Switch with 1 Gbps maximum bandwidth}
	\label{tab:linecardpower}
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{llllll} \toprule
			& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Active }\\\textbf{(1 Gbps~Bandwidth )}\end{tabular}} & \textbf{Low power state 1} & \textbf{Low power state 2} & \textbf{Low Power state 3} & \begin{tabular}[c]{@{}l@{}}\textbf{Line Card~ -}\\\textbf{Deepest Sleep State~}\end{tabular} \\ \hline
			\begin{tabular}[c]{@{}l@{}}Packet Forwarding\\~(Forwarding and \\replication Engines)\end{tabular} & 165W & 132W & 66W & 33W & 0W \\
			\rowcolor[rgb]{0.882,0.882,0.882}  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Active-Max Clock\\frequency\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}DVFS savings for\\the network processor.\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Clock gating the\\lookup~caches in\\the forwarding\\engines, Replication\\engines clock gated.\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Forwarding engine's \\Core clock and bus \\stopped.\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Architectural state\\flushed to DRAM\\and Forwarding\\engine and replication\\engines are power gated.\end{tabular} \\
			\begin{tabular}[c]{@{}l@{}}VoQ (M)\\(INPUT + OUTPUT)(max)\end{tabular} & \begin{tabular}[c]{@{}l@{}}15.5W +\\2 x 6 mW per MB of flow\end{tabular} & \begin{tabular}[c]{@{}l@{}}15.5W+\\1 x 6mW per MB flow\end{tabular} & 4W & 0 W & 0 W \\
			\rowcolor[rgb]{0.882,0.882,0.882}  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Both Input and\\Output buffers active\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Output VoQ buffer\\turned off\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}DRAM clock gated\\and contents lost.\end{tabular} & DRAM Power gated & DRAM power gated \\
			TCAM(max) & \begin{tabular}[c]{@{}l@{}}12W+ \\2.6 mW per MB of flow\end{tabular} & \begin{tabular}[c]{@{}l@{}}12W+2.6 mW per MB\\of flow\end{tabular} & \begin{tabular}[c]{@{}l@{}}12W+2.6 mW per MB\\of flow\end{tabular} & 12W & 0W \\
			\rowcolor[rgb]{0.882,0.882,0.882}  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}TCAM active and\\synchronized\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}TCAM Active and\\synchronized\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}TCAM active and\\synchronized\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}TCAM stopped,\\synchronized,\\and clock gated.\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}TCAM-routing\\tables flushed and\\power gated\end{tabular} \\
			Interconnect Fabric interface & 23W & 23W & 23W & 0 W & 0 W \\
			\rowcolor[rgb]{0.882,0.882,0.882}  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Active for Control\\plane operations\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Active for Control\\plane operations\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Active for Control\\plane operations.\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Power gated,\\Control plane\\operation stopped\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Power gated,\\Control plane\\operation stopped\end{tabular} \\
			Host Processor & 24 W & 22 W & 9 W & 9 W & 3 W \\
			\rowcolor[rgb]{0.882,0.882,0.882}  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Active and running\\Linecard OS\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Active and running\\Linecard OS, with\\DVFS\end{tabular} & C3 state. Halt mode. & C3 state. Halt mode & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}C5 state: deeper\\sleep state\end{tabular} \\
			Ports & 29 W & 15W & 4 W & 4 W & 4 W \\
			\rowcolor[rgb]{0.882,0.882,0.882}  & All 24 ports active & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}Output ports in Low\\Power Idle- Wake on Arrival\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}All ports in Low\\Power Idle-Wake\\on Arrival\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}All ports in Low\\Power Idle- Wake on Arrival\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.882,0.882,0.882}}l@{}}All ports in Low\\Power Idle- Wake on Arrival\end{tabular} \\ \hline
			\begin{tabular}[c]{@{}l@{}}\textbf{Max Power Consumption~~}\\\textbf{in each state (}\\\textbf{1 Gbps when active)}\end{tabular} & \textbf{310 W} & \textbf{250 W} & \textbf{151 W} & \textbf{45 W} & \textbf{7 W} \\ \bottomrule
		\end{tabular}
	}
\end{table*}

%\begin{sidewaystable}[!htp]\centering
%	\caption{Line Card Power model}\label{tab: }
%	\scriptsize
%	\begin{tabular}{lrrrrrrr}\toprule
%		&Active &Idle &Sleep State 1 &Sleep state 2 &Line Card Off &References \\\midrule
%		NP (Frequency X) &\cellcolor[HTML]{f4cccc}165.0 &\cellcolor[HTML]{f4cccc}165.0 &\cellcolor[HTML]{fff2cc}66.0 &\cellcolor[HTML]{d9ead3}22.0 &\cellcolor[HTML]{93c47d}0.0 & \\
%		DRAM (M) (INPUT + OUTPUT)(max) &\cellcolor[HTML]{f4cccc}32.5 &\cellcolor[HTML]{fce5cd}22.5 &\cellcolor[HTML]{fff2cc}12.5 &\cellcolor[HTML]{93c47d}0.0 &\cellcolor[HTML]{93c47d}0.0 & \\
%		TCAM(max) &\cellcolor[HTML]{f4cccc}36.5 &\cellcolor[HTML]{f4cccc}36.5 &\cellcolor[HTML]{f4cccc}36.5 &\cellcolor[HTML]{fff2cc}10.0 &\cellcolor[HTML]{93c47d}0.0 & \\
%		Interconnect Fabric interface &\cellcolor[HTML]{f4cccc}23.0 &\cellcolor[HTML]{f4cccc}23.0 &\cellcolor[HTML]{f4cccc}23.0 &\cellcolor[HTML]{93c47d}0.0 &\cellcolor[HTML]{93c47d}0.0 & \\
%		Host Processor &\cellcolor[HTML]{f4cccc}23.9 &\cellcolor[HTML]{f4cccc}23.9 &\cellcolor[HTML]{d9ead3}9.0 &\cellcolor[HTML]{d9ead3}9.0 &\cellcolor[HTML]{93c47d}3.0 & \\
%		Ports &\cellcolor[HTML]{f4cccc}29.0 &\cellcolor[HTML]{fce5cd}14.6 &\cellcolor[HTML]{b6d7a8}3.9 &\cellcolor[HTML]{b6d7a8}3.9 &\cellcolor[HTML]{93c47d}3.9 & \\
%		(Power Consumption at full Utilization) &309.9 &285.5 &150.9 &44.9 &6.9 & \\
%		\bottomrule
%	\end{tabular}
%\end{sidewaystable}
%


%\begin{table}[!htp]\centering
%	\caption{Switch Chassis power model.}\label{tab: }
%	\scriptsize
%	\begin{tabular}{lrrrr}\toprule
%		\textbf{Switch Chassis components} &\textbf{Atleast 1 Line Card Active} &\textbf{All Line Card in OFF state} &\textbf{References} \\\cmidrule{1-4}
%		\textbf{Route processing card} & & & \\\midrule
%		Hostprocessor &\cellcolor[HTML]{fff2cc}23.9 &\cellcolor[HTML]{d9ead3}0 & \\
%		DRAM-3GB &\cellcolor[HTML]{fff2cc}32.5 &\cellcolor[HTML]{d9ead3}0 & \\
%		Persistant Storage() &10 &\cellcolor[HTML]{d9ead3}0 & \\\midrule
%		\textbf{Switch Interconnect card} & & & \\\midrule
%		Switch Fabric and I/0 (40%load) &\cellcolor[HTML]{fff2cc}85 &\cellcolor[HTML]{d9ead3}0 & \\
%		Scheduler ASIC &\cellcolor[HTML]{fff2cc}23.9 &\cellcolor[HTML]{d9ead3}0 & \\\midrule
%		\textbf{Chassis Controller} & & & \\\midrule
%		Host-Processor &\cellcolor[HTML]{fff2cc}24 &\cellcolor[HTML]{fff2cc}24 & \\
%		DRAM-3GB &\cellcolor[HTML]{fff2cc}12 &\cellcolor[HTML]{fff2cc}12 & \\\midrule
%		\textbf{Power Proportional Chassis Components} & & & \\\midrule
%		Power supply losses per Active card (25\%) &\cellcolor[HTML]{fff2cc}93 &\cellcolor[HTML]{d9ead3}5 & \\
%		Cooling per Active Line Card (20\%) &\cellcolor[HTML]{fff2cc}77 &\cellcolor[HTML]{d9ead3}4 & \\
%		\bottomrule
%	\end{tabular}
%\end{table}

% \usepackage{booktabs}


\begin{table}
	\centering
	\scriptsize
	\caption{Switch Chassis power model.}
	\label{tab:switchchassis}
	\begin{tabular}{lll} 
		\toprule
		\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Switch Chassis }\\\textbf{components}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{At-least}\\\textbf{One}\\\textbf{Line card~}\\\textbf{Active}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{All Line }\\\textbf{Cards}\\\textbf{in OFF}\\\textbf{state}\end{tabular}}  \\ 
		\hline
		\multicolumn{3}{c}{\textbf{Route processing card}}                                                                                                                                                                                                                                                                                                                               \\ 
		\hline
		Hostprocessor                                                                                             & 24W                                                                                                                               & 0                                                                                                                                \\
		DRAM-3GB                                                                                                  & 32.5W                                                                                                                             & 0                                                                                                                                \\
		Persistent Storage                                                                                        & 10W                                                                                                                               & 0                                                                                                                                \\ 
		\hline
		\multicolumn{3}{c}{\textbf{\textbf{Switch Interconnect card}}}                                                                                                                                                                                                                                                                                                                   \\ 
		\hline
		Switch Fabric and~~I/0 (40\%load)                                                                         & 85W                                                                                                                               & 0                                                                                                                                \\
		Scheduler ASIC                                                                                            & 24W                                                                                                                               & 0                                                                                                                                \\ 
		\hline
		\multicolumn{3}{c}{\textbf{Chassis Controller}}                                                                                                                                                                                                                                                                                                                                  \\ 
		\hline
		Host-Processor                                                                                            & 24W                                                                                                                               & 24W                                                                                                                              \\
		DRAM-3GB                                                                                                  & 12W                                                                                                                               & 12W                                                                                                                              \\ 
		\hline
		\multicolumn{3}{c}{\textbf{Power Proportional Chassis Components}}                                                                                                                                                                                                                                                                                                               \\ 
		\hline
		Power supply losses~per Active card (25\%)                                                                & 93W                                                                                                                               & 5W                                                                                                                               \\
		Cooling per Active Line~\textasciitilde{}Card (20\%)                                                      & 77W                                                                                                                               & 4W                                                                                                                               \\
		\bottomrule
	\end{tabular}
\end{table}


\textbf{1. ASICs/ Network Processors:} The data plane operations of the switch such as
parsing the packet contents to read the header, looking up routing tables, and
forwarding data to the corresponding destination port are performed by the
networking processor. The processing is divided by two functional components:
Forwarding Engine and Replication Engine. The Replication engine separates the
header and data parts of a network packet and passes the header to the forwarding
engine. The replication engine also reassembles the packet after its processed
by the forwarding engine and in multicast communication duplicate packets to
different destination ports. The forwarding engine is the decision making
component in the line cards, and it uses the locally synchronized routing
tables, QoS and ACL lookups. According to Wobker's report \cite{wobkerPowerConsumptionHighend2012}, this
consumes 52\% of the total power in enterprise Cisco line cards.  Accordingly,
the ASIC/network processor's power consumption is computed to be 165 W. Based on
studies done by Iqbal et al. \cite{iqbalEfficienttrafficaware2012} and Luo et
al.

To construct the energy saving sleep states, we draw parallels to the design
of the sleep states in general purpose processors. In the first idle state, the
clock can be set to the lowest frequency therby resulting in 20\% savings. In
the first sleep state, the lookup caches in the forwarding engines can be flushed
and clock gated along with the replication engines. In the next sleep state, the core processing clock and processor bus is clockgated.
In the lowest sleep state state, the entire architectural state of the processor including runtime data from Fowarding information base rules, Qos Classification counters is written to the Linecard DRAM and power gated.
 % \cite{2005LuoLowpowernetwork}, we assume a 60\% power reduction due to power gating of ALU and micro engines in the network processor.
%Dynamic frequency scaling and power gating~\cite{} can be used to conserve power using idle states that saves power around an average of 30\%. Therefore, power consumption in low power mode will be 70\% of peak power.

\textbf{2. VoQ (DRAM memory and SRAM buffer):} In Cisco line cards, the Virtual Output
Queuing memory is used to provide buffering and queing function to manage the
QoS, packet replication, congestion control functions. The ingress DRAM is used to buffer incoming
packets and the egress DRAM buffer is used store data payload while the header
is being processed by the forwarding engine.  The active power consumption of
DRAM depends on the frequency of accesses, and leakage/static power depends on
the transistor technology. Micron Power calculators \cite{MicronMemoryPower} for
RLDDR3 (Reduced latency DRAM) show a power consumption of 1571 mW per 1.125 GB
of memory when active and 314 mW when in sleep.
There is also a high speed SRAM buffer which acts as a write-back cache for the
DRAM memory.

\textbf{3. TCAM (Ternary Content addressable memory):} The TCAM structre is used by the
L3 routing function and to store routing table entries synchronized locally from
the route processing card. A typical 4.5 Mb TCAM structure which is used to offload high-speed packet lookup, consumes 15 W of power \cite{guoResistiveTCAMAccelerator2011}. We model the static leakage power for a 4.5 Mb CAM structure using Cacti \cite{balasubramonianCACTINewTools2017}, which estimates the power consumed during the idle sleep period when memory is not accessed.

\textbf{4. Line card Interconnect fabric:} The line card communicates with the chassis
bus using the interconnect interface. The line card fabric interconnect consumes 23W during active power state \cite{panZerotimeWakeupLine2016}. % {\bf GV: Why shouldn't we assume that it would be zero when sleeping? The Huawei paper mentioned the HOST cpu will be active, updating the table from other line cards during sleep. I was not sure how much we will save.}

\textbf{5. Host processor and local DRAM:} Each line card includes a host processor which is used in line card boot and initialization process for copying routing table information from the switch fabric card. The processor is kept running in sleep mode to keep the routing tables synchronized and to wake up the line card on packet arrival. We assume a 30\% power reduction due to dynamic frequency scaling during line card sleep \cite{liuSleepScaleRuntimeJoint2014}.

\textbf{6. Ports:} To tackle the energy consumption in network equipment, the IEEE 802.3az standard introduces the Low Power Idle (LPI) mode of Ethernet ports, which is used when there is no data to transmit, rather than keeping the port in active state all the time~\cite{gunaratneReducingEnergyConsumption2008}. The idea behind LPI is to refresh and wake up the port when there is data to be transmitted; the wakeup duration is usually small. %Also, the energy consumption of a physical layer device (PHY) in LPI mode is significantly lower than when it is in the active mode~\cite{reviriego2012energy}.  %have table ~\ref{Switch Power model}.%the IEEE 802.3az standard introduces the Low Power Idle (LPI) mode of Ethenet ports, which is used when there is no data to transmit, rather than keep the equipment in active state all the time~\cite{christensen2010ieee}. The idea behind LPI is to refresh and wake up the port from LPI mode when there is signal to be transmitted, and the duration of which is usually small.
% Sai: I;m commenting this, as the statement is not consistent with the numbers in table given below. While over large periods, there is no signal transmission. Previous study shows that the energy consumption of a physical layer device (PHY) when it is in LPI mode is expected to be significantly lower than when it is in the active mode~\cite{reviriego2012energy}. Specifically, this has been confirmed for the case of Network Interface Cards (NICs) where reductions of 70\% in the power consumption of a 1Gb/s NIC have been reported in~\cite{reviriego2011initial}
%Based on measurements on Intel's 82573L Gigabit Ethernet Controller from Intel labs by wertheimer et. al. ~\cite{wertheimer802active}, in this paper we assume there are three power states for each switch port: active, LPI, and off, and corresponding average power consumption for each state under diffrent link rates is shown in table~\ref{table1:notation}.

%\begin{table}[htbp]	
%	%\vspace{0.05in}
%	%\vspace{-0.1in}
%	\captionsetup{font=footnotesize}
%	\begin{small}
%		%\begin{center}
%		\centering
%		\begin{tabular}{|c|c|c|}
%			\hline
%			{\bf Link Rate (Mbps)} &{\bf Active (mW)} &{\bf LPI (mW)}\\
%			\hline
%			{\normalsize 0} & 0 & 53 \\ 
%			\hline
%			{\normalsize 10} & 504 & 194 \\ 
%			\hline
%			{\normalsize 100} & 483 & 314 \\
%			\hline
%			{\normalsize 1000} & 1217 & 1010  \\
%			\hline
%		\end{tabular}
%		%\vspace{-0.5in}
%		\caption{Average power consumption for port in active and LPI state.}
%		\label{table1:notation}
%	\end{small}
%	%\end{center}
%\end{table}
%
%Table ~\ref{tab:linecardpower} shows the power consumption used in our experiments for .
%{\bf GV: Could you double check Sleepscale paper from ISCA 2014 by Nam Sung Kim's group to see how they derive low power mode power for platform components beyond the processor. They were really good in doing this, why not we adopt their model to compute sleep mode power figures?}
%\begin{table*}[t]
%
%	\begin{tabular}{|l|r|r|r|r|r|l|}
%		\hline
%		Component & \multicolumn{1}{l|}{Power Active}  & \multicolumn{1}{l|}{Idle} &  \multicolumn{1}{l|}{S1 state} & \multicolumn{1}{l|}{S2 State} & \multicolumn{1}{l|}{S3 State} & References \\ \hline
%		NPs/ ASICs & 165 & 66 & 66 & 22 & 0 & \cite{pan2016towards} \cite{2012IqbalEfficienttrafficawarea} \\ \hline
%		TCAM/Forwarding Engines & 37 +  & 37  & 37 & 37 & 0 &  \cite{2011GuoresistiveTCAMaccelerator} \cite{cacti-p:iccad}\\ \hline
%		DRAM Memory & 12.5 & 12.5 & 9 & 2.4 & 0 &  \cite{micronmemory}\\ \hline
%		Switch Fabric Interconnect & 23 & 23 & 23 & 23 & 23 & \cite{pan2016towards} \\ \hline
%		Host Processor & 29 & 29 & 29 & 29 & 6 & \cite{pan2016towards} \cite{liu2014sleepscale}  \\ \hline
%		Ports & 54 & 54 &  54 & 54 & 54 & \cite{wertheimer802active} \\ \hline
%		Power supply and cooling & 30 & 30 &  26 & 18 & 12 & \cite{pan2016towards} \cite{liu2014sleepscale} \\ \hline
%		Total & 304.5 & 259.5 & 244 & 185.4 & 95 &  \\ \hline
%		Wakeup Latency & - & trivial ($\approx 0$ms) & 100 ms &  500 ms & 2 secs & ~\cite{liu2014sleepscale,pan2016towards} \\ \hline
%	\end{tabular}
%	\caption{Network switch power and wakeup latency model for a Core Switch (100Gbps). Edge and Aggregate switch power numbers are scaled down to represent their lower 10Gbps bandwidth accordingly. }
%	\label{Switch Power model}
%\end{table*}
% \begin{table*}[t]

% 	\begin{tabular}{|l|r|r|r|r|r|l|}
% 		\hline
% 		Component & \multicolumn{1}{l|}{Power Active}  & \multicolumn{1}{l|}{Idle} &  \multicolumn{1}{l|}{S1 state} & \multicolumn{1}{l|}{S2 State} & \multicolumn{1}{l|}{S3 State} & References \\ \hline
% 		NPs/ ASICs & 165 & 66 & 66 & 22 & 0 & \cite{pan2016towards} \cite{2012IqbalEfficienttrafficawarea} \\ \hline
% 		TCAM/Forwarding Engines & 37 +  & 37  & 37 & 37 & 0 &  \cite{2011GuoresistiveTCAMaccelerator} \cite{cacti-p:iccad}\\ \hline
% 		DRAM Memory & 12.5 & 12.5 & 9 & 2.4 & 0 &  \cite{micronmemory}\\ \hline
% 		Switch Fabric Interconnect & 23 & 23 & 23 & 23 & 23 & \cite{pan2016towards} \\ \hline
% 		Host Processor & 29 & 29 & 29 & 29 & 6 & \cite{pan2016towards} \cite{liu2014sleepscale}  \\ \hline
% 		Ports & 54 & 54 &  54 & 54 & 54 & \cite{wertheimer802active} \\ \hline
% 		Power supply and cooling & 30 & 30 &  26 & 18 & 12 & \cite{pan2016towards} \cite{liu2014sleepscale} \\ \hline
% 		Total & 304.5 & 259.5 & 244 & 185.4 & 95 &  \\ \hline
% 		Wakeup Latency & - & trivial ($\approx 0$ms) & 100 ms &  500 ms & 2 secs & ~\cite{liu2014sleepscale,pan2016towards} \\ \hline
% 	\end{tabular}
% 	\caption{Network switch power and wakeup latency model for a Core Switch (100Gbps). Edge and Aggregate switch power numbers are scaled down to represent their lower 10Gbps bandwidth accordingly. }
% 	\label{Switch Power model}
% \end{table*}

%
%\begin{table}[htbp]
%	\small % "\footnotesize" not needed here
%	\captionsetup{size=small}
%	\setlength{\tabcolsep}{1pt}
%	\begin{flushleft}
%		\centering
%		\begin{tabular}{|c|c|c|c|}
%			\hline
%			Component & Active Power (W) & Sleep Power (W)  & Sources\\ \hline
%			ASICs/NW processor & 165 & 66 &  \cite{pan2016towards} \cite{2012IqbalEfficienttrafficawarea} \\ 
%			TCAM/Fwd. Engines & 15 & 1.26 & \cite{2011GuoresistiveTCAMaccelerator} \cite{cacti-p:iccad}\\ 
%			DRAM & 12.5 & 2.4 & \cite{micronmemory} \\
%			Interconnect Fabric & 23 & 23  &  \cite{pan2016towards} \\
%			Host Processor & 29 & 20 & \cite{pan2016towards} \cite{liu2014sleepscale} \\ 
%			Ports & 48 x 1.21 & 48 x 1.01 &  \cite{wertheimer802active} \\ 
%		%	Local Power supply &  &  &  \\ \hline
%			Local Pwr supply & 30 & 15 & \cite{pan2016towards} \cite{liu2014sleepscale} \\ \hline
%			Total & 332 & 176 &  \\ \hline
%		\end{tabular}
%	\end{flushleft}
%	\caption{Network switch power model.}
%	\label{Switch Power model}
%\end{table}

Apart from the line cards, we model a constant baseline power of 120 W for the rest of the switch in ON state, which includes switch supervisor module, the backplane, cooling systems, switch fabric card based on Pan et al. \cite{panZerotimeWakeupLine2016}.  The wakeup latency for each of the states is derived from sleep and wake up state conceptualized in section~\ref{sec:transition}
%From the sleep state proposed above and the analysis done by Pan et al \cite{pan2016towards} we consider a 10 \textmu s wakeup latency from sleep state and a 15s power-on time for the line card. 
%\subsubsection{Switch power reduction using component sleep}

\subsection{Modeling switch sleep state transition and wake up latency}

\label{sec:transition}
\begin{figure}
\captionsetup{font=small}
\centering\includegraphics[width=.5\textwidth]{figures/switchtransition.pdf}\caption{Illustration of a Switch Sleep and Wakeup Transition process with 3 sleep states.}
\label{figure13-sleepcycle}
\end{figure}

As shown in the Figure \ref{figure13-sleepcycle}, we model the sleep policy for a switch based on the power model described in section~\ref{sec:switchpower}. The line card unit of a switch is considered to be in active state when processing any output traffic, and idle when either there is no incoming traffic for certain period of time. In the first sleep state, the switch stops processing incoming packets but continues to receive new packets in the packet buffer to require the DRAM to be on the State. TCAM is not flushed to avoid the wakeup latency associated with re-populating the routing tables. In the second sleep state S2, the server's Energy consumption is reduced by setting the ASIC or Network processor to clock-gated state. In the second sleep state, additional savings can be achieved by turning off the DRAM, and deeper sleep state for the NP/ASIC. In the last sleep state, we clock gate the TCAM memories storing the routing tables, host processor and switch interconnects to be put in sleep state. 



==> 2020-popcorns-T-SUSC (copy)/systemdesign.tex <==
\section{Power models}
\label{sec:systemdesign}
\label{sec:system-model}



\subsection{Conceptual Network Switch Low Power States}
\label{sec:switchpower}
%\subsubsection{Switch Port {\color{blue}-------$>$Switch port low power idle state}}
%\label{sec:lpi}

%Specifically, this has been confirmed for the case of Network Interface Cards (NICs) where reductions of 70\% in the power consumption of a 1Gb/s NIC have been reported in~\cite{reviriego2011initial}.

 
%We assume that there are three power states for each switch port: active, LPI, and off, and the corresponding average power consumption for each state under different link rates is shown in Table~\ref{table1:notation}. These power numbers are based on measurements on Intel's 82573L Gigabit Ethernet Controller~\cite{wertheimer802active}.

% \begin{table}[htbp]
% 	%\vspace{0.05in}\cite{pan2016towards}
% 	%\vspace{-0.1in}
% 	\captionsetup{font=footnotesize}
% 	\begin{small}
% 		%\begin{center}
% 		\centering
% 		\begin{tabular}{|c|c|c|}
% 			\hline
% 			{\bf Link Rate (Mbps)} &{\bf Active (mW)} &{\bf LPI (mW)}\\
% 			\hline
% 			{\normalsize 0} & 0 & 0 \\
% 			\hline
% 			{\normalsize 10} & 504 & 194 \\
% 			\hline
% 			{\normalsize 100} & 483 & 314 \\
% 			\hline
% 			{\normalsize 1000} & 1217 & 1010  \\
% 			\hline
% 		\end{tabular}
% 		%\vspace{-0.5in}
% 		\caption{Average port power consumption in active and LPI states.}
% 		\label{table1:notation} 
% 	\end{small}
% 	%\end{center}
% \end{table}


\input{switchpower}

\subsection{Server Low-power States and Power Model}
\label{sec:serverpower}
%\include{server_power}
%\begin{asparaenum}
%%\item[\textbf{ACPI-defined low power states}] 
%\todo{Add table for each state by referring the SleepScale paper}.
With the focus on improving energy efficiency when servers are under-utilized, low-power states were created
with goal of reaching energy proportional computing. For standardization across computing platforms, Advanced Configuration
and Power Interface (ACPI)~\cite{acpi} specification gives the Operating system developers and hardware vendors common platform independent energy savings. 
 %The ACPI-defined interfaces have been adopted by several major operating system vendors~\cite{ACPI} 
ACPI has been historically well supported by various hardware vendors such as Intel and IBM~\cite{wareArchitectingPowerManagement2010}. ACPI uses global states, \emph{Gx}, to represent states of the
entire system that are visible to the user. We discuss the component-wise
breakdown of such system states as described in the table ~\ref{tab:serverpowermodel}.

Although processor sleep states can significantly reduce the power consumed by the processor, servers can still consume a considerable amount of power, as the platform may still remain active. As a result, in order to achieve further energy savings, \emph{system sleep states}, that also put platform components into low-power state, are considered for server farm power management. We consider additional full system sleep state. %\PopCorns uses \emph{S3} as full system sleep state as it can further achieve substantial energy savings especially at low demand for server utilization.

%,\todo{Equation for processor power ref for cpu power consumption}
%\todo{Have a diagram for server components and sleep}
%\todo{Describe Gstates}

\begin{itemize}
	\item CPU(s) Power: Low-power states are now an important feature that are
	widely supported in today's processors. In a multicore processor, each core
	can have different architectural components or features disabled or turned off
	by shutting down the clock signal or turning off power and such states are
	called C-states. A higher level C state or S state typically indicates more
	aggressive energy savings but also corresponds to long wakeup latencies.
	For multi-core processor, low-power sleep states are supported at both core
	level and package level. When all cores become idle and reside in some
	\emph{Core C state}, the entire package would be resolved to a greater power saving state, denoted as \emph{package sleep state}, which further reduces power.
	%\todo{Describe the Core state and package behavior in detail in the table.}
	
	
	
	\item{Chipset} The chipset and board consume energy used to support the main
	chipset, voltage regulators, bus control chips, interfaces for peripheral
	devices. According to Intel specifications~\cite{IntelX99Chipset} the chipset
	has TDP of 6.5W. The minimal power savings in the deeper sleep states of the
	system can be ignored.
	
	\item{DRAM}: The DRAM power consumption can be seperated into 3 parts ,
	read/write energy, Activate and pre-charge energy to open the specific row buffer to operate
	upon and refresh power to continuously perform the refresh cycle.
	Characterizing the DRAM power depends on several factors such as:
	
	1. DRAM technology DDR3, DDR4, LPDDR3L, etc with their respective power and
	performance characteristics.
	
	2. Workload : number of last level cache misses: An application whose working
	memory does not fit into the CPU cache can have a lot misses.
	
	3. Manufacturer optimizations: DRAM powerdown mode can be implemented
	differently by different manufacturers. The DRAM self-refresh cycle allows
	DRAM to be clock-gated from the external memory controller for self refreshing cycle.
	
	4. Memory clock speed. Higher clock improves performance buy consumes more memory.
	
	We used the micron power calculator to arrive the power consumption of the
	memory components as shown in the table ~\ref{tab:linecardpower}.
	
	\item{Power supply} We consider the AC-DC energy conversion loss which are
	typically 10\% of the power consumed by the system.
	
	\item{Fans}: The power consumption of a cooling fan is directly proportional to
	the cubic function of current fan speed utilization %~\cite{needfanspeed}.
	
\end{itemize}
% kWithin each \emph{Gx} state, there
% are one or more system sleep states, denoted as
% \emph{Sx}. For instance, \emph{S0} is the
% working state and \emph{S1}, \emph{S3} are the
% system sleep states. When a computer system is
% in the \emph{S0} state, the processor is
% allowed to be in a set of \emph{C} states such
% as \emph{C0}, \emph{C1}, and \emph{C6}. A
% higher-numbered C state typically indicates
% more aggressive energy savings but also
% corresponds to longer wake-up latencies. Modern
% processors generally provide high parallelism
% by integrating multiple cores within one
% package. Therefore, low-power sleep states are
% supported at both core level and package level.
% Typically, the package \emph{C} state is
% automatically resolved to the shallowest sleep
% state among all the cores. In the rest of the
% paper, we will denote package \emph{C}  state
% as package sleep state.
%Low-power states are now an important feature that are widely supported in
%today's computing systems. The Advanced Configuration and Power Interface (ACPI)~\cite{acpi} provides a standardized specification for platform-independent power management.
%The ACPI-defined interfaces have been adopted by severmal major operating system vendors~\cite{acpi_linux,acpi_bsd} and supported by various hardware vendors such as Intel and IBM~\cite{ibm_power7, intel_manual}. ACPI uses global states, \emph{Gx}, to represent states of the entire system that are visible to the user. Within each \emph{Gx} state, specifies various processor low power states, denoted as \emph{Cx}, and system low-power states, denoted as \emph{Sx}. For instance, \emph{S0} is the working state and \emph{S3}, \emph{S4} are the system sleep states. When a computer system is in the \emph{S0} state, the processor is allowed to be in a set of \emph{C} states such as \emph{C0}, \emph{C1}, \emph{C3}, and \emph{C6}.



% \usepackage{array}
% \usepackage{graphicx}
% \usepackage{colortbl}
% \usepackage{booktabs}




% \usepackage{graphicx}
% \usepackage{colortbl}
% \usepackage{booktabs}


% \usepackage{graphicx}
% \usepackage{booktabs}
% \usepackage{colortbl}


\begin{table*}
	\small	\centering
	\setlength{\extrarowheight}{0pt}
	\addtolength{\extrarowheight}{\aboverulesep}
	\addtolength{\extrarowheight}{\belowrulesep}
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\caption{A Representative Server Power model with Multi-socket Xeon processors and 128GB DDR3 }
	\label{tab:serverpowermodel}
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{lcllll} 
			\toprule
			\textbf{Server Power Component } & \textbf{Number of units } & \textbf{Active } & \textbf{Idle (G0) } & \textbf{G1 } & \textbf{G2 } \\ 
			\hline
			\begin{tabular}[c]{@{}l@{}}\textbf{CPU}\\\textbf{(Intel Xeon E5}\\\textbf{V2 2690) }\end{tabular} & 2 & 135W & 108W & 22W & 15W \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Average sustainable\\power consumption (TDP)\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}All CPUs/cores set\\to lowest DVFS \\frequency with\\20\% savings\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}All cores of all CPUs\\in C3 state- Clock\\Stopped and Cache\\flushed but other\\architectural state\\maintained\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}All cores of all CPUs\\in C6 state- Power\\gating the CPU, after\\saving the architectural\\state to the DRAM\end{tabular} \\
			\textbf{ Chipset } & 1 & 8W & 8W & 8W & 8W \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Chipset powering \\the interfaces and\\peripherals\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Chipset powering\\the interfaces and\\peripherals\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Chipset powering the\\interfaces and\\peripherals\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Chipset powering the\\interfaces and peripherals\end{tabular} \\
			\begin{tabular}[c]{@{}l@{}}\textbf{ Memory }\\\textbf{(8x16GB DDR3) }\end{tabular} & 8 & 1.45W & 0.29W & 0.29W & 0.29W \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}DRAM serving a normal\\utilization~of reads writes\\(25\% of all CPU~cycles\\each) + ACT~power (228mW) +\\I/0 power (540mw) + Background +\\Termination power(672mW)\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Memory without new\\Reads or Writes, with ACT\\and background power\\consumption, and\\Background power 57mW.\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Memory without new\\Reads or Writes, \\with ACT and\\background power consumption, and\\Background power 57mW.\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Memory without new\\Reads or Writes, with\\ACT and background\\power consumption,\\and Background\\power 57mW.\end{tabular} \\
			\begin{tabular}[c]{@{}l@{}}\textbf{ Disks }\\\textbf{(8 TB SSDs}\\\textbf{in RAID) }\end{tabular} & 4 & 10W & 10W & 1W & 1W \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  & Active mode & Active mode & standby power & standby power \\
			\textbf{ Network Interface card } & 2 & 3W & 3W & 1W & 1W \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  & Active mode & Wake-on-LAN mode & Wake-on-LAN mode & Wake-on-LAN mode \\
			\textbf{ Power Supply losses } & 2 & 38 W & 31W & 7W & 5W \\
			\rowcolor[rgb]{0.851,0.851,0.851}  & \multicolumn{1}{l}{} & 10\% current system power consumption & 10\% current system power consumption & 10\% current system power consumption & 10\% current system power consumption \\
%			\begin{tabular}[c]{@{}l@{}}\textbf{Cooling Fans}\\\textbf{15W fans}\end{tabular} & \multicolumn{1}{l}{2} & 10.5W & 5W & 5W & 0 W \\
			\begin{tabular}[c]{@{}l@{}}\textbf{Cooling Fans}\\\textbf{15W fans}\end{tabular} & 2 & 10.5W & 5W & 5W & 0 W \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  & 70\% of Full Power & 30\% Power & 30\% Power & Off \\ 
			\hline
			\textbf{Total} & \multicolumn{1}{l}{} & \textbf{385W} & \textbf{308W} & \textbf{73W} & \textbf{~51W} \\ 
			\hline
			\textbf{ Transition Time - To sleep } &  & 0usecs & 10 usecs & 100 usecs & 500 msecs \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  &  & DVFS transition time & Transition to C3 state & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.851,0.851,0.851}}l@{}}Saving Architectural state of CPU to ram\\and~power supply\\power up\end{tabular} \\ 
			\hline
			\textbf{ Wakeup latency } &  & 0 usecs & 100 usecs & 100 msecs & 1 second \\
			\rowcolor[rgb]{0.851,0.851,0.851}  &  &  & CPU frequency scale & Transiting all cores to C0 state & Transitioning CPU to Active state \\
			\bottomrule
		\end{tabular}
	}
\end{table*}

%Figure~\ref{fig:power_profile} shows the power consumption for Xeon-E5 2680 processor with C1 and C6 processor sleep state enabled respectively. The power numbers are collected using PAPI API that interacts with the RAPL (Runing Average Power Limit) interfaces. %From the figure we can see that processor in  package C6 sleep state consumes much less power than processor in active state.
%When the processor is in the \emph{C0} state, it may be associated with a performance state \emph{Px}, which corresponds to a specific DVFS setting. A hierarchical view of the low-power states specified in ACPI is shown in~\ref{fig:acpi_diagram}. The combination of system low-power state and CPU low-power state is used to characterize the low-power mode of an entire server. 
%\begin{figure}[h]
%	\centering
%	\centering
%	\includegraphics[scale=0.6]{./figure/power-profile.pdf}
% \caption{Power profile of a 10-core Xeon processor with different C-state configurations. The y-axis is the range of power for the processor with the specific number of cores active and various utilization levels ranging from 10\% to 100\%.} %Note that each of the active cores settings, we generate various level of utilization to the active cores and measured the power, which explains why the power consumption for a specific number of active cores are a range of numbers.  }
%	\label{fig:power_profile}
%\end{figure}
%\footnote{We use a microbenchmark that can calibrate itself and occupy the core according to each utilization setting. To occupy multiple cores, we run multiple processes of this microbenchmark, each pinned to a specific core.}

%\subsection{Modeling Server Power}





% \begin{table}[!h]
% 	\small % "\footnotesize" not needed here
% 	\captionsetup{size=small}
% 	\setlength{\tabcolsep}{1pt}
% 	\begin{flushleft}
% 		\centering
% 		\begin{tabular}{|c|c|c|c|c|c|c|}
% 			\hline
% 			Active State  & Idle & S0-C6  & S3 & S6 & Source \\ \hline
% 			107W + 60W * (Task's CPU utilization\%)& 107W  & 86W & 60W & 22W & \cite{yao2015dual}\cite{yao2017wasp} \\
% 			\hline
% 		\end{tabular}
% 	\end{flushleft}
% 	\caption{Server power model for the active and 3 sleep states for the server.}
% 	\label{Serverpowermodel}
% \end{table}

\subsection{Modeling Job}
More and more applications are being designed using a modular microservices-based paradigm, where inter-dependent tasks are hosted on different servers. The modularisation of job helps reduce complexities in software development, with independently update-able software programs in a scalable 'single-service instance per server' deployment pattern.  
We model the execution of jobs at the server side as consisting of multiple inter-dependent tasks that include both spatial and temporal inter-dependence. Application tasks are typically executed by specific server types. For example, a web service request will first be processed by an application or web server, and a search request is processed by a database server, and this kind of task relationship is called spatial inter-dependence. In terms of temporal inter-dependence, a task cannot start executing until all of its 'parent' tasks have finished their execution, and until after their results have been communicated to the server assigned to the task. A job is considered to have finished when all of its tasks finish execution. As for servers, there are multiple cores per server and one core can only process one task. We support asynchronous task execution by allowing the server running the parent task to  release the cpu, after all flows are completed to the child tasks' server even if it is waiting in the queue for execution.

Each job $j$ can be represented as a directed acyclic graph (DAG) $G^j(V^j, E^j)$, where $V^j$ is the set of tasks of job $j$. In DAG, if there is a link from task $i$ to task $r$, then task $i^j$ must finish and communicate its results to task $r^j$ before $r^j$ can start processing. Each task $v^j \in V^j$ has a workload requirement, namely task size or execution time requirement $w^j_v$ for the core. For each link in $E^j$, there is a data transfer size $D^j_l$ associated with it, which denotes the bandwidth requirement to transfer the result over link $l$ (from the task at the head of DAG link to the task at the tail) when assigned a network flow. Figure~\ref{figure1} shows an example of a job DAG.

%\begin{figure}[htbp]
%	\captionsetup{font=small}
%	\centering
%	\vspace{-0.1in}
%	\includegraphics[scale=1.0]{./figures/wsDAG.eps}
%	\caption[test]{Example of a web service job DAG. Task 1 is executed by the application server, while task 2 is assigned to be processed by database server.\protect\footnotemark}
%	\label{fig:wsDAG}
%	\vspace{-0.1in}
%\end{figure}

\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.4\linewidth]{figures/DAG.pdf}\caption{Example of a job DAG. Numbers 1-6 denote task 1-task 6 respectively. Numbers around the tasks represent task size, while numbers on the links represent flow size.}
	\label{figure1}
\end{figure}

\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.3\textwidth]{figures/fat_tree.png}
	\caption{Fat tree topology with K=4 (16 servers).}
	\label{figure12}
\end{figure}


\subsection{Data Center System}
\label{sec:dc-sys}
Figure~\ref{figure12} shows the classic fat tree topology used in our network-server system, where each subset is called a 'pod'. In our system, each switch consists of a number of distributed cards plugged into the backplane, which provides the physical connectivity~\cite{panZerotimeWakeupLine2016}. Among these cards, there are multiple line cards for forwarding packets or flows, and can be in active, sleep, or off state. In turn, each line card contains several ports connecting to external links, which can also be in active, LPI, or off state. A typical schematic of switch, line card, and port is shown in Figure~\ref{figure13}.

%\begin{figure}[!h]
%	\captionsetup{font=small}
%	\centering\includegraphics[width=0.3\textwidth]{figures/switch.pdf}\caption{Schematic view of switch, line card and ports}
%	\label{figure13}
%\end{figure}



==> 2020-popcorns-T-SUSC (copy)/trace_eva.tex <==
\section{Evaluation on Real System}
\label{sec:evaluation}

\begin{figure*}[htbp]
	\centering
	\captionsetup{font=small}
	\includegraphics[scale=0.56]{./figure/combine-energy.pdf}
	\caption{\label{fig:per-server-energy} Energy measured on a server farm with 10 servers with different energy management policies.  The first three groups of bars represent energy breakdown in each server when Active-Idle, Delay-Doze and \titlename are applied, respectively. The rightmost three bars illustrate the total server farm energy consumption for Active-Idle (black bar), Delay-Doze (gray bar) and \titlename respectively (white bar).}	
\end{figure*}

We evaluate \titlename on a testbed with 10 Dell Poweredge servers equipped with Inten Xeon-based processors with all of the servers deployed on a dedicated rack. We installed a modified version of the Apache HTTP server for our Local Power Controller. We extended the Local Power Controller to also include a Delay-Doze timer. The Global Server Farm Power Manager is added to an additional apache server with the \emph{mod\_proxy\_balancer} module used for load balancing. Specifically, the load balancer performs operating mode transitions in servers (as discussed in Section~\ref{sec:handler}); this is done by sending special HTTP requests (\emph{/hostname/trans-to-active-mode/}, \emph{/hostname/trans-to-lp-mode}) to the application server. It also monitors the power state for each server, and manages the server wakeups (from system sleep) using IPMI interface supported by Dell systems. The special requests are handled by the local power controller that would determine the server low-power transitions accordingly. We set up a custom cpuidle governor which allows direct processor C-state transitions from userspace (e.g., C0-C6). For power measurement, we leverage two techniques: the RAPL interface for fine-grained component power, and the IPMI's system power management interface for coarse-grained server power. We evaluate the effectiveness of \titlename by providing two sets of workloads to the system: the non-bursty Wikipedia workload, that does not require server provisioning, and four bursty NLANR workloads~\cite{nlanr}, that require server provisioning to handle bursty workloads (See section~\ref{sec:provision}).

\subsection{Wikipedia Trace}
\label{sec:bursty-trace}

We performed real system energy measurements by deploying Wikipedia software stack, namely Wikipedia application (Mediawiki), database system (Mysql) on servers. We compare \titlename against Active-Idle and Delay-Doze approaches described in Section~\ref{sec:smartlp}. To capture detailed energy breakdown, we leverage RAPL interface for fine-grained power measurement. The RAPL utility records the CPU and RAM power values periodically. We configure \titlename with the $T_s$, $T_w$ and $\tau$ parameters that achieve energy-latency Pareto-optimality with tail latency constraint set to 2.0. Similarly, for Delay-Doze, we explore various
values of the delay-timer and choose the setting that achieves the best power with the same tail latency constraint. From our experiments, we get actual CPU and RAM energy consumption for each server. To get the overall server energy, we also factored in the platform energy shown in Table~\ref{table:powermode}. 

Figure~\ref{fig:per-server-energy} shows the per-server energy breakdown in terms of CPU, DRAM, and platform energy. With Active-Idle power management, all the 10 servers have similar energy consumption. With Delay-Doze, some of the servers are able to stay in system sleep state for longer periods of time, thus saving energy. With \titlename, we can clearly see that most of the servers drastically reduce energy consumption, and only a minimal subset of servers (server\#6 and \#10) are used for servicing jobs. Note that the energy consumption of server\#10 is slightly higher than that of Active-Idle power management since the server is at a higher utilization level while other servers remained inactive. Overall, \titlename gains 39\% reduction in energy saving compared to Delay-Doze, and 56\% energy savings compared to Active-Idle.

\begin{figure}[htbp]
	\centering
	\subfloat[ny09]{
		\includegraphics[scale=0.34]{./figure/ny09.pdf}
		\label{fig:nlanr-ny09}
		\hspace{0.05in}
	}
	\subfloat[pa09]{
		\includegraphics[scale=0.34]{./figure/pa09.pdf}
		\label{fig:nlanr-pa09}
		%\hspace{0.2in}
	}
	
	\subfloat[pa10]{
		\includegraphics[scale=0.34]{./figure/pa10.pdf}
		\label{fig:nlanr-pa10}
		\hspace{0.05in}
	}
	\subfloat[uc09]{
		\includegraphics[scale=0.34]{./figure/uc09.pdf}
		\label{fig:nlanr-uc09}
		%\hspace{0.2in}
	}
	\caption{System utilization for four bursty traces.}
	\label{fig:utilizations}
\end{figure}
\begin{figure}[htbp]
	\centering
	\includegraphics[scale=0.45]{./figure/trace-eval/trace_result.pdf}
	\caption{Normalized energy consumption relative to peak energy on a 10-server cluster}
	\label{fig:traceresults}
\end{figure}

\subsection{Bursty Traces}
\label{sec:nonbursty-trace}

 As the raw NLANR network traces~\cite{nlanr} present job arrivals that are too infrequent for the server farm system with 10 application servers (less than 2\%), we speed up the trace by scaling the 24-hour trace to one hour. We choose four traces, namely \emph{ny09}, \emph{pa09}, \emph{pa10} and \emph{uc09}. Figure~\ref{fig:utilizations} shows the utilization levels (scaled) for the four traces over one hour. All traces exhibit bursty traffic patterns. For example, the \emph{ny09} trace has highly fluctuating utilizations ranging from 4\% to 45\% with a large number of spikes. To run the traces, we set up a software stack similar to the one in Section~\ref{sec:bursty-trace}. Each request in the trace is serviced by a PHP script that accesses a pre-defined set of pages randomly, and we note that the average service time is about the same as Wikipedia web requests.
 
To enable server provisioning, the Server Farm Power Manager additionally samples the server farm utilization levels based on the job arrival rates. Utilization is calculated as the product of job arrival rate and average job execution time. Standard deviation on the samples for utilization levels is calculated every 120 seconds. The number of provisioned servers is calculated dynamically (See Section~\ref{sec:provision} for details). Note that, in our comparative studies, the delay-timer values are re-evaluated for each trace such that best possible energy savings are had while meeting the QoS constraints. Figure~\ref{fig:traceresults} shows the energy consumption for the four bursty workloads using Active-Idle, Delay-Doze and \titlename. The energy is normalized to the peak energy which is $PeakPower*Time$. The energy reduction for \titlename ranges from 34\% to 40\% compared to Active-Idle. Even with the best delay timer settings, Delay-Doze only achieves 9\% to 12\% energy reduction in bursty workloads. We observe that due to the job arrival rate spikes (especially for \emph{uc09}), in order for Delay-Doze to meet the tail latency constraint of 2.0, the delay timer has to be set to larger values, and in turn the servers have limited chance to enter system sleep state.



==> ack.tex <==
\section*{Acknowledgment}

\label{ack}
This material is based upon work supported in part by the National Science Foundation 
under CAREER Award CCF-1149557 and CNS-1320226.

==> algorithms__Santosh_Dayapule_s_conflicted_copy_2019-08-08_.tex <==
\section{Solution Approach}
\label{sec:algorithms}
Modeling this joint power optimization problem in DCN as an Integer Linear Programming (ILP) formulation is a solution, and optimization tools like MathProg can be used to provide a near-optimal result. However, the computation complexity increases exponentially with the number of servers and switches~\cite{wang2012carpo}. In a typical data center with tens of thousands of servers and hundreds of switches, it is computationally prohibitive to solve the optimization problem. We therefore propose a computationally-efficient heuristic algorithm in this section. 

\begin{comment}
In this section, we first present an Integer Linear Programming (ILP) formulation for the joint optimization problem in details. We then propose heuristic algorithms for solving the optimization problem efficiently.
%We then propose two heuristics for the static case, and later adapt them to the dynamic case.

\subsection{ILP formulation}
In the ILP formulation, the input parameters are shown in Table~\ref{table2:notation} .

\begin{table}
	%\centering
	\caption{\label{table2:notation} Notations in ILP formulation}
	\scalebox{0.5}{
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Meaning} \\ 
		\hline
		$v$ & an arbitrary network node  \\
		\hline
		$s$ & an arbitrary server  \\
		\hline
		$V$ & set of network nodes (e.g. servers, switches)  \\
		\hline
		$S$ & set of servers  \\
		\hline
		$j$ & an arbitrary job  \\
		\hline
		$L$ & set of links in the network  \\
		\hline
		$P_{m,n}^{linecard}$ & power consumption of line card $m$ in switch $n$ \\
		\hline
		$P_{n}^{base}$ & power consumption of all parts other than line cards in switch $n$ \\
		\hline
		$N^{switch}$ & number of switches  \\
		\hline
		$P_{c,s}^{core}$ & power consumption of core $c$ in server $s$ \\
		\hline
		$P_{s}^{base}$ & power consumption of all parts other than cores in server $s$ \\
		\hline
		$N_{s}^{core}$ & number of cores in server $s$  \\
		\hline
		$N^{server}$ & number of servers  \\
		\hline
		$T^{j}$ & set of tasks in job $j$  \\
		\hline
		$t^{j}$ & an arbitrary task in job $j$, $t^{j}\in{T^{j}}$  \\
		\hline
		$N^{job}$ & number of jobs  \\
		\hline
		$B_{r,t}^{j}$ & bandwidth requirement between task $r$ and task $t$ of job $j$, task $r$ is in server $s_r$, task $t$ is in server $s_t$  \\
		\hline
		$l_{n_1,n_2}$ & link between node $n_1$ and $n_2$, $l_{n_1,n_2}$ $\in$ L  \\
		\hline
		$C_{l_{n_1,n_2}}$ & capacity of link $l_{n_1,n_2}$  \\
		\hline
		$L_{m, n}$ & set of links connected to line card $m$ in switch $n$  \\
		\hline
		$f_{l_{n_1,n_2}}$ & number of flows on link $l_{n_1,n_2}$ \\
		\hline
		$l_{p,s_1,q,s_2}$ & link between line card p in switch $s_1$ and line card q in switch $s_2$ $s$ to node $d$ \\
		\hline
		$l_{s,d}$ & an arbitrary path from node $s$ to node $d$ \\
		\hline
		$f_{l_{n_1,n_2}}$ & set of flows on link $l_{n_1,n_2}$ \\
		\hline
		$d^{l_{n_1,n_2}}_f$ & data rate of flow $f$ on link $l_{n_1,n_2}$ \\
		\hline
	\end{tabular}}
\end{table}

\begin{center}
	\scalebox{0.8}{
	Objective: ${Minimize(P^{switches}+P^{servers})}$}
	\scalebox{0.8}{
	$=\min{\sum_{n=1}^{N^{switch}}(P^{base}_n+\sum_{m=1}^{N_n^{linecard}}P_{m,n}^{linecard}x_m^n) +\sum_{s=1}^{N^{server}}(P_s^{base}+\sum_{c=1}^{N_s^{core}}P_{c,s}^{core}z_c^s)}$}
		
		%\sum_{k=1}^{H}(\left\lceil \frac{w_i^j}{k} \right\rceil-1)a^j_{i, v, k}}$}

\end{center}

Decision Variables:

a)
\begin{equation*}
a^{j}_{t, c, s}=
\begin{cases}
1, \quad\makebox{if task } t \makebox{ of job } j \makebox{ is assigned to core } c \makebox{ in server }  s  \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

b)

\begin{equation*}
z^{j}_{t, r, s}=
\begin{cases}
1, \quad\makebox{if task } t \makebox{ and } r \makebox{ of job } j \makebox{ are assigned to server }  s  \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

c)
\begin{equation*}
y^{s}_{c}=
\begin{cases}
1, \quad\makebox{if core } c \makebox{ in server } s \makebox{ is operating; } \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

d)
\begin{equation*}
x^{n}_{m}=
\begin{cases}
1, \quad\makebox{if line card } m \makebox{ in switch } n \makebox{ is active; } \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

d)
\begin{equation*}
\lambda^{l}_{p_{s,d}}=
\begin{cases}
1, \quad\makebox{if link } l \makebox{ is on path } p_{s,d} \makebox{;} \\
0, \quad\makebox{otherwise }
\end{cases}
\end{equation*}

Constraints:

a) Each task of each job can be assigned to only one core. For all $j, t$
\begin{equation*}
\sum_{s=1}^{N^{server}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}

b) The number of tasks being executed on a server cannot exceed the number of its cores. For all $s$
\begin{equation*}
\sum_{j=1}^{N^{job}} \sum_{t\in{T^j}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}

c) Constraints to find the value of $z^{j}_{t, r, s}$. For all $j, t, r, s$
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \leq 1 + z^{j}_{t, r, s}
\end{equation*}
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \geq 2z^{j}_{t, r, s}
\end{equation*}

d) If link $l_{n_1,n_2}$ is on path $p_{s,d}$, there must exist another link from node $n_1, n_2$ respectively on this path.
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \leq 1 + z^{j}_{t, r, s}
\end{equation*}
\begin{equation*}
\sum_{c=1}^{N^{core}_s}a^{j}_{t, c, s} +  \sum_{c=1}^{N^{core}_s}a^{j}_{r, c, s} \geq 2z^{j}_{t, r, s}
\end{equation*}

e) If link $l_{s_1,s_2}$ is on the task communication path $p_{s,d}$, then the corresponding line cards in $s_1$ and $s_2$ must be active and the link between them is also on $p_{s,d}$. For $l_{p,s_1,q,s_2}$ $\in$ $L_{p,s_1}$, $l_{p,s_1,q,s_2}$ $\in$ $L_{q,s_2}$
\begin{equation*}
\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} = \lambda^{l_{s_1,s_2}}_{p_{s,d}} = x^{s_1}_{p} = x^{s_2}_{q}
\end{equation*}
\begin{equation*}
x^{s_1}_{p}\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} \geq \lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}}
\end{equation*}
\begin{equation*}
x^{s_2}_{q}\lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}} \geq \lambda^{l_{p,s_1,q,s_2}}_{p_{s,d}}
\end{equation*}

f) Line card $m$ in switch $n$ is off only when all the links connected to it are not on any path.
\begin{equation*}
\left| L_{m,n} \right| x^{n}_{m} \geq \sum_{l\in{L_{m,n}}}\lambda^{l}_{p_{s,d}}
\end{equation*}

g) Total flow rate on a link cannot exceed the link capacity.
\begin{equation*}
\sum_{f\in{f_{l_{n_1,n_2}}}}^{N^{server}} \sum_{c=1}^{N_s^{core}} a^{j}_{t, c, s} = 1
\end{equation*}
\end{comment}

\subsection{Heuristic Algorithms}
In this section, we first present a power management algorithm for the transition of line card and port power state, a simple power transition algorithm for servers, and then propose joint job placement and network routing algorithm for solving the optimization problem efficiently.

%It is computationally prohibitive and NP-hrad to solve the ILP problem above and get the optimal solution for large-scale cases. We therefore propose two computation-efficient heuristic algorithms in this section. The main idea of our algorithm is to jointly consider the status of server pool and network before assigning jobs.

\subsubsection{Power State Transition Algorithm}

{\color{blue}remove the port Low Power Idle (LPI) transition from the algorithm (save very little power), add more line card power states, the transition algorithm to control the transition}

\begin{table}
	\centering
	\captionsetup{font=small}
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Description} \\ 
		\hline
		$T_s$ & traffic threshold for port waking up  \\
		\hline
		$T_a$ & traffic threshold for port turning into LPI state  \\
		\hline
		$Q_{iL}$& current traffic load at port $i$ in line card $L$  \\
		\hline
		$\tau_{wakeup}^{port}$ & port wakeup delay  \\
		\hline
		$\tau_{wakeup}^{LC}$ & line card wakeup delay  \\
		\hline
		$\tau_{LPI}^{port}$ & port turning into LPI state delay \\
		\hline
		$\tau_{sleep}^{LC}$ & line card turning into sleep state delay \\
		\hline	
	\end{tabular}
	\caption{\label{algorithm1table} Notations in PopCorns power state transition algorithm.}
\end{table}

As not all switches in DCN need to be active all the time, if we can intelligently control the transition of active and low power state for ports and line cards, then data center network power consumption could be saved. Therefore, we propose the Power State Transition Algorithm~\ref{algorithm1} to implement network power management. The notations are elaborated in Table~\ref{algorithm1table}. An overview of our approach is shown in Figure~\ref{figure3}. We assume that there is a global controller that keeps record of all the line cards, ports, and server status, including their power state, queue size, etc. The global controller monitors the current traffic load (number of pending flows or packets) at each port and decides whether the current line card power state should change. It then decides if the port state should change as a feedback. In our design, we couple the line card and port power state and their transition: if a line card is in sleep or off state, then all the ports are also in LPI or off state; if a line card is active, then its ports can be in LPI or active state, and LPI ports can be woken up to become active in a short time. %~\ref{algorithm1} describes our proposed design in details.


\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.5\textwidth]{figures/Presentation2.pdf}
	\caption{Power state transition overview.}
	\label{figure3}
\end{figure}


\begin{algorithm}
	\SetAlgoNoLine
	\caption{Power State Transition Algorithm}
	\label{algorithm1}
	\KwIn{$T_s$, $T_a$, $Q_{iL}$}
	\KwOut{Line card and port state transition}
	Initialization: All line cards are in sleep state, all ports are in LPI state\;
	
	\While{there are jobs to be executed}
	{
		\If{a flow arrives at port $i$ of line card $L$ at time $t$}
		{
			\If{$L$ is in sleep state} {
				\If{$Q_{iL} > T_s$} {
					$L$ begins waking up from sleep state\;
					$i$ begins waking up from LPI state\;
				} 
				\Else
				{
					$L$ begins waking up after $\tau_{wakeup}^{LC}$\;
					$i$ begins waking up after $\tau_{wakeup}^{port}$\;
				}
				
			} 
		}
		\If{a flow is transimitted from port $i$ of line card $L$ at time $t$} {
			\If{$Q_{iL} < T_s$} {
				$i$ starts transition to LPI after $\tau_{LPI}$\;
				\If{after $\tau_{LPI}$, all the ports of $L$ are in LPI state} {
					$L$ starts transition to sleep state after $\tau_{sleep}^{LC}$;
				}
			}
		}
	}
	
\end{algorithm}

\subsubsection{Server State Transition Algorithm}

{\color{blue}multi-core servers, multiple power states}

As mentioned in Section~\ref{sec:serverpower}, we simply model two power states for the server: active and C6 sleep state. Algorithm~\ref{algorithm4} describes our policy on managing the server power states. We assume that each server in DCN has a local queue to buffer the tasks, and tasks should first be dispatched to active servers whose queue size do not exceed a threshold. The threshold controls the job latency.

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Server State Transition Algorithm}
	\label{algorithm4}
	\KwIn{ server wakeup latency $\tau_{wakeup}^{server}$, local queue of server $S$}
	\KwOut{Server power state transition}
	
		\If{a task arrives at a server $S$}
		{
			\If{$S$ is in sleep state} {
				$S$ begins waking up after wakeup latency $\tau_{wakeup}^{server}$\;
			} 
		   \Else {
		   		task is put in the local queue of $S$\;
	   		}
		}
		\If{a task is finished executing at a server $S$}
		{
			\If{local queue of $S$ is empty} {
				$S$ begins turning into sleep state\;
			} 
		}
	
	
\end{algorithm}

\subsubsection{Cooperative Network-Server Algorithm}

{\color{blue}periodical global control/computation, traffic prediction like TS-Bat}

The main idea of our algorithm is to jointly consider the status of server pool and network before assigning jobs. To be more specific, for a job consisting of several pairs of interdependent tasks, if we place task pairs based on their interdependence, and choose the core pair with the minimum routing cost, instead of randomly placing them on available cores without awareness of communication requirement between tasks, then the placement together with its corresponding routing path must be the optimal. And in the context of this paper, network routing cost is energy consumption, since every line card on the chosen routing path has to be active, or it will have to be woken up.

Based on this idea, we propose the Cooperative Network-Server (CNS) Algorithm~\ref{algorithm2}. The notations are elaborated in Table~\ref{algorithm2table}. In the initial stage, we compute and store all possible routing paths between any pair of network nodes. As mentioned in the previous section, we have a global controller to keep track of all the line cards, ports, and server statuses. Thus, when a job consisting of a set of interdependent tasks arrive, we first check the server side to select all server pairs whose power state is active and local queue sizes do not exceed a threshold. If no server statisfies these requirements, then servers with full local queue and servers in C6 sleep state will be selected. Note that if a task is assigned to a server in sleep state, then the server will be awoken immediately and enter active state after a wakeup latency. For each server pair we select possible routing paths between them from the pre-computed routing paths set. Along each path, line cards could be active, sleeping, or off, and ports could be active, LPI, or off, but if we assign a path to the task pair, all the line cards and ports along it should become active. In other words, we need to wake up the inactive line cards and ports on the chosen path, which results in extra power consumption and wakeup latency. Based on this, we can compute and assign a weight, which is a measurement of the number of active line cards and ports, to each possible routing path, and choose the server pair with minimum routing cost. And our proposed Cooperative Network-Server Algorithm will output the least-weight path and its corresponding server pair for each task pair.

\begin{table}
	\centering
	\captionsetup{font=small}
		\scalebox{0.7}{
	\begin{tabular}{|c|c|c|}
		\hline
		\bf{Symbol}& \bf{Description} \\ 
		\hline
		$P$ & all the routing paths between any pair of network nodes  \\
		\hline
		$Q_s$ & local queue size of server $s$  \\
		\hline
		$T_s^{server}$ & local queue size threshold of server $s$\\
		\hline
		$S$ & all the servers in DCN  \\
		\hline
		$S_{ava}$ & all the servers whose current queue size doesn't exceed $T_s^{server}$  \\
		\hline
		$P_{x, y}$ & all the routing paths between node $x$ and $y$ in DCN\\
		\hline
	\end{tabular}
}
	\caption{\label{algorithm2table} Notations in PopCorns Cooperative Network-Server Algorithm.}
\end{table}

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Cooperative Network-Server Algorithm}
	\label{algorithm2}
	\KwIn{$P$, $Q_s$, $T_s$, line cards and ports power state, task dependency within a job}
	\KwOut{Job placement and corresponding routing path}
	
	\While{job $j$ consisting of task set $T^j$ arrives}
	{
		\For{each pair of interdependent tasks $(T^j_m, T^j_n)$ in $T^j$}
		{
			select $S_{ava}$ from $S$\;
			\For {each pair of available servers $(x, y)$ in $S_{ava}$}
			{
				compute $P(x, y)$ for server pair $(x, y)$ from $P$\;
				\For {each path $p$ in $P(x, y)$}
				{
					get power states of all the ports and line cards along $P$ from the global controller, compute path weight $w(x, y)$ in terms of energy consumption\;
				}
			}
			choose the least-weight path associated with corresponding server pair for task pair $(T^j_m, T^j_n)$\;
		}
	}
\end{algorithm}

{\color{blue}
\begin*{algorithm}
	\SetAlgoNoLine
	\caption{Popcorns Weight assignment algorithm}
	\label{algorithm3}
	\KwIn{$i$, $j$, Server/line card power state, Number of flows on Link (i,j), LinkBandwidth, FlowSize, AverageNumberOfHops }
	\KwOut{$W(i,j)$ Weight for the edge connecting nodes i and j} 
	
	LinkWeight(i,j) \leftarrow 0;
	
	\If{$i$ is Server}
	{
		LinkWeight(i,j) + \leftarrow (ServerActivePower - Current Sleep state power) * taskSize + EdgeLinkBW /FlowSize;
	}
	\If{$j$ is a Switch} 
	{
		AvailableBandwidth = min(EdgeLinkBW,MaxLinkRate(i,j)/number_of_flows);
		
		LinkWeight (i,j)+ \leftarrow Switch $j$ ActivePower * FlowSize/EdgeLinkBW ;
		
		delayedTime \leftarrow  (FlowSize/(EdgeSwitchBW - AvailableBandwidth);
		LinkWeight (i,j) + \leftarrow  (Switch $j$ ActivePower + 2 * ServerActivePower) * delayTime / AverageHopCount;
	}
\end*{algorithm}
}

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Job scheduling Algorithm}
	\label{algorithm2}
	\KwIn{$P$, $Q_s$, $T_s$, line cards and ports power state, task dependency within a job}
	\KwOut{Job placement and corresponding routing path}

	\While{job $j$ consisting of task set $T^j$ arrives}
	{
		\For{each pair of interdependent tasks $(T^j_m, T^j_n)$ in $T^j$}
		{
			select $S_{ava}$ from $S$\;
			\For {each pair of available servers $(x, y)$ in $S_{ava}$}
			{
				compute $P(x, y)$ for server pair $(x, y)$ from $P$\;
				\For {each path $p$ in $P(x, y)$}
				{
					get power states of all the ports and line cards along $P$ from the global controller, compute path weight $w(x, y)$ in terms of energy consumption\;
				}
			}
			choose the least-weight path associated with corresponding server pair for task pair $(T^j_m, T^j_n)$\;
		}
	}
\end{algorithm}

\begin{algorithm}
	\SetAlgoNoLine
	\caption{Job Scheduling Algorithm}
	\label{algorithm3}
	\KwIn{input}
	\KwOut{output}
	\If{there is job to be finished}{then-block}
	content...
\end{algorithm}

==> delaytimer_tstw.tex <==
\section{Workload Adaptation}
\label{sec:tstw_exp}
\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.3]{./figure/algorithm_chart.pdf}
	\caption{\titlename Power Management Framework}
	\label{fig:alg_overview}
\end{figure}
While delay timers are useful in saving energy, we note that they lack workload awareness. Large values of delay timers could cause the system to remain in higher power states for longer than necessary resulting in increased energy consumption, while too small values for delay timers result in premature entry into low-power states. This can be problematic on two counts: 
\begin{inparaenum}
\item The transition energy between power states can be high. 
\item The wakeup latencies from low-power states can degrade system performance.
\end{inparaenum} 

To incorporate workload-awareness, we explore a two-level adaptive strategy that controls the active and low-power state transitions using a  local server power controller and a global server farm power manager. 

\subsection{\titlename: Workload-Adaptive Algorithm}
\label{sec:handler}
We now present the design for our \titlename framework. As shown in Figure~\ref{fig:alg_overview}, the server farm power manager in the front end monitors the current load (number of pending jobs per server) and sends control commands to the local power controller. The server farm power manager puts the servers in either active or sleep modes. The bottom part of Figure~\ref{fig:alg_overview} presents state transitions coordinated by the local server power controllers. 


\begin{table}[htbp]	
	\captionsetup{font=footnotesize}
	\begin{footnotesize}
		%\begin{center}
		\begin{center}
		\caption{Notations in \titlename power management algorithm}
		\begin{tabular}{|c|l|}
			\hline
			{\bf Symbol} &{\bf \hspace{0.8in}Description}\\
			\hline
			{\normalsize $V_{act}$} & servers in active/package sleep mode \\ 
			\hline
			{\normalsize $V_{s}$} & servers in system sleep mode \\ 
			\hline
			{\normalsize $T_{s}$} & workload threshold to reduce active servers \\
			\hline
			{\normalsize $T_{w}$} & workload threshold to increase active servers \\
			\hline
			{\normalsize $N_{p}$} & number of provisioned shallow sleep servers \\
			\hline
			{\normalsize $\tau$} & delay time before entering system sleep \\
			\hline		
		\end{tabular}
		\label{table:notation}
		\end{center}
	\end{footnotesize}
	%\end{center}
\end{table}

\begin{algorithm}[ht]
	\footnotesize
	%\SetAlgoLined
	\KwIn{$T_{s}$, $T_{w}$, $N_{p}$, $\tau$, $n$ (total number of servers)}
	%\small
	%\tcc{By default, all servers are placed in $\mathcal{V}_{act}$}
	%\tcc{Initial state of each server is $lp_1$, the shallowest sleep state}
	\small
	%
	%\tcc{$jop\_threshold$ -- empirically estimated score value that may likely 
	%indicate JOP attack}
	%
	Initialization: 
	$V_{act}=\{s_1,s_2,...,s_n\} $; $V_{s}=\{\}$\;
	%	\For{i in [1,n]}{
	%		power state of $s_i$ $\leftarrow$ $idle$\;
	%		initial processor frequency  $f$ for $s_i$\;
	%	}
	\While{there are unfinished jobs}{
		
		\If{a new job $j$ arrives at time $t_a$}{		  
			%add $j$ to the global queue\;
			%$qsize \leftarrow qsize + 1$\;
			%update $H_q$ with $(t_a, qsize)$\;
			%		        \If{an active server with free core exists} {
			%		          schedule the new job on a free core\;
			%		          // priority: highest utilized server first\;
			%		          continue\;
			%		        }
			%            collect total number of jobs in system\;
			%		    add $j$ to the global queue\;
			compute $load\_per\_active\_server$\;
			\If{$load\_per\_active\_server>T_w$ and $|V_{s}|>0$}{
				%\If{$V_{s}$ is not empty}{
				retrieve a server $s$ from $V_{s}$\;
				$V_{act}$.add($s$)\; 
				%					//$s$ will be in active mode\;
				create a \emph{trans\_to\_active\_mode} request \emph{$tta\_r$}\;
				send \emph{$tta\_r$} to server $s$'s power controller\;
				%}
			}
			%      {
			%       keep $\mathcal{V}_{act}$ and $\mathcal{V}_{lp}$ unchanged\;
			%       }
		}
		
		\If{a job $j$ finishes at time $t_d$}{
			%$qsize \leftarrow qsize - 1$\;
			%update $H_q$ with $(t_d, qsize)$\;
			%	collect total number of jobs in system\;
			compute $load\_per\_active\_server$\;
			\If{$load\_per\_active\_server<T_s$ and $|V_{act}|>0$ }{
				%	\If{$V_{act}$ is not empty}{
				retrieve a server $s$ in $V_{act}$\;
				$V_{s}$.add($s$) \;
				%	//$s$ will be set to sleep mode\;
				create a \emph{trans\_to\_sleep\_mode} request \emph{$tts\_r$}\;
				\If{count of shallow sleep servers$>N_{p}$}{
					\emph{$tts\_r$}.enableDelayTimer($\tau$)\;
				}
			    \Else{
			    	\emph{$tts\_r$}.enableDelayTimer(infinity)\;
		    	}
				send \emph{$tts\_r$} to server $s$'s power controller\;
				%	}
			}
			%       {
			%        keep $\mathcal{V}_{act}$ and $\mathcal{V}_{lp}$ unchanged\;
			%        }
		}	
	}
	\caption{Global Server Farm Power Manager}
	\label{alg:scheduler}	
\end{algorithm}

\titlename automatically activates servers when the pending load becomes too high (that could lead to higher average job latency), and then places servers in low-power sleep mode to conserve energy when the workload becomes light. We achieve our goal of balancing energy consumption and latency by estimating the current load and placing servers in different power modes. There are two important parameters in Algorithm~\ref{alg:scheduler} that govern transitioning between active and sleep modes: 1. $T_s$, workload threshold per active server below which \titlename will put an active server to sleep, and 2. $T_w$, workload threshold per active server above which \titlename will wake up an inactive server.

{\bf Global Server Farm Power Manager}: All servers are initially in the shallow low-power state, and arriving jobs are placed in the server's local job queue. As jobs arrive, the \emph{load per active mode server} is computed dynamically by the power manager in the front end based on the number of jobs sent to individual servers and the completed jobs. The global server farm power manager maintains lists of servers in active and sleep modes. When new jobs arrive, it first checks if current load per active server is above $T_w$. If so, it selects a server in sleep server pool (if available) and sends a power mode transition request to the active state for that server. When the load per active server falls below $T_s$, the power manager selects an active server and sends a power mode transition request to enter sleep mode. Algorithm~\ref{alg:scheduler} describes the \titlename power manager with its notations shown in Table~\ref{table:notation}. 
 

\textbf{Local Server Power Controller:} The processor transitions to package sleep state when it becomes idle, and stays in that state until it receives the request to wakeup from the global power manager. If the server receives a request for transition to sleep mode, it will first finish up all the pending jobs in the local queue and then enters package sleep after which a delay timer is started. The server enters system sleep upon delay timer expiration. However, if the scheduler chooses to wake up the server before timer expiration (e.g., due to sudden load increase), the timer is reset and the server goes back to active mode.

For large server farms, we can adopt one of two possible solutions: 
\begin{inparaenum}
	\item Adopt a distributed power management approach where energy is optimized within individual domains of servers with their own power managers.
	\item Adopt a hierarchical solution with multiple levels of global power managers. 
\end{inparaenum} 
We note that a distributed power management approach may be more scalable with lower implementation complexity compared to a hierarchical approach that may involve longer latencies for decision making and higher bookkeeping overheads for the servers. 

\subsection{Adaptive Server Provisioning}
\label{sec:provision}
Job arrival pattern may have local spikes (bursty), during which the service latency may suffer, especially when the servers are in low power modes. To mitigate this problem, we provision a subset of servers in shallow sleep states dynamically by setting their delay timer values to infinity. \titlename determines the number of provisioned servers {\it dynamically} through measuring the current standard deviation in the job arrival rate observed over a period of 2 minutes. Specifically, the server provision module samples the number of arrivals and calculates the utilization for each sample period (one second in our current setting). It then uses the sampling window to determine the standard deviation in the level of system utilization. The module will provision $\alpha\times stdev\times number\_servers$ dynamically in shallow sleep state. $\alpha$ is a tunable parameter. By default we set it to 3.0, since it typically covers a vast majority of the population (e.g., more than 99\% of the population in Gaussian distribution).  


==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
\subsection{Processor/System Low-power States and Power Model}
%\begin{asparaenum}
%\item[\textbf{ACPI-defined low power states}] 

%Emerging from embedded devices, low-power states are now an important feature targeted for power management in modern computer systems. Advanced Configuration and Power Interface (ACPI)~\cite{acpi} provides a standardized specification for platform-independent power management. The ACPI-defined interfaces have been adopted by several major operating system vendors~\cite{acpi_linux,acpi_bsd} and supported by various hardware vendors such as Intel and IBM~\cite{ibm_power7, intel_manual}. ACPI uses global states, \emph{Gx}, to represent states of the entire system that are visible to the user. Within each \emph{Gx} state, there are one or more system sleep states, denoted as \emph{Sx}. For instance, \emph{S0} is the working state and \emph{S1}, \emph{S3} are the system sleep states. When a computer system is in the \emph{S0} state, the processor is allowed to be in a set of \emph{C} states such as \emph{C0}, \emph{C1}, and \emph{C6}. A higher-numbered C state typically indicates more aggressive energy savings but also corresponds to longer wake-up latencies. Modern processors generally provide high parallelism by integrating multiple cores within one package. Therefore, low-power sleep states are supported at both core level and package level. Typically, the package \emph{C} state is automatically resolved to the shallowest sleep state among all the cores. In the rest of the paper, we will denote package \emph{C}  state as package sleep state. 
Low-power states are now an important feature that are widely supported in today's computing systems. The Advanced Configuration and Power Interface (ACPI)~\cite{acpi}
% provides a standardized specification for platform-independent power management. 
%The ACPI-defined interfaces have been adopted by several major operating system vendors~\cite{acpi_linux,acpi_bsd} and supported by various hardware vendors such as Intel and IBM~\cite{ibm_power7, intel_manual}. ACPI uses global states, \emph{Gx}, to represent states of the entire system that are visible to the user. Within each \emph{Gx} state, 
specifies various processor low power states, denoted as \emph{Cx}, and system low-power states, denoted as \emph{Sx}. 
%For instance, \emph{S0} is the working state and \emph{S3}, \emph{S4} are the system sleep states. When a computer system is in the \emph{S0} state, the processor is allowed to be in a set of \emph{C} states such as \emph{C0}, \emph{C1}, \emph{C3}, and \emph{C6}. 
A higher level C state or S state typically indicates more aggressive energy savings but also corresponds to longer wake-up latencies. 
%Modern processors generally provide high parallelism by integrating multiple cores within one package. 
For multi-core processor, low-power sleep states are supported at both core level and package level. When all cores become idle and  reside in some \emph{Core C state}, the entire package would be resolved to a certain C state, denoted as \emph{package sleep state}, which further reduces power. 
%Typically, the package \emph{C} state is automatically resolved to the shallowest sleep state among all the cores. 
Although processor sleep states can significantly reduce the power consumed by the processor, servers can still consume a considerable amount of power, as the platform may still remain active. As a result, in order to achieve further energy savings, \emph{system sleep states}, that also put platform components into low-power state, are considered for server farm power management.
%we consider additional full system sleep state. \titlename uses \emph{S3} as full system sleep state as it can further achieve substantial energy savings especially at low demand for server utilization.
%Other system sleep state such as \emph{S4} introduces hundreds of seconds of wakeup overhead, which is not applicable to latency sensitive workloads.  
%Figure~\ref{fig:power_profile} shows the power consumption for Xeon-E5 2680 processor with C1 and C6 processor sleep state enabled respectively. The power numbers are collected using PAPI API that interacts with the RAPL (Runing Average Power Limit) interfaces. %From the figure we can see that processor in  package C6 sleep state consumes much less power than processor in active state. 
%When the processor is in the \emph{C0} state, it may be associated with a performance state \emph{Px}, which corresponds to a specific DVFS setting. A hierarchical view of the low-power states specified in ACPI is shown in~\ref{fig:acpi_diagram}. The combination of system low-power state and CPU low-power state is used to characterize the low-power mode of an entire server. 
%\begin{figure}[h]
%	\centering
%	\vspace{-0.1in}
%	\centering
%	\includegraphics[scale=0.6]{./figure/power-profile.pdf}
%	\caption[Test]{Power profile of a 10-core Xeon processor with different C-state configurations. The y-axis is the range of power for the processor with the specific number of cores active and various utilization levels ranging from 10\% to 100\%.} %Note that each of the active cores settings, we generate various level of utilization to the active cores and measured the power, which explains why the power consumption for a specific number of active cores are a range of numbers.  }
%	\label{fig:power_profile}
%	\vspace{-0.1in}
%\end{figure}
%\footnote{We use a microbenchmark that can calibrate itself and occupy the core according to each utilization setting. To occupy multiple cores, we run multiple processes of this microbenchmark, each pinned to a specific core.}
\subsection{Server and Job Model}
We model the server farm as a multi-server system that could process multiple jobs (upto the number of total cores) at a time. 
%In this paper, we use four synthetic workloads with average job execution times shown in brackets next to them: Google search [4.2 ms], Apache [75 ms], Mail [92 ms] and DNS query [194 ms] jobs, and one real system trace, Wikipedia, with an average workload execution time of 3.5 ms. 
%The job execution time parameters were derived from prior works and actual workload traces~\cite{wiki_trace,meisner2012dreamweaver}. 
{\em Utilization factor} is defined as the product of the job arrival rate and the average execution time, which is also the fraction of time that the server is expected to be busy executing a job.
%The term {\em Utilization factor} is defined as $\rho=\frac{\lambda}{\mu}$, the fraction of time the server is expected to be busy executing a job. 
We assume that a system-wide load balancer dispatches jobs to the servers within the server farm. 
%{\bf FAN: Plug in details about the window of observation, number of servers}. 
The {\em job latency} is defined as the time elapsed from when a job arrives to when the job completes its execution and departs the server. In this paper, the $90^{th}$ percentile job latency is considered as the QoS target.
%\begin{figure}[ht]
%	\centering
%	%\subfloat[b][Overview of \titlename Hiearchical Algorithms]{
%	\includegraphics[scale=0.3]{./figure/algorithm_chart.pdf}
%	%}
%	%	\vspace{-0.3in}
%	%	\subfloat[b][MPPP]{
%	%		\includegraphics[scale=0.58]{../figure/scalability/google_scal_mmpp.pdf}
%	%		\label{fig:google_scal_mmpp}}
%	\caption{\titlename Power Management Framework.}
%	\label{fig:alg_overview}
%	\vspace{-0.2in}
%\end{figure}



==> exp_setup.tex <==
\section{Experimental Setup} 
We perform two sets of experiments: 1. simulations to explore the Pareto-optimal energy-latency tradeoff as well as corresponding $T_s$, $T_w$ and $\tau$ settings, and 2. prototype implementation on a testbed with web server deployment. In this section, we elaborate on the experimental setup for both approaches.
\begin{figure}[htbp]
	\captionsetup{font=small}
	\centering
	\includegraphics[scale=0.60]{./figure/power_profile_cloud.pdf}
	\caption[test]{Power profile of a 10-core Xeon E5 processor with C0-C1 and C0-C6 transition settings whenever the server is idle.\protect\footnotemark}
	\label{fig:power_profile}
\end{figure}
\footnotetext{We use a microbenchmark that can calibrate itself and occupy the core based on required utilization settings. To occupy multiple cores, we run multiple copies of this microbenchmark each pinned to a core.}

\begin{table}[htbp]
	\footnotesize
	\captionsetup{font=small}
	\centering	
    \caption{Power (W) breakdown for a system with $n_{a}$ active cores} 
	\begin{tabular}{|p{1.5cm}<{\centering}|p{1.3cm}<{\centering}|p{1.4cm}<{\centering}|p{1.3cm}<{\centering}|p{0.8cm}<{\centering}|}
		\hline
		\multirow{2}{*}{\bf Component} & Core sleep C1$^{\ast}$& Core sleep C6 $^{\dagger}$& Pkg. sleep C6 &  System sleep \\
		\hline
		%	{\bf Component} & Core sleep & Core sleep&Pack. sleep & Server sleep \\
		%	& C1& C6 & C6&   \\
		%  \hline
		\multirow{2}{*}{CPU} & 33.0+$3.1\times(n_{a}-1)$ & 23.0+$3.8\times(n_{a}-1)$ & \multirow{2}{*}{8.3} & \multirow{2}{*}{8.3} \\
		%\hline
		%{Chipset~\cite{liu2014sleepscale}} & 3.7 & 3.7 & 3.7 & 3.7 \\
		\hline
		RAM~\cite{intel_e5}     & 10.8 & 10.8 & 4.9 & 1.4 \\
		\hline
		Platform~\cite{powernap}     & 45.5 & 45.5 & 23.6 & 4.8 \\
		\hline
		\multirow{2}{*}{Total Power} & 89.3+$3.1\times(n_{a}-1)$ & 79.3+$3.8\times(n_{a} -1)$ & \multirow{2}{*}{36.8} & \multirow{2}{*}{14.5} \\
		\hline	
	\end{tabular} \\
	${\ast} $ processor is active and the rest of the idle cores are in $C1$ state. \\ 
	$\dagger$ processor is active and the rest of the idle cores are in $C6$ state.
	\label{table:powermode}
\end{table}

\begin{table}[htbp]
	\footnotesize
	\captionsetup{font=small}
	\centering
    \caption{Processor/System low-power states and wakeup latencies}
	\begin{tabular}{|c|c|c|}
		\hline
		Low-power State & Wake-up latency \\ \hline
		core sleep C1   & 10 $\mu$s           \\ \hline
		core sleep C6   & 82 $\mu$s           \\ \hline
		package sleep C6   & 1 ms           \\ \hline
		system sleep    & 5 s      \\ \hline
	\end{tabular}    
	\vspace{-0.15in}
	\label{table:latency-table}
\end{table}

\subsection{Processor Power Profile and Server Power Model}

We profile the power consumption of the Intel Xeon E-5 processor~\cite{intel_e5} using Intel's \emph{Running Average Power Limit} (RAPL) interface. We build a customized cpuidle governor that allows specified low-power state transitions. The processor is programmed to transition between active state (C0) and low-power state $Cx$ (e.g., C1, C6). Figure~\ref{fig:power_profile} shows the measured power consumption of the processor for two configurations: \emph{C0-C1}, \emph{C0-C6} and at utilization levels from 0\% to 100\%. Using linear regression, a power model is built for the processor based on the sleep state selection and the number of active cores at full utilization. Table~\ref{table:powermode} shows the power consumption when a certain state is chosen for sleep mode. Table~\ref{table:latency-table} shows the wakeup latencies for various low-power states. Note that the processor sleep state transition latencies are reported by the Linux cpuidle driver~\cite{pallipadi2007cpuidle}.

\subsection{Simulation Platform}

\titlename uses an event-driven simulator based on Bighouse~\cite{bighouse} that models server farm workloads and multi-server activity. We simulate a server farm with 100 ten-core servers (by default).  In all of our experimental results, we report the steady state statistics by disregarding the warm-up period of the first 10,000 jobs. In the simulation, we use short latency (Web service-like) jobs with $s=4.2 ms$ and long latency (DNS service-like) jobs with $s=194 ms$ as representatives based on prior studies~\cite{powernap}. For each of the representative workloads, we generate synthetic job arrivals with different utilization levels (0.1 for low, 0.3 for average~\cite{barroso_isca07}, and 0.6 for high). Random job arrivals are modeled by Poisson process~\cite{meisner2012dreamweaver}. Besides synthetic workload, we also perform simulation based on Wikipedia traces.

\subsection{Real System Experiments on Testbed}

We deploy a testbed with a cluster of 10 application servers together with one load-generating server and one load-balancing server; all servers support Intelligent Power Management Interface (IPMI) interface~\cite{openipmi} for system-level power monitoring. Each application server is configured with the apache web service. The load generator keeps sending web requests to the system according to real system traces (See Section~\ref{sec:evaluation} for further details).


==> job_model.tex <==
\subsection{Modeling Job{\color{blue}-------$>$Multi-task v.s. single-task job models}}
We model the execution of jobs at the server side as follows. A job consists of multiple inter-dependent tasks that include both spatial and temporal inter-dependence. Application tasks are typically executed by specific server types. For example, a web service request will first be processed by an application or web server, and a search request is processed by a database server, and this kind of task relationship is called spatial inter-dependence. In terms of temporal inter-dependence, a task cannot start executing until all of its 'parent' tasks have finished their execution, and until after their results have been communicated to the server assigned to the task. A job is considered to have finished when all of its tasks finish execution. As for servers, there are multiple cores per server and one core can only process one task. In this paper, we configure single-core processor for the servers.

Each job $j$ can be represented as a directed acyclic graph (DAG) $G^j(V^j, E^j)$, where $V^j$ is the set of tasks of job $j$. In DAG, if there is a link from task $i$ to task $r$, then task $i^j$ must finish and communicate its results to task $r^j$ before $r^j$ can start processing. Each task $v^j \in V^j$ has a workload requirement, namely task size or execution time requirement $w^j_v$ for the core. For each link in $E^j$, there is a data transfer size $D^j_l$ associated with it, which denotes the bandwidth requirement to transfer the result over link $l$ (from the task at the head of DAG link to the task at the tail) when assigned a network flow. Figure~\ref{figure1} shows an example of a job DAG.

%\begin{figure}[htbp]
%	\captionsetup{font=small}
%	\centering
%	\vspace{-0.1in}
%	\includegraphics[scale=1.0]{./figures/wsDAG.eps}
%	\caption[test]{Example of a web service job DAG. Task 1 is executed by the application server, while task 2 is assigned to be processed by database server.\protect\footnotemark}
%	\label{fig:wsDAG}
%	\vspace{-0.1in}
%\end{figure}

\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.15\textwidth]{figures/DAG.pdf}\caption{Example of a job DAG. Numbers 1-6 denote task 1-task 6 respectively. Numbers around the tasks represent task size, while numbers on the links represent flow size.}
	\label{figure1}
\end{figure}

\begin{figure}
	\captionsetup{font=small}
	\centering\includegraphics[width=0.5\textwidth]{figures/fat_tree.png}
	\caption{Fat tree topology.}
	\label{figure12}
\end{figure}

==> trace_eva.tex <==
\section{Evaluation on Real System}
\label{sec:evaluation}

\begin{figure*}[htbp]
	\centering
	\captionsetup{font=small}
	\includegraphics[scale=0.56]{./figure/combine-energy.pdf}
	\caption{\label{fig:per-server-energy} Energy measured on a server farm with 10 servers with different energy management policies.  The first three groups of bars represent energy breakdown in each server when Active-Idle, Delay-Doze and \titlename are applied, respectively. The rightmost three bars illustrate the total server farm energy consumption for Active-Idle (black bar), Delay-Doze (gray bar) and \titlename respectively (white bar).}	
\end{figure*}

We evaluate \titlename on a testbed with 10 Dell Poweredge servers equipped with Inten Xeon-based processors with all of the servers deployed on a dedicated rack. We installed a modified version of the Apache HTTP server for our Local Power Controller. We extended the Local Power Controller to also include a Delay-Doze timer. The Global Server Farm Power Manager is added to an additional apache server with the \emph{mod\_proxy\_balancer} module used for load balancing. Specifically, the load balancer performs operating mode transitions in servers (as discussed in Section~\ref{sec:handler}); this is done by sending special HTTP requests (\emph{/hostname/trans-to-active-mode/}, \emph{/hostname/trans-to-lp-mode}) to the application server. It also monitors the power state for each server, and manages the server wakeups (from system sleep) using IPMI interface supported by Dell systems. The special requests are handled by the local power controller that would determine the server low-power transitions accordingly. We set up a custom cpuidle governor which allows direct processor C-state transitions from userspace (e.g., C0-C6). For power measurement, we leverage two techniques: the RAPL interface for fine-grained component power, and the IPMI's system power management interface for coarse-grained server power. We evaluate the effectiveness of \titlename by providing two sets of workloads to the system: the non-bursty Wikipedia workload, that does not require server provisioning, and four bursty NLANR workloads~\cite{nlanr}, that require server provisioning to handle bursty workloads (See section~\ref{sec:provision}).

\subsection{Wikipedia Trace}
\label{sec:bursty-trace}

We performed real system energy measurements by deploying Wikipedia software stack, namely Wikipedia application (Mediawiki), database system (Mysql) on servers. We compare \titlename against Active-Idle and Delay-Doze approaches described in Section~\ref{sec:smartlp}. To capture detailed energy breakdown, we leverage RAPL interface for fine-grained power measurement. The RAPL utility records the CPU and RAM power values periodically. We configure \titlename with the $T_s$, $T_w$ and $\tau$ parameters that achieve energy-latency Pareto-optimality with tail latency constraint set to 2.0. Similarly, for Delay-Doze, we explore various
values of the delay-timer and choose the setting that achieves the best power with the same tail latency constraint. From our experiments, we get actual CPU and RAM energy consumption for each server. To get the overall server energy, we also factored in the platform energy shown in Table~\ref{table:powermode}. 

Figure~\ref{fig:per-server-energy} shows the per-server energy breakdown in terms of CPU, DRAM, and platform energy. With Active-Idle power management, all the 10 servers have similar energy consumption. With Delay-Doze, some of the servers are able to stay in system sleep state for longer periods of time, thus saving energy. With \titlename, we can clearly see that most of the servers drastically reduce energy consumption, and only a minimal subset of servers (server\#6 and \#10) are used for servicing jobs. Note that the energy consumption of server\#10 is slightly higher than that of Active-Idle power management since the server is at a higher utilization level while other servers remained inactive. Overall, \titlename gains 39\% reduction in energy saving compared to Delay-Doze, and 56\% energy savings compared to Active-Idle.

\begin{figure}[htbp]
	\centering
	\subfloat[ny09]{
		\includegraphics[scale=0.34]{./figure/ny09.pdf}
		\label{fig:nlanr-ny09}
		\hspace{0.05in}
	}
	\subfloat[pa09]{
		\includegraphics[scale=0.34]{./figure/pa09.pdf}
		\label{fig:nlanr-pa09}
		%\hspace{0.2in}
	}
	
	\subfloat[pa10]{
		\includegraphics[scale=0.34]{./figure/pa10.pdf}
		\label{fig:nlanr-pa10}
		\hspace{0.05in}
	}
	\subfloat[uc09]{
		\includegraphics[scale=0.34]{./figure/uc09.pdf}
		\label{fig:nlanr-uc09}
		%\hspace{0.2in}
	}
	\caption{System utilization for four bursty traces.}
	\label{fig:utilizations}
\end{figure}
\begin{figure}[htbp]
	\centering
	\includegraphics[scale=0.45]{./figure/trace-eval/trace_result.pdf}
	\caption{Normalized energy consumption relative to peak energy on a 10-server cluster}
	\label{fig:traceresults}
\end{figure}

\subsection{Bursty Traces}
\label{sec:nonbursty-trace}

 As the raw NLANR network traces~\cite{nlanr} present job arrivals that are too infrequent for the server farm system with 10 application servers (less than 2\%), we speed up the trace by scaling the 24-hour trace to one hour. We choose four traces, namely \emph{ny09}, \emph{pa09}, \emph{pa10} and \emph{uc09}. Figure~\ref{fig:utilizations} shows the utilization levels (scaled) for the four traces over one hour. All traces exhibit bursty traffic patterns. For example, the \emph{ny09} trace has highly fluctuating utilizations ranging from 4\% to 45\% with a large number of spikes. To run the traces, we set up a software stack similar to the one in Section~\ref{sec:bursty-trace}. Each request in the trace is serviced by a PHP script that accesses a pre-defined set of pages randomly, and we note that the average service time is about the same as Wikipedia web requests.
 
To enable server provisioning, the Server Farm Power Manager additionally samples the server farm utilization levels based on the job arrival rates. Utilization is calculated as the product of job arrival rate and average job execution time. Standard deviation on the samples for utilization levels is calculated every 120 seconds. The number of provisioned servers is calculated dynamically (See Section~\ref{sec:provision} for details). Note that, in our comparative studies, the delay-timer values are re-evaluated for each trace such that best possible energy savings are had while meeting the QoS constraints. Figure~\ref{fig:traceresults} shows the energy consumption for the four bursty workloads using Active-Idle, Delay-Doze and \titlename. The energy is normalized to the peak energy which is $PeakPower*Time$. The energy reduction for \titlename ranges from 34\% to 40\% compared to Active-Idle. Even with the best delay timer settings, Delay-Doze only achieves 9\% to 12\% energy reduction in bursty workloads. We observe that due to the job arrival rate spikes (especially for \emph{uc09}), in order for Delay-Doze to meet the tail latency constraint of 2.0, the delay timer has to be set to larger values, and in turn the servers have limited chance to enter system sleep state.


